Layered Drawing of Undirected Graphs with Generalized Port Constraints

The aim of this research is a practical method to draw cable plans of complex machines. Such plans consist of electronic components and cables connecting specific ports of the components. Since the machines are configured for each client individually, cable plans need to be drawn automatically. The drawings must be well readable so that technicians can use them to debug the machines. In order to model plug sockets, we introduce port groups; within a group, ports can change their position (which we use to improve the aesthetics of the layout), but together the ports of a group must form a contiguous block. We approach the problem of drawing such cable plans by extending the well-known Sugiyama framework such that it incorporates ports and port groups. Since the framework assumes directed graphs, we propose several ways to orient the edges of the given undirected graph. We compare these methods experimentally, both on real-world data and synthetic data that carefully simulates real-world data. We measure the aesthetics of the resulting drawings by counting bends and crossings. Using these metrics, we experimentally compare our approach to Kieler [JVLC 2014], a library for drawing graphs in the presence of port constraints. Our method produced 10--30 % fewer crossings, while it performed equally well or slightly worse than Kieler with respect to the number of bends and the time used to compute a drawing.

==> nbpCM_generated_2021-08-06_17-27-03.tex <==
ports/kieler	mixed/kieler	nodes/kieler	vtcs
1.0452488687782806	1.0633484162895928	1.081447963800905	68.0
1.0263424518743667	1.0243161094224924	1.044579533941236	182.0
0.9540229885057471	0.9770114942528736	1.1149425287356323	33.0
1.0713305898491083	1.0823045267489713	1.046639231824417	172.0
1.0838709677419356	1.0677419354838709	1.064516129032258	145.0
1.0201342281879195	1.0536912751677852	1.087248322147651	81.0
0.9876160990712074	1.0309597523219813	1.0495356037151702	90.0
1.070469798657718	1.0771812080536913	1.070469798657718	142.0
1.0791057609630266	1.0705073086844368	1.0722269991401547	224.0
1.0	0.967741935483871	0.967741935483871	41.0
1.0590979782270606	1.0870917573872472	1.0715396578538103	150.0
0.9819168173598554	1.0795660036166366	1.0795660036166366	142.0
0.987220447284345	1.02555910543131	1.0319488817891374	96.0
1.0082236842105263	1.0082236842105263	1.0394736842105263	204.0
0.963963963963964	0.9099099099099099	1.0	48.0
1.0169252468265162	1.0169252468265162	1.0366713681241184	134.0
1.1033707865168538	1.1033707865168538	1.0764044943820226	139.0
0.9821428571428571	1.0357142857142858	1.0	41.0
1.115138592750533	1.1108742004264391	1.0895522388059702	145.0
1.0661870503597122	1.0920863309352518	1.0661870503597122	169.0
0.8532110091743119	0.926605504587156	0.8532110091743119	23.0
1.0441176470588236	1.0522875816993464	1.0800653594771241	228.0
0.9965217391304347	0.9408695652173913	0.9547826086956521	127.0
1.048151332760103	1.065348237317283	1.063628546861565	236.0
0.970873786407767	0.9611650485436893	0.9368932038834952	100.0
1.048780487804878	1.070460704607046	1.0921409214092141	109.0
1.0	1.0465116279069768	1.0465116279069768	32.0
1.093189964157706	1.064516129032258	1.1433691756272402	75.0
1.0400801603206413	1.0681362725450902	1.0480961923847696	133.0
1.0357941834451903	1.0447427293064877	1.0626398210290828	111.0
1.0	1.0198019801980198	1.0132013201320131	84.0
1.0483271375464684	1.0483271375464684	1.0780669144981412	134.0
1.018970189701897	1.0542005420054201	1.065040650406504	174.0
1.0711462450592886	1.08300395256917	1.08300395256917	143.0
1.1231422505307855	1.1061571125265393	1.029723991507431	126.0
1.063730084348641	1.0899718837863168	1.0731021555763824	213.0
1.0425531914893618	1.0921985815602837	1.049645390070922	89.0
0.9550561797752809	0.9662921348314607	1.0449438202247192	43.0
0.9912663755458515	0.9912663755458515	1.0	49.0
1.0676923076923077	1.08	1.08	78.0
1.0683760683760684	1.064957264957265	1.123076923076923	115.0
1.0230642504118617	1.0790774299835255	1.0395387149917628	142.0
1.0446428571428572	1.0386904761904763	1.0446428571428572	156.0
1.0613496932515338	1.0920245398773005	1.098159509202454	158.0
1.0	1.008695652173913	1.0434782608695652	68.0
1.0	1.0	0.6	9.0
0.937984496124031	1.0310077519379846	1.062015503875969	39.0
1.0	1.0	1.0	11.0
1.1167883211678833	1.1119221411192215	1.1508515815085159	128.0
1.0761904761904761	1.1047619047619048	1.1142857142857143	131.0
0.75	0.75	1.25	20.0
1.0	1.0	1.0	12.0
1.0141843971631206	0.9716312056737588	1.0283687943262412	40.0
1.0685871056241427	1.0548696844993142	1.0823045267489713	179.0
1.083989501312336	1.0892388451443569	1.141732283464567	91.0
1.1136363636363635	1.106060606060606	1.128787878787879	71.0
1.0712250712250713	1.0883190883190883	1.1139601139601139	205.0
0.9874213836477987	1.0251572327044025	1.0	36.0
1.0410958904109588	1.0456621004566211	1.0456621004566211	126.0
0.9152542372881356	0.8305084745762712	0.9491525423728814	58.0
1.0357142857142858	1.096938775510204	1.0765306122448979	99.0
1.0554156171284634	1.070528967254408	1.0856423173803527	150.0
1.0496277915632755	1.0397022332506203	1.0297766749379653	91.0
0.9669421487603306	0.9889807162534435	1.022038567493113	105.0
1.0052631578947369	1.0421052631578946	1.0052631578947369	105.0
1.0113636363636365	1.0	1.0340909090909092	52.0
1.0987654320987654	1.0658436213991769	1.0905349794238683	104.0
1.1366459627329193	1.0993788819875776	1.2236024844720497	68.0
1.0333333333333334	1.0380952380952382	1.1095238095238096	129.0
1.0721003134796239	1.0909090909090908	1.084639498432602	189.0
1.0253164556962024	1.0084388185654007	1.0421940928270041	61.0
1.0831826401446654	1.0687160940325497	1.0687160940325497	157.0
0.52	0.76	0.76	8.0
1.0	1.0	1.0	7.0
1.1171003717472119	1.0985130111524164	1.1115241635687731	213.0
0.75	0.75	0.75	4.0
1.0590405904059041	1.007380073800738	1.044280442804428	154.0
1.0	1.0	1.0	16.0
1.0235294117647058	1.0235294117647058	1.0494117647058823	169.0
1.0417910447761194	0.991044776119403	1.035820895522388	132.0
1.0778032036613272	1.1006864988558351	1.1189931350114417	126.0
0.9842395587076438	0.9952718676122931	1.0063041765169425	203.0
1.0390455531453362	1.0650759219088937	1.0607375271149675	109.0
1.0397727272727273	1.0397727272727273	1.0113636363636365	79.0
1.0437158469945356	1.1202185792349726	1.098360655737705	50.0
0.9215686274509803	0.8901960784313725	0.9764705882352941	46.0
1.046376811594203	1.0811594202898551	1.046376811594203	105.0
0.9298245614035088	0.9298245614035088	0.9473684210526315	57.0
1.067476383265857	1.05668016194332	1.0512820512820513	143.0
1.062937062937063	1.055944055944056	1.020979020979021	96.0
1.0703703703703704	1.0592592592592593	1.025925925925926	131.0
1.1320754716981132	1.1132075471698113	1.2452830188679245	47.0
1.1201923076923077	1.1009615384615385	1.1009615384615385	117.0
1.0	1.0053475935828877	1.0909090909090908	90.0
0.7543859649122807	0.8596491228070176	0.8596491228070176	24.0
0.9946666666666667	1.032	1.048	98.0
1.0952380952380953	1.0952380952380953	1.0952380952380953	15.0
1.0	1.0	1.0	4.0
1.0617495711835334	1.0308747855917668	1.0445969125214407	129.0
1.1498371335504887	1.1824104234527688	1.1433224755700326	81.0
1.0392857142857144	1.0285714285714285	1.025	139.0
1.0803212851405624	1.0481927710843373	1.0562248995983936	92.0
1.0471567267683772	1.0748959778085991	1.0804438280166435	168.0
1.0746268656716418	1.0845771144278606	1.1044776119402986	117.0
1.0	1.0	1.0	7.0
1.0520673813169985	1.0826952526799387	1.0735068912710566	158.0
1.0180831826401446	1.0289330922242315	1.057866184448463	136.0
0.8924731182795699	0.9139784946236559	0.9139784946236559	34.0
1.0790123456790124	1.0592592592592593	1.0716049382716049	162.0
1.0465116279069768	1.1395348837209303	1.1395348837209303	34.0
1.0648508430609598	1.0752269779507133	1.1037613488975357	177.0
0.9727272727272728	1.0909090909090908	1.0363636363636364	76.0
1.0646976090014064	0.9774964838255977	1.0646976090014064	164.0
1.3214285714285714	1.3214285714285714	1.2261904761904763	55.0
1.0952380952380953	1.1216931216931216	1.0846560846560847	122.0
1.0550206327372764	1.0632737276478679	1.0632737276478679	180.0
1.0	1.0	1.0	6.0
1.0518518518518518	1.0592592592592593	1.0666666666666667	127.0
1.0763358778625953	1.0641221374045802	1.0519083969465648	140.0
1.0	1.0553846153846154	1.0369230769230768	78.0
1.014336917562724	0.9713261648745519	0.985663082437276	69.0
1.055790363482671	1.040574809805579	1.0507185122569738	243.0
1.0425531914893618	1.0425531914893618	1.127659574468085	34.0
1.3333333333333333	1.3333333333333333	1.3333333333333333	28.0
1.0843373493975903	1.0602409638554218	1.1024096385542168	87.0
0.9473684210526315	0.868421052631579	0.8421052631578947	22.0
1.075046904315197	1.0637898686679175	1.0712945590994372	142.0
1.061965811965812	1.1047008547008548	1.0876068376068375	219.0
0.9583333333333334	0.8333333333333334	1.0	29.0
1.0	1.0615384615384615	1.0615384615384615	17.0
1.013179571663921	0.957166392092257	0.9934102141680395	120.0
1.08876560332871	1.1220527045769764	1.1359223300970873	168.0
1.0857787810383748	1.0406320541760723	1.090293453724605	114.0
0.9556962025316456	0.9493670886075949	1.018987341772152	93.0
0.9090909090909091	0.7272727272727273	0.7272727272727273	15.0
0.9411764705882353	0.8235294117647058	0.9411764705882353	14.0
1.1214953271028036	1.0093457943925233	1.1401869158878504	64.0
1.1155433287482805	1.0852819807427785	1.0880330123796425	120.0
1.0750246791707798	1.102665350444225	1.0888450148075024	219.0
1.0357142857142858	1.0178571428571428	1.1071428571428572	56.0
1.0272727272727273	1.0	1.0636363636363637	94.0
1.0932038834951456	1.0815533980582523	1.0776699029126213	132.0
1.058091286307054	1.103734439834025	1.0829875518672198	115.0
0.9367088607594937	0.9113924050632911	0.9683544303797469	82.0
1.0	1.0	1.0	5.0
1.1157407407407407	1.0833333333333333	1.1157407407407407	127.0
1.0869565217391304	1.0905797101449275	1.0833333333333333	145.0
1.0744416873449132	1.1042183622828785	1.1215880893300247	195.0
1.0929432013769362	1.072289156626506	1.0963855421686748	150.0
1.031496062992126	1.047244094488189	1.125984251968504	32.0
1.0546875	1.015625	1.04296875	120.0
1.0220750551876379	0.9801324503311258	0.9845474613686535	155.0
1.0	0.9338842975206612	0.9338842975206612	40.0
1.0633802816901408	1.056338028169014	1.0633802816901408	108.0
1.018018018018018	0.963963963963964	1.0360360360360361	41.0
0.9787234042553191	1.0106382978723405	1.0319148936170213	24.0
0.9294117647058824	0.9764705882352941	1.0941176470588236	29.0
0.974169741697417	1.029520295202952	1.055350553505535	135.0
1.088235294117647	1.0522875816993464	1.0784313725490196	146.0
1.0753768844221105	1.0477386934673367	1.0829145728643217	200.0
1.129496402877698	1.1103117505995204	1.091127098321343	129.0
1.037914691943128	0.995260663507109	1.018957345971564	105.0
1.0948275862068966	1.0258620689655173	1.1293103448275863	81.0
1.0495867768595042	1.0661157024793388	1.0743801652892562	134.0
0.9806295399515739	0.9418886198547215	1.0145278450363195	103.0
1.0264550264550265	1.037037037037037	1.0423280423280423	98.0
0.9775280898876404	0.9775280898876404	1.0224719101123596	36.0
1.1055408970976253	0.9894459102902374	1.0686015831134565	78.0
1.0873634945397816	1.0748829953198127	1.0748829953198127	169.0
1.0712589073634204	1.0712589073634204	1.0380047505938241	113.0
0.974025974025974	1.0311688311688312	1.0415584415584416	119.0
0.9846153846153847	0.9307692307692308	1.0076923076923077	76.0
1.0869565217391304	1.0747826086956522	1.0660869565217392	251.0
1.0830324909747293	1.1010830324909748	1.0902527075812274	157.0
1.0868761552680222	1.077634011090573	1.088724584103512	208.0
1.031201248049922	1.0904836193447738	1.0842433697347893	154.0
1.0929487179487178	1.0480769230769231	1.1121794871794872	190.0
1.0563758389261746	1.0697986577181209	1.0644295302013422	124.0
0.9714285714285714	0.9428571428571428	0.9428571428571428	39.0
1.0636042402826855	1.0424028268551238	1.098939929328622	92.0
0.9755351681957186	1.0122324159021407	1.0305810397553516	98.0
1.0527306967984935	1.0677966101694916	1.0941619585687383	138.0
1.1219512195121952	1.146341463414634	1.2439024390243902	53.0
1.1108508977361435	1.088992974238876	1.079625292740047	250.0
1.0869565217391304	1.0217391304347827	1.0	40.0
1.0249376558603491	1.0249376558603491	1.0698254364089776	112.0
1.1215469613259668	1.0994475138121547	1.1104972375690607	86.0
1.0	1.2222222222222223	1.2222222222222223	21.0
1.0	1.0	1.0	30.0
1.092116917626218	1.1062887511071744	1.0974313551815766	226.0
1.0276243093922652	0.988950276243094	1.0828729281767955	103.0
1.0954907161803713	1.0583554376657824	1.063660477453581	97.0
1.0597014925373134	1.0835820895522388	1.1194029850746268	106.0
1.1008695652173912	1.1182608695652174	1.111304347826087	140.0
1.0	1.0636942675159236	1.0	87.0
1.0907759882869692	1.0409956076134699	1.0878477306002927	183.0
1.0974658869395713	1.0818713450292399	1.0818713450292399	139.0
1.0643564356435644	1.0544554455445545	1.0742574257425743	118.0
1.0394736842105263	1.0	1.0263157894736843	41.0
1.0907127429805616	1.08207343412527	1.0777537796976242	143.0
1.0	1.0	1.0	15.0
1.0196078431372548	1.0784313725490196	1.1372549019607843	57.0
1.0792540792540792	1.0745920745920745	1.0326340326340326	113.0
1.0	1.0618556701030928	1.0	45.0
0.9798994974874372	0.9698492462311558	1.015075376884422	107.0
0.9617834394904459	0.9299363057324841	1.0	88.0
1.0754716981132075	1.0754716981132075	1.0377358490566038	34.0
1.044424700133274	1.0550866281652598	1.0648600621945803	352.0
1.0878136200716846	1.0878136200716846	1.0806451612903225	247.0
1.0317880794701986	1.0688741721854305	1.047682119205298	158.0
0.75	1.0	1.0	20.0
1.043010752688172	0.978494623655914	1.086021505376344	23.0
1.0772727272727274	1.1045454545454545	1.1272727272727272	122.0
1.0	1.0	1.0	10.0
1.0	1.4444444444444444	1.4444444444444444	18.0
1.085343228200371	1.0667903525046383	1.0927643784786643	146.0
0.6666666666666666	1.0	0.6666666666666666	6.0
1.051044083526682	1.0185614849187936	1.0788863109048723	127.0
1.0952380952380953	1.0714285714285714	1.0873015873015872	107.0
1.0803212851405624	1.0803212851405624	1.037483266398929	189.0
1.038709677419355	0.9354838709677419	1.0903225806451613	42.0
1.051107325383305	1.020442930153322	1.0374787052810903	167.0
1.1087267525035764	1.1030042918454936	1.111587982832618	133.0
1.0442338072669826	1.0410742496050553	1.0537124802527646	140.0
0.9876543209876543	0.9753086419753086	0.9876543209876543	52.0
1.0884955752212389	1.0707964601769913	1.079646017699115	103.0
1.0861244019138756	1.1033492822966506	1.0746411483253588	203.0
1.031496062992126	1.062992125984252	1.094488188976378	55.0
1.010204081632653	1.0408163265306123	1.0204081632653061	49.0
1.075657894736842	1.075657894736842	1.0723684210526316	143.0
1.0509259259259258	1.0601851851851851	1.1064814814814814	118.0
1.0192307692307692	1.0	1.0528846153846154	97.0
1.0798065296251511	1.0725513905683193	1.0918984280532043	183.0
0.930635838150289	0.930635838150289	1.092485549132948	22.0
0.8367346938775511	0.8367346938775511	0.8979591836734694	38.0
1.082004555808656	1.0956719817767653	1.1047835990888382	191.0
1.087227414330218	1.0685358255451713	1.074766355140187	103.0
1.0348432055749128	1.0	1.0348432055749128	112.0
1.0588235294117647	1.0147058823529411	1.0588235294117647	66.0
1.065040650406504	1.032520325203252	1.065040650406504	89.0
1.1043324491600353	1.090185676392573	1.0919540229885059	252.0
1.0347826086956522	1.0472049689440994	1.0372670807453417	154.0
1.0812807881773399	1.0714285714285714	1.103448275862069	174.0
1.0903790087463556	1.1049562682215743	1.1020408163265305	156.0
1.0506970849176172	1.0785804816223068	1.0988593155893536	197.0
1.099290780141844	1.0939716312056738	1.1187943262411348	233.0
1.0	1.0769230769230769	1.0769230769230769	38.0
1.1103117505995204	1.0767386091127098	1.1103117505995204	127.0
1.017751479289941	1.0414201183431953	1.0414201183431953	99.0
1.0785219399538106	1.0877598152424943	1.103156274056967	245.0
1.1168831168831168	1.0649350649350648	1.1168831168831168	69.0
1.0920096852300243	1.0677966101694916	1.0968523002421307	128.0
1.088176352705411	1.0961923847695392	1.1002004008016033	145.0
1.0648854961832062	1.0114503816793894	1.0801526717557253	120.0
1.1026894865525672	1.0904645476772616	1.078239608801956	178.0
1.065359477124183	1.065359477124183	1.065359477124183	93.0
1.0720871751886	1.0653813914501258	1.0838222967309303	243.0
1.0510204081632653	1.0459183673469388	1.0357142857142858	122.0
1.0686274509803921	1.1568627450980393	1.088235294117647	59.0
1.0	1.010909090909091	1.0436363636363637	112.0
1.0	1.0	0.8076923076923077	28.0
1.05	1.06875	1.05	142.0
1.0502901353965184	1.0386847195357833	1.0309477756286267	121.0
1.1481481481481481	1.0740740740740742	1.1481481481481481	24.0
1.0738552437223043	1.06794682422452	1.0738552437223043	157.0
1.053763440860215	1.043010752688172	1.053763440860215	161.0
0.9818181818181818	1.018181818181818	1.0909090909090908	31.0
0.994579945799458	0.978319783197832	1.08130081300813	108.0
1.069767441860465	1.0174418604651163	1.052325581395349	104.0
1.054054054054054	1.027027027027027	1.0675675675675675	94.0
1.0986666666666667	1.0826666666666667	1.1146666666666667	122.0
1.1437125748502994	1.0119760479041917	1.1437125748502994	42.0
1.0462633451957295	1.0284697508896796	1.0747330960854093	145.0
1.031496062992126	1.047244094488189	1.073490813648294	88.0
1.0436363636363637	1.0533333333333332	1.0678787878787879	190.0
1.0365296803652968	0.9908675799086758	1.091324200913242	74.0
1.0588235294117647	1.0	0.9558823529411765	63.0
0.9849624060150376	0.9849624060150376	0.9548872180451128	50.0
1.1604938271604939	1.0864197530864197	1.1728395061728396	68.0
1.0361663652802893	1.0289330922242315	1.0253164556962024	158.0
1.084664536741214	1.071884984025559	1.0878594249201279	240.0
1.0734341252699784	1.0129589632829374	1.0647948164146868	102.0
1.0992167101827677	1.08355091383812	1.114882506527415	97.0
1.0	1.375	1.0	28.0
1.0	0.9473684210526315	1.0789473684210527	36.0
1.0509915014164306	1.158640226628895	1.0623229461756374	89.0
1.079744816586922	1.0574162679425838	1.0733652312599682	165.0
1.1158798283261802	1.0987124463519313	1.1072961373390557	152.0
1.0952380952380953	1.0952380952380953	1.0	28.0
1.1145833333333333	1.0625	1.0833333333333333	52.0
1.0792602377807134	1.0871862615587846	1.095112285336856	187.0
1.045	0.995	1.05	90.0
1.055045871559633	1.018348623853211	1.073394495412844	60.0
0.5384615384615384	0.5384615384615384	0.8461538461538461	13.0
1.1179245283018868	1.1273584905660377	1.1226415094339623	94.0
1.0521008403361345	1.0638655462184874	1.0924369747899159	233.0
1.0831556503198294	1.0533049040511726	1.070362473347548	227.0
1.0	1.0	1.0	6.0
1.0482456140350878	1.0570175438596492	1.0789473684210527	135.0
1.0440097799511003	1.061124694376528	1.0880195599022005	152.0
1.1379310344827587	0.9310344827586207	1.0	38.0
1.0	1.0	1.0	6.0
0.9943181818181818	1.0625	1.0227272727272727	93.0
0.9166666666666666	0.9166666666666666	0.9230769230769231	85.0
1.0655737704918034	1.0327868852459017	1.0	63.0
1.2285714285714286	1.1714285714285715	1.2285714285714286	36.0
1.0710059171597632	1.029585798816568	1.0532544378698225	98.0
0.96875	0.96875	0.84375	23.0
1.0339869281045753	1.026143790849673	1.0339869281045753	169.0
0.9487179487179487	1.0341880341880343	0.9829059829059829	42.0
0.8596491228070176	0.8596491228070176	0.8596491228070176	14.0
1.0903954802259888	0.9943502824858758	1.0508474576271187	79.0
0.8461538461538461	0.9076923076923077	1.0769230769230769	49.0
1.048780487804878	1.146341463414634	1.1219512195121952	33.0
1.1666666666666667	0.8333333333333334	0.8333333333333334	13.0
1.0808625336927224	1.0485175202156334	1.091644204851752	109.0
0.8526315789473684	0.9368421052631579	1.0210526315789474	24.0
1.0536193029490617	1.0509383378016086	1.0509383378016086	190.0
1.008714596949891	1.0435729847494553	1.0697167755991286	111.0
1.0476190476190477	1.0272108843537415	1.0816326530612246	144.0
1.1818181818181819	1.121212121212121	1.121212121212121	26.0
0.9322033898305084	0.9491525423728814	0.9830508474576272	58.0
1.0945945945945945	1.0495495495495495	1.0810810810810811	115.0
1.0383631713554988	1.0639386189258313	1.040920716112532	198.0
1.0721153846153846	1.0817307692307692	1.0929487179487178	239.0
1.0864553314121037	1.0403458213256485	1.1037463976945245	87.0
1.0	1.0475319926873858	1.0621572212065813	110.0
1.1793721973094171	1.1793721973094171	1.188340807174888	85.0
1.1078998073217727	1.092485549132948	1.0809248554913296	143.0
1.0517241379310345	1.0775862068965518	1.0646551724137931	134.0
0.9269102990033222	1.0465116279069768	1.0398671096345515	117.0
1.0305188199389623	1.0630722278738556	1.0508646998982707	186.0
1.0659898477157361	1.0786802030456852	1.0964467005076142	156.0
0.9411764705882353	1.0196078431372548	1.0	36.0
1.0642857142857143	1.0535714285714286	1.0571428571428572	140.0
1.075356415478615	1.0835030549898168	1.0936863543788187	233.0
1.081180811808118	1.0910209102091022	1.0934809348093482	161.0
1.125	1.0267857142857142	1.1071428571428572	122.0
1.0086206896551724	1.043103448275862	1.0	57.0
1.0	1.00836820083682	1.0585774058577406	68.0
1.0533333333333332	1.0266666666666666	1.0533333333333332	37.0
1.0779944289693593	1.0501392757660166	1.052924791086351	202.0
1.0	1.0	1.0402684563758389	56.0
0.7142857142857143	0.9047619047619048	0.9047619047619048	8.0
1.077922077922078	1.025974025974026	1.0584415584415585	74.0
1.0774032459425718	1.079900124843945	1.0749063670411985	128.0
1.0759493670886076	1.0042194092827004	1.0337552742616034	118.0
1.0	1.0	1.0	6.0
1.0	1.0	1.0	4.0
1.0446428571428572	1.0178571428571428	1.0625	39.0
1.074294205052006	1.1277860326894502	1.0594353640416048	163.0
1.2222222222222223	1.0	1.0	14.0
1.031413612565445	1.0837696335078535	1.0837696335078535	92.0
0.9473684210526315	0.868421052631579	0.9473684210526315	20.0
1.1217532467532467	1.103896103896104	1.099025974025974	239.0
1.0606796116504855	1.0703883495145632	1.087378640776699	186.0
1.096728307254623	1.0711237553342816	1.0711237553342816	161.0
1.0554272517321017	0.9861431870669746	1.0323325635103926	123.0
0.9512195121951219	1.048780487804878	0.9512195121951219	32.0
1.0740740740740742	1.0740740740740742	1.0	24.0
1.1012658227848102	1.0632911392405062	1.0843881856540085	142.0
1.092378752886836	1.0646651270207852	1.0831408775981524	139.0
0.9393939393939394	1.121212121212121	1.0	22.0
1.0765027322404372	1.0255009107468125	1.116575591985428	124.0
1.0	1.0	1.0	11.0
1.0932277924362357	1.117854001759015	1.116094986807388	245.0
0.7777777777777778	1.0	1.2222222222222223	8.0
1.0382775119617225	1.0318979266347688	1.025518341307815	152.0
1.0288461538461537	1.0769230769230769	1.0288461538461537	60.0
1.064516129032258	1.060215053763441	1.0516129032258064	131.0
1.0761904761904761	1.0761904761904761	1.0698412698412698	108.0
1.033734939759036	1.0530120481927712	1.0530120481927712	216.0
0.9782608695652174	0.9782608695652174	1.0434782608695652	30.0
1.0156657963446476	0.9738903394255874	1.0	103.0
1.085219707057257	1.1091877496671105	1.1198402130492677	186.0
1.074600355239787	1.0781527531083481	1.014209591474245	129.0
1.0245901639344261	1.0327868852459017	1.1147540983606556	85.0
0.9534883720930233	0.9069767441860465	0.9767441860465116	61.0
1.0	0.8333333333333334	1.1666666666666667	18.0
1.0604534005037782	1.0957178841309825	1.105793450881612	130.0
1.0746666666666667	1.04	1.048	171.0
1.1264266900790167	1.1035996488147497	1.1088674275680421	237.0
0.75	0.75	0.75	14.0
1.0941176470588236	1.0549019607843138	1.0705882352941176	99.0
1.065217391304348	1.0043478260869565	1.0347826086956522	135.0
1.0300751879699248	1.0526315789473684	1.0601503759398496	88.0
1.0	0.9586206896551724	1.0689655172413792	47.0
1.0463960231980116	1.0828500414250206	1.096106048053024	244.0
1.0461538461538462	1.0461538461538462	1.1538461538461537	52.0
0.9705882352941176	1.0588235294117647	1.088235294117647	34.0
0.9899497487437185	1.020100502512563	1.0552763819095476	113.0
1.0823970037453183	1.114856429463171	1.0923845193508115	202.0
1.0808080808080809	1.0740740740740742	1.0572390572390573	135.0
1.093278463648834	1.0905349794238683	1.0768175582990398	177.0
1.0668058455114822	1.033402922755741	1.058455114822547	195.0
1.0169491525423728	1.0338983050847457	1.0169491525423728	47.0
1.0	1.0	1.0	12.0
1.0176991150442478	1.0353982300884956	1.0619469026548674	85.0
1.0589604344453065	1.0620636152055858	1.0713731574864236	240.0
1.0534591194968554	1.059748427672956	1.078616352201258	157.0
1.0434332988624613	1.0599793174767322	1.0682523267838677	191.0
1.0	0.8974358974358975	1.0	22.0
1.083752093802345	1.0603015075376885	1.0938023450586265	147.0
1.0495049504950495	1.0693069306930694	1.0891089108910892	116.0
1.0681265206812651	1.0827250608272505	1.0681265206812651	114.0
1.0515463917525774	1.0824742268041236	1.0721649484536082	84.0
1.0045351473922903	1.036281179138322	1.0634920634920635	118.0
1.056701030927835	1.0798969072164948	1.0902061855670102	183.0
1.0483675937122128	1.0483675937122128	1.0918984280532043	151.0
1.0287929125138426	0.9712070874861573	1.0287929125138426	154.0
1.073394495412844	1.0504587155963303	1.055045871559633	105.0
1.040983606557377	1.0081967213114753	1.0245901639344261	51.0
1.0594795539033457	1.037174721189591	1.1115241635687731	82.0
1.0732984293193717	1.0586387434554974	1.0837696335078535	244.0
0.920265780730897	0.9003322259136213	0.9601328903654485	86.0
1.074235807860262	1.0698689956331877	1.1048034934497817	137.0
1.0240963855421688	1.072289156626506	1.0963855421686748	81.0
1.0334928229665072	1.0478468899521531	1.0861244019138756	108.0
1.028892455858748	1.028892455858748	1.0545746388443018	160.0
0.9523809523809523	0.9285714285714286	0.8928571428571429	101.0
0.9735449735449735	1.0476190476190477	1.0423280423280423	97.0
1.0108108108108107	0.9675675675675676	1.054054054054054	65.0
1.0508083140877598	1.0138568129330254	1.069284064665127	130.0
0.9922779922779923	1.0154440154440154	1.0514800514800515	148.0
1.5	1.5	1.5	13.0
1.0310880829015545	1.0829015544041452	1.1243523316062176	53.0
1.0847457627118644	1.0	1.1016949152542372	69.0
1.112	1.064	1.08	39.0
1.0181268882175227	1.0845921450151057	1.0785498489425982	107.0
1.0107816711590296	0.967654986522911	1.0	84.0
1.0873563218390805	1.0689655172413792	1.0827586206896551	113.0
1.0457380457380456	1.0706860706860706	1.054054054054054	229.0
1.0830188679245283	1.0440251572327044	1.060377358490566	200.0
1.012084592145015	1.1027190332326284	1.0845921450151057	91.0
1.0542986425339367	0.9819004524886877	1.009049773755656	63.0
1.0330188679245282	1.070754716981132	1.0660377358490567	163.0
1.0403669724770641	1.055045871559633	1.0440366972477064	120.0
0.9820627802690582	0.9910313901345291	1.0448430493273542	71.0
1.0182232346241458	1.0501138952164009	1.0592255125284737	138.0
1.0723684210526316	1.013157894736842	1.0921052631578947	98.0
1.0495867768595042	1.0	0.9504132231404959	43.0
1.0558659217877095	1.0446927374301676	1.0558659217877095	73.0
0.8666666666666667	0.8666666666666667	0.7333333333333333	22.0
1.0626398210290828	1.0268456375838926	1.0447427293064877	112.0
1.0578947368421052	1.0491228070175438	1.1070175438596492	240.0
1.0452830188679245	0.9547169811320755	1.0226415094339623	73.0
0.973753280839895	0.973753280839895	1.041994750656168	95.0
1.095890410958904	1.1095890410958904	1.095890410958904	73.0
1.1003134796238245	1.0815047021943573	1.0815047021943573	103.0
1.080568720379147	1.0829383886255923	1.0710900473933649	179.0
1.0935875216637783	1.0554592720970537	1.097053726169844	142.0
1.029673590504451	0.9762611275964391	0.9940652818991098	99.0
1.0502793296089385	1.0754189944134078	1.0698324022346368	190.0
1.099502487562189	1.0696517412935322	1.0895522388059702	115.0
1.0759162303664922	1.0471204188481675	1.0418848167539267	176.0
1.0847457627118644	1.0508474576271187	1.0677966101694916	118.0
1.1252900232018561	1.111368909512761	1.111368909512761	133.0
1.0272108843537415	1.0453514739229024	1.0498866213151927	126.0
0.9107142857142857	0.875	0.9821428571428571	45.0
1.0509554140127388	1.1401273885350318	1.178343949044586	53.0
1.0606896551724139	1.0910344827586207	1.0910344827586207	161.0
1.0	1.0	1.0	12.0
1.0659025787965617	1.0687679083094557	1.0945558739255015	115.0
1.0684931506849316	1.0136986301369864	1.0410958904109588	41.0
1.0	1.1149425287356323	1.2988505747126438	59.0
1.0066815144766148	1.0	1.066815144766147	166.0
1.02020202020202	1.02020202020202	1.0606060606060606	39.0
1.1048034934497817	1.1310043668122272	1.1397379912663756	96.0
1.106312292358804	1.0863787375415281	1.159468438538206	79.0
1.0646976090014064	1.1012658227848102	1.1040787623066104	118.0
1.0839363241678726	1.069464544138929	1.0955137481910275	177.0
1.125	1.0	1.125	17.0
1.0858369098712446	1.1158798283261802	1.03862660944206	121.0
1.0299625468164795	1.0674157303370786	1.097378277153558	133.0
1.0126182965299684	1.0315457413249212	1.0063091482649842	93.0
1.0648298217179903	1.106969205834684	1.0907617504051863	149.0
0.8461538461538461	0.8461538461538461	1.0	13.0
1.07503234152652	1.054333764553687	1.07503234152652	170.0
1.0574886535552193	1.075642965204236	1.0968229954614221	165.0
1.0	1.0	1.0	6.0
0.8217270194986073	0.8774373259052924	0.9944289693593314	95.0
1.065040650406504	0.967479674796748	1.065040650406504	48.0
1.0529801324503312	1.1059602649006623	1.0662251655629138	94.0
1.028436018957346	1.066350710900474	1.161137440758294	57.0
1.0284900284900285	1.0626780626780628	1.0940170940170941	159.0
1.0485436893203883	1.087378640776699	1.0776699029126213	62.0
1.049272116461366	1.0627099664053752	1.0940649496080628	221.0
1.0450704225352112	1.056338028169014	1.0619718309859154	112.0
1.0234375	0.9375	1.078125	51.0
0.9428571428571428	0.9510204081632653	1.0489795918367346	64.0
1.1155555555555556	1.0888888888888888	1.08	59.0
1.054468085106383	1.0987234042553191	1.0953191489361702	232.0
1.0489396411092986	1.0619902120717781	1.0783034257748776	149.0
1.0579216354344123	1.0477001703577513	1.0988074957410563	129.0
1.0434782608695652	1.0186335403726707	1.0248447204968945	89.0
1.0827886710239651	1.0326797385620916	1.0697167755991286	104.0
1.0869565217391304	1.0543478260869565	1.0217391304347827	75.0
1.0966921119592876	1.1221374045801527	1.1323155216284988	115.0
1.0954653937947494	1.0859188544152745	1.1193317422434368	133.0
1.0122699386503067	1.030674846625767	1.030674846625767	90.0
1.096732026143791	1.0705882352941176	1.091503267973856	199.0
1.0737893927747886	1.0691775557263643	1.0983858570330516	252.0
1.0712694877505569	1.0623608017817372	1.0979955456570156	141.0
1.0231660231660231	1.1003861003861004	1.0733590733590734	148.0
0.9679144385026738	0.9144385026737968	1.085561497326203	84.0
1.0637254901960784	1.0637254901960784	1.088235294117647	123.0
1.0853658536585367	1.0396341463414633	1.0670731707317074	147.0
1.1025641025641026	1.0256410256410255	1.0769230769230769	62.0
1.0326797385620916	1.0392156862745099	1.0413943355119826	162.0
1.0236686390532543	1.044378698224852	1.029585798816568	171.0
1.0670103092783505	1.0154639175257731	1.0670103092783505	97.0
1.0541871921182266	1.1083743842364533	1.0886699507389161	113.0
1.0783034257748776	1.0783034257748776	1.1272430668841762	141.0
1.063157894736842	1.0894736842105264	1.0763157894736841	168.0
1.0676056338028168	1.1098591549295775	1.123943661971831	130.0
1.1027397260273972	1.11986301369863	1.0856164383561644	127.0
1.0	1.0	1.0	8.0
0.968503937007874	0.84251968503937	0.984251968503937	57.0
0.9289340101522843	0.9390862944162437	0.9695431472081218	40.0
1.059299191374663	1.0431266846361187	1.091644204851752	184.0
1.064102564102564	1.0833333333333333	1.1057692307692308	164.0
1.0375838926174497	1.07248322147651	1.0563758389261746	165.0
0.9470899470899471	0.9365079365079365	1.0	56.0
0.9489795918367347	0.9795918367346939	1.0051020408163265	86.0
1.0978077571669478	1.09106239460371	1.0826306913996628	240.0
1.081145584725537	1.081145584725537	1.107398568019093	109.0
1.1060419235511714	1.088779284833539	1.0789149198520345	215.0
1.0285714285714285	1.0	1.0	25.0
1.064516129032258	1.1935483870967742	1.1935483870967742	25.0
1.0807291666666667	1.0911458333333333	1.1223958333333333	201.0
1.0937223695844385	1.0848806366047745	1.0884173297966402	237.0
1.064516129032258	1.0675883256528418	1.086021505376344	156.0
1.0518444666001994	1.0558325024925224	1.0458624127617149	217.0
1.1688888888888889	1.1333333333333333	1.1688888888888889	91.0
1.0588235294117647	1.0336134453781514	1.0448179271708684	185.0
1.0212201591511936	1.026525198938992	1.0689655172413792	103.0
1.0611724723874256	1.0713678844519967	1.0900594732370434	244.0
1.0795454545454546	1.0643939393939394	1.053030303030303	124.0
1.0	0.7777777777777778	1.0	5.0
1.0103092783505154	1.0240549828178693	1.0721649484536082	142.0
0.7931034482758621	0.8620689655172413	0.7931034482758621	16.0
1.076555023923445	1.0526315789473684	1.0287081339712918	121.0
1.0672413793103448	1.053448275862069	1.0586206896551724	247.0
1.1046511627906976	1.0968992248062015	1.1007751937984496	149.0
1.0	2.0	2.0	12.0
1.0	1.0	1.0	8.0
1.0	0.8974358974358975	1.0769230769230769	47.0
1.0598802395209581	1.095808383233533	1.0934131736526946	176.0
1.0956340956340955	1.137214137214137	1.1496881496881497	149.0
0.8181818181818182	0.9090909090909091	1.0	13.0
1.029325513196481	1.0410557184750733	1.0586510263929618	116.0
0.8235294117647058	0.7058823529411765	0.8823529411764706	14.0
1.0686695278969958	0.9957081545064378	1.0257510729613735	127.0
0.8947368421052632	1.0526315789473684	1.0	19.0
1.0901639344262295	1.069672131147541	1.0778688524590163	127.0
0.8857142857142857	0.8857142857142857	1.0285714285714285	22.0
0.9475218658892128	1.0233236151603498	1.0699708454810495	80.0
1.0589569160997732	1.1043083900226758	1.072562358276644	119.0
1.0203045685279188	0.9796954314720813	1.0101522842639594	54.0
1.0510774142059058	1.0622505985634478	1.0766161213088588	231.0
1.070921985815603	1.0212765957446808	1.0638297872340425	65.0
1.0472813238770686	1.0189125295508275	1.1040189125295508	110.0
1.1041214750542299	1.1127982646420824	1.1084598698481563	135.0
1.0628930817610063	1.029350104821803	1.0587002096436058	125.0
1.0	0.7777777777777778	0.7777777777777778	16.0
1.103161397670549	1.1064891846921796	1.1430948419301166	165.0
1.0754716981132075	1.0943396226415094	1.0849056603773586	111.0
1.0126984126984127	1.1015873015873017	1.0444444444444445	94.0
1.0844720496894409	1.0944099378881988	1.0795031055900621	164.0
0.9333333333333333	0.8666666666666667	0.8333333333333334	25.0
1.0232558139534884	1.0	0.9767441860465116	34.0
1.0680272108843538	1.0408163265306123	1.0714285714285714	139.0
1.0684596577017116	1.078239608801956	1.0537897310513447	132.0
0.9354838709677419	0.9596774193548387	1.0161290322580645	67.0
0.8666666666666667	1.0	0.8666666666666667	19.0
1.0	1.0	1.0	9.0
1.0323383084577114	1.0472636815920398	1.072139303482587	200.0
1.0549828178694158	0.993127147766323	1.006872852233677	89.0
1.0	1.03690036900369	1.044280442804428	97.0
1.0912052117263844	1.0846905537459284	1.1140065146579805	191.0
1.0317460317460319	1.0952380952380953	1.126984126984127	53.0
1.0555555555555556	1.0222222222222221	0.9777777777777777	53.0
0.9856115107913669	0.9856115107913669	0.9424460431654677	36.0
1.0	1.0	1.0	7.0
1.0631163708086786	1.0433925049309665	1.0986193293885602	121.0
1.037122969837587	1.0464037122969838	1.0696055684454757	131.0
1.0651629072681705	1.0701754385964912	1.055137844611529	107.0
1.0796019900497513	1.0696517412935322	1.1592039800995024	63.0
1.0792079207920793	1.099009900990099	1.1287128712871286	123.0
1.0518962075848304	1.0439121756487026	1.0638722554890219	107.0
1.0498220640569396	1.0640569395017794	1.0711743772241993	157.0
1.046204620462046	0.9801980198019802	1.0	90.0
1.0512820512820513	1.044871794871795	1.064102564102564	103.0
1.0303030303030303	0.9913419913419913	1.0606060606060606	122.0
1.0845070422535212	0.9436619718309859	0.9859154929577465	48.0
1.0704225352112675	1.0788732394366196	1.0901408450704226	162.0
1.0890052356020943	1.1151832460732984	1.12565445026178	118.0
1.0662983425414365	1.0441988950276244	1.0607734806629834	88.0
1.0727762803234502	1.0619946091644206	1.064690026954178	171.0
1.0907504363001745	1.087260034904014	1.087260034904014	117.0
1.0597014925373134	1.0298507462686568	1.0597014925373134	38.0
1.07035175879397	1.0804020100502512	1.100502512562814	70.0
1.0765027322404372	1.0819672131147542	1.0792349726775956	159.0
1.1666666666666667	1.0555555555555556	1.1111111111111112	29.0
1.1643835616438356	1.1369863013698631	1.1095890410958904	34.0
1.1311475409836065	1.1311475409836065	1.0655737704918034	43.0
1.16	1.24	1.24	19.0
1.078740157480315	1.078740157480315	1.073490813648294	121.0
1.0913811007268952	1.078920041536864	1.1017653167185877	226.0
1.0494505494505495	1.0494505494505495	1.065934065934066	99.0
1.031390134529148	1.053811659192825	1.0179372197309418	112.0
1.1016597510373445	1.0829875518672198	1.070539419087137	220.0
1.1296296296296295	0.9814814814814815	1.0555555555555556	43.0
1.082191780821918	1.086105675146771	1.1056751467710373	148.0
1.0682226211849193	1.082585278276481	1.1077199281867145	130.0
1.0763358778625953	1.16793893129771	1.1221374045801527	49.0
1.0763983628922238	1.1009549795361528	1.0900409276944065	119.0
0.9166666666666666	1.0	0.9166666666666666	36.0
1.0119047619047619	1.0476190476190477	1.0476190476190477	64.0
1.1045130641330165	1.0688836104513064	1.0878859857482186	175.0
0.926605504587156	1.036697247706422	1.110091743119266	49.0
1.0795847750865053	1.0484429065743945	1.0726643598615917	145.0
0.9466666666666667	0.9466666666666667	0.92	22.0
1.2222222222222223	1.4444444444444444	1.4444444444444444	14.0
1.0092165898617511	1.055299539170507	1.055299539170507	53.0
2.0	2.0	2.0	5.0
1.0767386091127098	1.0767386091127098	1.1247002398081534	110.0
1.0825958702064897	1.0176991150442478	1.1002949852507375	105.0
1.040983606557377	1.0737704918032787	1.0573770491803278	192.0
1.0485436893203883	1.0776699029126213	1.0	66.0
0.9041095890410958	0.9726027397260274	1.0136986301369864	49.0
1.0601092896174864	1.0874316939890711	1.1120218579234973	170.0
1.0165289256198347	1.0330578512396693	1.0495867768595042	57.0
0.972972972972973	1.0216216216216216	1.0216216216216216	94.0
1.0716417910447762	0.982089552238806	1.035820895522388	94.0
1.0954979536152796	1.08731241473397	1.08731241473397	169.0
0.8518518518518519	0.8518518518518519	1.0	22.0
1.0878048780487806	1.0902439024390245	1.1097560975609757	203.0
0.9711191335740073	0.9566787003610109	1.0216606498194947	90.0
0.8620689655172413	0.7241379310344828	0.9310344827586207	22.0
1.0846994535519126	1.0573770491803278	1.0956284153005464	176.0
1.1209068010075567	1.0755667506297228	1.0906801007556675	120.0
1.0940438871473355	1.1065830721003134	1.0564263322884013	116.0
1.0714285714285714	1.042857142857143	1.0714285714285714	63.0
1.1101449275362318	1.0811594202898551	1.0840579710144929	182.0
1.062111801242236	1.124223602484472	1.0745341614906831	50.0
1.0666666666666667	1.0512820512820513	1.035897435897436	119.0
1.1024258760107817	1.05570530098832	1.0880503144654088	241.0
1.0953253895508708	1.0549954170485794	1.082493125572869	206.0
1.070628768303187	1.0275624461670974	1.053402239448751	220.0
1.0509554140127388	1.0764331210191083	0.9872611464968153	56.0
1.0567741935483872	1.0619354838709678	1.064516129032258	126.0
1.058968058968059	1.0884520884520885	1.0884520884520885	119.0
1.1081081081081081	1.117117117117117	1.135135135135135	75.0
1.0032894736842106	1.0460526315789473	1.0263157894736843	153.0
1.0681003584229392	1.028673835125448	1.060931899641577	140.0
1.0659898477157361	1.0609137055837563	1.0659898477157361	112.0
1.0893470790378006	1.0807560137457044	1.0721649484536082	244.0
1.0353513035793196	1.0388864339372514	1.0494918250110472	356.0
1.125	1.1041666666666667	1.0625	42.0
0.9565217391304348	1.0724637681159421	1.1304347826086956	47.0
1.073959938366718	1.0523882896764252	1.0431432973805854	150.0
1.2307692307692308	1.1538461538461537	1.2307692307692308	31.0
1.075993091537133	1.069084628670121	1.075993091537133	140.0
0.9470899470899471	0.9576719576719577	0.9576719576719577	51.0
1.0714285714285714	1.1428571428571428	0.8571428571428571	12.0
1.0621761658031088	1.072538860103627	1.0414507772020725	48.0
1.068212824010914	1.08731241473397	1.0763983628922238	191.0
1.065040650406504	0.967479674796748	1.0	39.0
1.0	1.0	1.0	5.0
1.0485436893203883	1.0776699029126213	1.0614886731391586	141.0
1.0793103448275863	1.0827586206896551	1.0758620689655172	249.0
0.9426229508196722	0.9098360655737705	0.9590163934426229	37.0
0.9454545454545454	0.9272727272727272	1.0545454545454545	34.0
1.2857142857142858	1.2857142857142858	1.0	15.0
1.0652818991097923	1.0356083086053411	1.0356083086053411	90.0
1.0639658848614073	0.9957356076759062	1.0767590618336886	120.0
1.0437158469945356	1.018214936247723	1.0801457194899817	117.0
1.050420168067227	1.0336134453781514	0.9831932773109243	40.0
1.0108695652173914	1.0217391304347827	1.0869565217391304	65.0
1.0512820512820513	1.0512820512820513	1.0647773279352226	167.0
1.117252931323283	1.0904522613065326	1.050251256281407	155.0
1.0798226164079823	1.0931263858093125	1.0620842572062084	128.0
1.0660247592847318	1.0825309491059147	1.096286107290234	171.0
1.0878048780487806	1.1219512195121952	1.0878048780487806	108.0
1.14	1.09	1.12	76.0
1.0	1.0	1.0	6.0
1.0899074482150728	1.0899074482150728	1.0749228735125607	357.0
0.8181818181818182	0.6363636363636364	0.6363636363636364	18.0
1.0688259109311742	1.0	1.0526315789473684	109.0
1.0482897384305836	1.028169014084507	1.06841046277666	116.0
1.0038240917782026	0.9847036328871893	0.9961759082217974	137.0
0.9710843373493976	0.9228915662650602	1.0240963855421688	100.0
1.065040650406504	1.0731707317073171	1.056910569105691	166.0
1.0264900662251655	1.0662251655629138	1.0529801324503312	86.0
0.8695652173913043	0.9565217391304348	0.9130434782608695	27.0
1.0706521739130435	1.0733695652173914	1.078804347826087	116.0
1.0589225589225588	1.0606060606060606	1.0824915824915824	229.0
1.0704225352112675	1.0774647887323943	1.091549295774648	113.0
1.092485549132948	1.0809248554913296	1.0346820809248556	48.0
1.0244648318042813	1.0489296636085628	1.0795107033639144	82.0
1.0338983050847457	1.0677966101694916	1.0593220338983051	87.0
1.08	1.0	1.08	20.0
1.05668016194332	1.0539811066126856	1.0944669365721997	129.0
0.8285714285714286	0.8857142857142857	1.0	31.0
0.9743589743589743	0.9743589743589743	0.9487179487179487	65.0
1.0716253443526171	1.1019283746556474	1.1101928374655647	190.0
1.053853296193129	1.0817084493964717	1.0761374187558033	203.0
1.0612244897959184	1.0442176870748299	1.0442176870748299	140.0
1.062780269058296	1.0089686098654709	1.0807174887892377	84.0
1.055045871559633	1.0305810397553516	1.0672782874617737	80.0
1.0049627791563276	1.0794044665012408	1.0595533498759304	104.0
1.066147859922179	1.1089494163424125	1.0972762645914398	108.0
0.926829268292683	0.926829268292683	0.975609756097561	49.0
1.18	1.0	1.26	40.0
1.059748427672956	1.0943396226415094	1.069182389937107	148.0
0.9310344827586207	0.9310344827586207	1.0689655172413792	22.0
1.0499168053244592	1.0665557404326123	1.0732113144758735	144.0
1.036231884057971	1.0507246376811594	1.0289855072463767	71.0
0.9697885196374623	0.9274924471299094	1.0181268882175227	97.0
1.0776699029126213	1.058252427184466	1.0922330097087378	106.0
1.0398009950248757	1.0348258706467661	1.0845771144278606	115.0
1.0743494423791822	1.0475836431226766	1.0698884758364313	247.0
1.072538860103627	1.0518134715025906	1.0414507772020725	70.0
1.0	0.9627329192546584	0.9751552795031055	80.0
1.0	0.8571428571428571	0.8571428571428571	27.0
1.0104712041884816	1.0418848167539267	1.0	41.0
1.079646017699115	1.0353982300884956	1.0442477876106195	88.0
0.7142857142857143	1.0	1.0	9.0
1.079295154185022	1.1027900146842877	1.091042584434655	147.0
1.0340425531914894	1.025531914893617	1.102127659574468	91.0
1.0744777475022707	1.056312443233424	1.0835603996366938	204.0
1.0636363636363637	1.0545454545454545	1.0272727272727273	50.0
1.0666666666666667	1.0256410256410255	1.0	90.0
1.1333333333333333	1.2666666666666666	1.0	18.0
1.078918918918919	1.0810810810810811	1.094054054054054	320.0
1.0575427682737168	1.0653188180404354	1.0668740279937792	241.0
1.038910505836576	1.0739299610894941	1.0428015564202335	132.0
1.0209424083769634	1.0523560209424083	1.1570680628272252	77.0
0.9682539682539683	1.0158730158730158	0.9841269841269841	45.0
1.08	1.16	1.18	60.0
0.9304347826086956	1.017391304347826	1.017391304347826	30.0
1.124	1.108	1.148	150.0
1.0390243902439025	1.0390243902439025	1.0390243902439025	61.0
0.9787234042553191	0.9574468085106383	0.8936170212765957	26.0
1.0564826700898589	1.0641848523748396	1.0385109114249038	167.0
1.065155807365439	1.0991501416430596	1.0991501416430596	121.0
1.05668016194332	1.0728744939271255	1.0931174089068827	224.0
1.2	1.1655172413793105	1.1448275862068966	83.0
0.949748743718593	1.0402010050251256	1.0100502512562815	104.0
1.0	0.6666666666666666	1.0	6.0
1.0561797752808988	1.0730337078651686	1.095505617977528	162.0
1.0724233983286908	1.0278551532033426	1.0501392757660166	103.0
0.978021978021978	0.7802197802197802	1.021978021978022	30.0
1.0288184438040346	0.9798270893371758	1.0259365994236311	131.0
1.0627450980392157	1.0901960784313725	1.0941176470588236	139.0
1.0610997963340123	1.089613034623218	1.0957230142566192	242.0
1.1	1.1	1.0	33.0
0.9444444444444444	0.9444444444444444	0.9444444444444444	78.0
1.0583016476552598	1.0278833967046894	1.0785804816223068	155.0
1.1074964639321074	1.0905233380480905	1.115983026874116	205.0
1.0513761467889908	1.0220183486238532	1.0660550458715596	130.0
1.016260162601626	1.0	1.08130081300813	58.0
1.0672897196261681	1.0785046728971963	1.0934579439252337	118.0
1.0422535211267605	1.056338028169014	1.0845070422535212	54.0
1.0307328605200945	1.0543735224586288	1.0685579196217494	204.0
1.0393700787401574	0.937007874015748	1.0708661417322836	76.0
1.111368909512761	1.0928074245939676	1.1160092807424593	106.0
1.0493150684931507	1.093150684931507	1.082191780821918	101.0
1.0393700787401574	1.015748031496063	1.047244094488189	66.0
1.0	1.047945205479452	1.0616438356164384	74.0
1.1080196399345335	1.1374795417348609	1.1309328968903436	190.0
1.0	1.0	1.0909090909090908	22.0
1.0667779632721202	1.0884808013355594	1.0784641068447411	241.0
1.0326086956521738	1.065217391304348	1.0579710144927537	126.0
1.022514071294559	1.0600375234521575	1.0675422138836772	104.0
1.0380952380952382	1.019047619047619	1.0166666666666666	150.0
1.0404040404040404	1.0252525252525253	1.1414141414141414	109.0
1.054421768707483	0.9319727891156463	1.0408163265306123	38.0
1.1904761904761905	1.0952380952380953	1.1904761904761905	24.0
1.0622641509433963	1.0867924528301887	1.0547169811320756	220.0
1.050467289719626	1.0392523364485982	1.0579439252336449	195.0
0.0	0.0	0.0	9.0
1.0048192771084337	0.9855421686746988	1.0289156626506024	98.0
0.9658119658119658	0.9829059829059829	1.0854700854700854	67.0
1.098846787479407	1.0691927512355848	1.0906095551894563	229.0
1.0545454545454545	1.0472727272727274	1.0472727272727274	157.0
0.9076923076923077	0.8953846153846153	0.9692307692307692	82.0
1.01	1.06	1.06	95.0
0.948051948051948	1.0	1.0	28.0
0.9827586206896551	0.9827586206896551	0.9655172413793104	35.0
1.1227197346600333	1.1293532338308458	1.142620232172471	150.0
1.069767441860465	1.0348837209302326	1.069767441860465	51.0
1.0479302832244008	1.056644880174292	1.0740740740740742	124.0
1.0449438202247192	1.0449438202247192	1.0449438202247192	53.0
1.0	1.0277777777777777	1.0833333333333333	43.0
0.9649122807017544	1.0175438596491229	1.105263157894737	42.0
1.0415430267062316	1.0949554896142433	1.1186943620178043	90.0
1.0943643512450851	1.0707732634338138	1.0838794233289646	170.0
1.1477045908183632	1.0998003992015968	1.127744510978044	110.0
1.0869565217391304	1.0562659846547315	1.1074168797953965	93.0
1.0671834625322998	1.062015503875969	1.0516795865633075	108.0
1.0025284450063212	1.0632111251580278	1.0632111251580278	194.0
1.0	1.0	1.0	9.0
0.7857142857142857	0.8571428571428571	0.7857142857142857	15.0
1.080701754385965	1.0736842105263158	1.0982456140350878	244.0
0.9869706840390879	1.0390879478827362	1.0749185667752443	120.0
1.0684931506849316	1.1232876712328768	1.1369863013698631	140.0
1.1062176165803108	1.0829015544041452	1.1010362694300517	172.0
1.0952380952380953	1.0714285714285714	1.0793650793650793	80.0
1.0946745562130178	1.106508875739645	1.047337278106509	67.0
1.1538461538461537	1.1538461538461537	1.1538461538461537	16.0
1.0299251870324189	1.0149625935162094	1.0448877805486285	117.0
1.087962962962963	1.0787037037037037	1.1157407407407407	128.0
0.9663865546218487	1.0336134453781514	1.0168067226890756	58.0
1.0952380952380953	1.0595238095238095	1.119047619047619	52.0
0.9948453608247423	1.0515463917525774	1.0721649484536082	96.0
1.0721649484536082	0.9896907216494846	1.1030927835051547	84.0
0.8814814814814815	0.9259259259259259	1.0148148148148148	49.0
1.0481622306717364	1.0760456273764258	1.0659062103929025	173.0
1.0136674259681093	1.0136674259681093	1.0592255125284737	113.0
1.0	1.0740740740740742	1.0185185185185186	42.0
1.0	1.0	1.0	13.0
1.098550724637681	1.0869565217391304	1.1130434782608696	179.0
0.9775280898876404	0.9550561797752809	1.0	28.0
1.0	1.0	1.0	10.0
1.0518731988472623	1.0518731988472623	1.0979827089337175	110.0
0.9555555555555556	0.9888888888888889	0.9777777777777777	35.0
1.0	1.0	1.0	7.0
1.0161290322580645	1.032258064516129	1.0483870967741935	51.0
1.1212976022566996	1.1128349788434415	1.0959097320169253	167.0
1.0473118279569893	1.038709677419355	1.064516129032258	120.0
1.023407022106632	1.0312093628088426	1.0494148244473342	187.0
1.0690376569037656	1.0753138075313808	1.0439330543933054	213.0
1.0	1.0	1.0	10.0
1.098415346121768	1.0950792326939116	1.085070892410342	236.0
0.927710843373494	0.9036144578313253	1.0120481927710843	68.0
1.0	1.0	1.0	1.0
1.0818291215403129	1.0794223826714802	1.1010830324909748	134.0
1.0613026819923372	1.049808429118774	1.0613026819923372	121.0
1.146341463414634	1.056910569105691	1.032520325203252	87.0
1.0646651270207852	1.1062355658198615	1.0831408775981524	132.0
1.0394088669950738	1.0492610837438423	1.0738916256157636	101.0
0.9857142857142858	0.9285714285714286	1.042857142857143	64.0
0.922879177377892	0.9640102827763496	0.9897172236503856	100.0
1.1	1.1205882352941177	1.1029411764705883	162.0
1.057052297939778	1.057052297939778	1.0729001584786053	169.0
0.9337349397590361	1.0	0.9819277108433735	88.0
0.9176470588235294	0.9764705882352941	0.9411764705882353	63.0
1.0225352112676056	1.0225352112676056	1.028169014084507	93.0
1.0588832487309645	1.0406091370558375	1.0934010152284264	230.0
1.0570264765784114	1.0692464358452138	1.0081466395112015	126.0
1.098901098901099	1.0714285714285714	1.0384615384615385	93.0
1.0376175548589341	1.0376175548589341	1.0188087774294672	151.0
1.0463847203274215	1.0463847203274215	1.0763983628922238	153.0
1.056470588235294	1.0376470588235294	1.0658823529411765	134.0
1.066334991708126	1.0530679933665008	1.0928689883913765	121.0
1.108	1.116	1.14	146.0
1.0819584885577436	1.0734433209153804	1.0819584885577436	320.0
0.9867695700110254	1.0044101433296582	1.0418963616317531	156.0
1.0	0.7777777777777778	0.7777777777777778	13.0
1.0611961057023644	1.0445062586926286	1.0500695410292071	183.0
1.0683937823834198	1.0746113989637305	1.0911917098445596	243.0
1.0796324655436447	1.0520673813169985	1.0735068912710566	151.0
1.105726872246696	1.0969162995594715	1.0881057268722467	128.0
1.0310077519379846	1.0310077519379846	1.124031007751938	51.0
1.0755048287971904	1.0825285338015804	1.061457418788411	240.0
0.9393939393939394	1.0	0.8787878787878788	24.0
1.1403508771929824	1.1637426900584795	1.128654970760234	92.0
1.0561797752808988	1.0224719101123596	1.0337078651685394	46.0
1.1007751937984496	1.0568475452196382	1.0723514211886305	170.0
1.0246913580246915	1.0246913580246915	1.0740740740740742	47.0
1.0695915279878971	1.0695915279878971	1.0847201210287443	156.0
0.9477124183006536	0.9869281045751634	1.0392156862745099	50.0
1.064343163538874	1.0804289544235925	1.1018766756032172	111.0
1.025995125913891	1.0471161657189276	1.0536149471974006	203.0
1.0784313725490196	1.0991926182237601	1.0968858131487889	172.0
1.1169811320754717	1.1018867924528302	1.0679245283018868	144.0
1.1403508771929824	1.0701754385964912	1.0116959064327486	64.0
1.095959595959596	1.1515151515151516	1.1414141414141414	99.0
1.059090909090909	1.0727272727272728	1.0636363636363637	113.0
1.04221635883905	0.9894459102902374	1.0158311345646438	96.0
1.085427135678392	1.1155778894472361	1.1105527638190955	127.0
1.0526315789473684	0.9298245614035088	1.1228070175438596	39.0
1.0583554376657824	1.0689655172413792	1.026525198938992	90.0
0.9650145772594753	0.9737609329446064	1.0524781341107872	103.0
1.0271739130434783	1.0869565217391304	1.065217391304348	91.0
1.0544747081712063	1.038910505836576	1.0505836575875487	150.0
1.0628930817610063	1.0251572327044025	1.0628930817610063	58.0
1.0981912144702843	1.0775193798449612	1.103359173126615	108.0
1.037313432835821	1.0335820895522387	1.0522388059701493	147.0
1.0244399185336048	1.0529531568228105	1.0773930753564154	114.0
1.0632411067193677	1.051383399209486	1.023715415019763	115.0
1.0	1.0345821325648414	0.9942363112391931	101.0
0.8333333333333334	0.8333333333333334	0.8333333333333334	11.0
1.059900166389351	1.0665557404326123	1.0632279534109816	114.0
1.1014492753623188	1.0	1.0289855072463767	59.0
1.0746268656716418	1.0	1.1044776119402986	47.0
1.0829694323144106	1.074235807860262	1.0655021834061136	113.0
0.825	0.875	0.875	21.0
1.0851063829787233	1.0212765957446808	1.0638297872340425	47.0
1.1305361305361306	1.0885780885780887	1.1258741258741258	131.0
1.122093023255814	1.12015503875969	1.12015503875969	210.0
1.0395256916996047	0.9920948616600791	1.0039525691699605	135.0
1.0372093023255815	1.0651162790697675	1.0465116279069768	62.0
1.0760233918128654	1.04093567251462	1.0292397660818713	83.0
1.0884955752212389	1.0176991150442478	1.0707964601769913	61.0
1.0700152207001523	1.0669710806697108	1.0365296803652968	165.0
1.0899742930591259	1.1028277634961439	1.1182519280205656	140.0
0.972972972972973	1.009009009009009	1.0360360360360361	48.0
0.9665271966527197	0.9832635983263598	1.0209205020920502	109.0
1.0450281425891181	1.0600375234521575	1.0975609756097562	160.0
0.875	1.0	0.8125	30.0
1.0760456273764258	1.1064638783269962	1.0456273764258555	88.0
1.0175438596491229	1.0701754385964912	1.0263157894736843	89.0
1.0	1.0	1.0	13.0
1.0418410041841004	1.0460251046025104	1.0627615062761506	133.0
0.9285714285714286	1.0714285714285714	1.0	23.0
1.061744966442953	1.018791946308725	1.0966442953020135	164.0
0.8983050847457628	0.7627118644067796	0.8983050847457628	36.0
1.035190615835777	1.035190615835777	1.0879765395894427	80.0
1.0098039215686274	1.0294117647058822	1.0686274509803921	119.0
1.039344262295082	1.062295081967213	1.0688524590163935	152.0
0.75	0.75	0.75	8.0
1.103359173126615	1.0852713178294573	1.0904392764857882	123.0
0.8181818181818182	0.8181818181818182	0.8181818181818182	13.0
0.9669421487603306	0.8842975206611571	0.9669421487603306	46.0
1.0337837837837838	1.0675675675675675	1.0405405405405406	82.0
1.091703056768559	1.0873362445414847	1.0873362445414847	127.0
1.0359897172236503	1.025706940874036	1.0668380462724936	93.0
1.0610169491525423	1.0745762711864406	1.0768361581920904	167.0
0.9973614775725593	1.0263852242744063	1.0395778364116095	189.0
0.9603960396039604	1.0792079207920793	1.0396039603960396	26.0
1.05	1.0642857142857143	1.1071428571428572	84.0
1.113821138211382	1.0596205962059622	1.0921409214092141	93.0
1.0854700854700854	1.1196581196581197	1.2393162393162394	47.0
1.096774193548387	1.10752688172043	1.043010752688172	39.0
1.108910891089109	1.0627062706270627	1.0825082508250825	164.0
0.8823529411764706	1.0	1.0470588235294118	26.0
0.7272727272727273	0.6818181818181818	0.7272727272727273	18.0
0.9866666666666667	0.96	1.0266666666666666	54.0
1.018018018018018	1.006006006006006	1.0	79.0
1.0579710144927537	1.0	1.0811594202898551	104.0
1.0803212851405624	1.0562248995983936	1.0856760374832664	171.0
1.0921787709497206	1.106145251396648	1.111731843575419	129.0
1.093697713329615	1.093697713329615	1.0970440602342444	309.0
0.7142857142857143	0.7142857142857143	0.7142857142857143	4.0
1.096551724137931	1.1011494252873564	1.1011494252873564	131.0
0.9551282051282052	0.967948717948718	1.0256410256410255	96.0
1.091549295774648	1.0651408450704225	1.1003521126760563	244.0
1.0695652173913044	1.0289855072463767	1.0956521739130434	163.0
1.0833333333333333	0.9166666666666666	0.8333333333333334	25.0
1.091533180778032	1.0251716247139588	1.0526315789473684	165.0
1.047887323943662	1.0535211267605633	1.0929577464788733	161.0
1.0399002493765586	1.0299251870324189	1.084788029925187	103.0
1.068062827225131	1.0994764397905759	1.0890052356020943	113.0
1.0178571428571428	1.0714285714285714	1.0535714285714286	57.0
1.0440165061898212	1.0577716643741404	1.0577716643741404	174.0
1.0904347826086958	1.097391304347826	1.0695652173913044	143.0
1.0657142857142856	1.0914285714285714	1.12	164.0
1.0869565217391304	0.9130434782608695	1.2608695652173914	25.0
1.0858585858585859	1.0808080808080809	1.101010101010101	130.0
1.0794701986754967	1.0397350993377483	1.0728476821192052	79.0
0.958656330749354	1.0310077519379846	1.0516795865633075	109.0
1.0215285252960171	1.038751345532831	1.0430570505920345	163.0
1.1439114391143912	1.1586715867158672	1.136531365313653	113.0
1.125	1.08	1.12	213.0
1.0893300248138957	1.0769230769230769	1.0843672456575681	176.0
1.0	1.0	1.0	6.0
0.6666666666666666	0.6666666666666666	0.6666666666666666	2.0
0.6428571428571429	0.5714285714285714	0.7857142857142857	20.0
1.0907975460122699	1.0907975460122699	1.0760736196319018	195.0
1.064367816091954	1.07816091954023	1.0551724137931036	133.0
0.9897435897435898	1.0068376068376068	1.0205128205128204	139.0
1.0648148148148149	1.1111111111111112	1.125	102.0
1.1245059288537549	1.1146245059288538	1.1185770750988142	230.0
1.0537897310513447	1.019559902200489	1.0342298288508558	87.0
1.0	1.0	1.0	20.0
1.0235294117647058	1.0470588235294118	1.0	59.0
1.1196581196581197	1.1324786324786325	1.0897435897435896	151.0
1.0211267605633803	1.0105633802816902	1.0422535211267605	136.0
0.9859154929577465	1.028169014084507	1.028169014084507	37.0
1.1074074074074074	1.0851851851851853	1.1	129.0
1.0625	1.015625	1.03125	58.0
1.1081967213114754	1.0754098360655737	1.0950819672131147	145.0
1.0909990108803165	1.0850642927794263	1.0949554896142433	220.0
0.9905882352941177	1.0235294117647058	1.0282352941176471	108.0
0.8774193548387097	0.9161290322580645	0.9290322580645162	89.0
1.0271317829457365	1.0465116279069768	1.0891472868217054	111.0
0.5	0.5	0.5	5.0
1.0683229813664596	1.093167701863354	1.0745341614906831	102.0
0.9878048780487805	0.9512195121951219	0.9634146341463414	78.0
1.0598802395209581	1.0658682634730539	1.0658682634730539	108.0
0.9885714285714285	1.0114285714285713	1.0685714285714285	61.0
1.0871212121212122	1.0757575757575757	1.1136363636363635	153.0
1.0721311475409836	1.0327868852459017	1.0459016393442624	86.0
1.0898502495840265	1.0465890183028286	1.0831946755407653	186.0
0.9240506329113924	0.6962025316455697	0.9240506329113924	28.0
1.0	0.9620253164556962	1.1012658227848102	46.0
1.104109589041096	1.0657534246575342	1.0602739726027397	112.0
1.0785597381342062	1.0851063829787233	1.0949263502454991	188.0
0.9313984168865436	0.9313984168865436	0.978891820580475	90.0
1.0676923076923077	1.0676923076923077	1.0369230769230768	96.0
1.0275862068965518	1.0	1.0459770114942528	164.0
1.0873180873180872	1.0706860706860706	1.079002079002079	118.0
1.0962566844919786	1.053475935828877	1.085561497326203	92.0
1.068522483940043	1.0728051391862956	1.0899357601713062	145.0
1.0792079207920793	1.0198019801980198	1.00990099009901	97.0
0.8536585365853658	0.9512195121951219	0.9024390243902439	34.0
1.016025641025641	1.0416666666666667	1.0480769230769231	113.0
1.0776699029126213	1.087378640776699	1.0776699029126213	71.0
1.0588235294117647	1.0526315789473684	1.108359133126935	168.0
1.0364963503649636	0.9890510948905109	1.0291970802919708	159.0
1.0497335701598578	1.0603907637655416	1.074600355239787	159.0
1.0940499040307101	1.053742802303263	1.09021113243762	201.0
1.0609523809523809	1.0304761904761905	1.1028571428571428	111.0
1.0833333333333333	1.1666666666666667	1.0833333333333333	39.0
1.0513698630136987	1.0308219178082192	1.095890410958904	137.0
0.8918918918918919	0.8378378378378378	1.0	17.0
1.0842433697347893	1.0686427457098284	1.1185647425897036	172.0
1.0769971126082771	1.0481231953801733	1.0731472569778633	196.0
1.0	1.0	1.0	5.0
0.8571428571428571	1.0	1.0	19.0
1.0813464235624124	1.0785413744740533	1.1122019635343618	160.0
1.0859845227858986	1.0825451418744625	1.1014617368873603	239.0
0.84	0.68	0.52	18.0
0.9487179487179487	1.1794871794871795	1.2307692307692308	37.0
1.0	1.0	1.064516129032258	22.0
1.0566037735849056	0.9433962264150944	0.9811320754716981	30.0
1.0646976090014064	1.0506329113924051	1.0843881856540085	188.0
1.0632911392405062	1.0928270042194093	1.1139240506329113	140.0
0.8620689655172413	1.0	0.9310344827586207	21.0
1.075268817204301	1.053763440860215	1.096774193548387	126.0
1.0	1.0	1.105263157894737	25.0
1.0674955595026643	1.0461811722912966	1.074600355239787	160.0
1.0	1.0	1.125	20.0
1.048780487804878	1.0260162601626017	1.0520325203252032	130.0
1.0530973451327434	1.0943952802359882	1.1415929203539823	91.0
0.9940652818991098	0.9821958456973294	0.9881305637982196	110.0
1.0454545454545454	1.0681818181818181	1.0643939393939394	124.0
1.0748129675810474	1.0798004987531171	1.0997506234413965	123.0
0.8608695652173913	0.9304347826086956	0.9652173913043478	22.0
1.107981220657277	1.0938967136150235	1.0985915492957747	128.0
0.9836734693877551	0.9918367346938776	1.0326530612244897	60.0
1.0	1.0	1.0	5.0
1.0588235294117647	1.088235294117647	1.1176470588235294	50.0
0.9576719576719577	0.9947089947089947	0.8994708994708994	86.0
1.0165289256198347	0.9834710743801653	0.9669421487603306	86.0
0.9908675799086758	1.0091324200913243	1.0365296803652968	64.0
1.1056338028169015	1.0422535211267605	1.091549295774648	68.0
0.9215686274509803	1.0	1.0196078431372548	35.0
0.9794344473007712	0.9280205655526992	0.9897172236503856	102.0
1.0444444444444445	1.0074074074074073	1.0814814814814815	91.0
1.0952380952380953	1.2380952380952381	1.1428571428571428	37.0
1.013986013986014	1.013986013986014	1.0	36.0
1.0341463414634147	1.053658536585366	1.0585365853658537	112.0
1.115267947421638	1.115267947421638	1.1011122345803843	199.0
0.9444444444444444	0.8611111111111112	0.9722222222222222	29.0
1.0670731707317074	1.076219512195122	1.0945121951219512	174.0
1.09009009009009	1.1036036036036037	1.0855855855855856	125.0
0.9703703703703703	1.0296296296296297	1.0	67.0
1.0392156862745099	1.0336134453781514	1.0392156862745099	110.0
0.8095238095238095	0.9047619047619048	0.9047619047619048	34.0
1.1031307550644567	1.1141804788213627	1.1141804788213627	142.0
1.0666666666666667	1.08	1.0711111111111111	141.0
0.9495798319327731	0.9943977591036415	1.0392156862745099	88.0
1.074600355239787	1.0603907637655416	1.0213143872113677	105.0
1.060931899641577	1.043010752688172	1.086021505376344	125.0
1.041871921182266	1.0566502463054188	1.0738916256157636	161.0
1.0947368421052632	1.1228070175438596	1.1228070175438596	136.0
1.0	1.0	1.6666666666666667	11.0
1.078048780487805	1.0195121951219512	1.0292682926829269	86.0
1.0583190394511148	1.0308747855917668	1.0686106346483706	135.0
1.0564516129032258	1.0806451612903225	1.1209677419354838	90.0
1.0776978417266188	1.0661870503597122	1.1179856115107913	169.0
1.0086206896551724	1.1120689655172413	1.2241379310344827	64.0
1.0714285714285714	1.1020408163265305	1.1428571428571428	76.0
1.0	1.0	1.0	9.0
1.0	0.9662921348314607	1.0674157303370786	30.0
1.0685714285714285	1.0617142857142856	1.0685714285714285	168.0
1.0668449197860963	1.0748663101604279	1.0561497326203209	151.0
1.0628717077315208	1.0781648258283771	1.0560747663551402	223.0
1.0853658536585367	1.08130081300813	1.1585365853658536	128.0
1.0844444444444445	1.0177777777777777	1.12	122.0
1.0	1.0	1.0	9.0
1.0744186046511628	1.0465116279069768	1.0651162790697675	157.0
1.0495436766623207	1.0234680573663624	1.1016949152542372	155.0
0.9738562091503268	1.026143790849673	1.1045751633986929	42.0
0.9	1.0	1.0	14.0
0.9655172413793104	1.103448275862069	1.0344827586206897	35.0
0.9661016949152542	0.847457627118644	1.0338983050847457	43.0
1.0	1.0	1.0	7.0
1.025974025974026	0.961038961038961	1.025974025974026	41.0
1.0411522633744856	1.0658436213991769	1.1042524005486969	174.0
1.2222222222222223	1.2222222222222223	1.1111111111111112	20.0
1.0484848484848486	1.0363636363636364	1.0545454545454545	87.0
1.14519906323185	1.135831381733021	1.1077283372365339	129.0
1.0	1.0176991150442478	1.0176991150442478	63.0
1.0932203389830508	1.11864406779661	1.1271186440677967	89.0
1.060483870967742	1.0725806451612903	1.0665322580645162	221.0
0.8208955223880597	0.9402985074626866	0.8507462686567164	19.0
1.0980066445182723	1.0980066445182723	1.0930232558139534	248.0
0.9787234042553191	0.9361702127659575	1.0	24.0
1.0865384615384615	1.1057692307692308	1.0961538461538463	118.0
1.0074074074074073	1.0222222222222221	1.0592592592592593	89.0
1.0682926829268293	1.048780487804878	1.078048780487805	120.0
1.0962025316455697	1.0911392405063292	1.1164556962025316	124.0
1.0664451827242525	1.0033222591362125	1.0365448504983388	144.0
1.0	0.8260869565217391	0.9130434782608695	17.0
1.060897435897436	1.0544871794871795	1.0769230769230769	166.0
1.0893203883495146	1.0699029126213593	1.0932038834951456	116.0
1.0571428571428572	1.0714285714285714	1.1	51.0
1.011461318051576	1.0515759312320916	1.0630372492836677	96.0
1.059090909090909	1.0272727272727273	1.0863636363636364	138.0
1.038647342995169	1.1014492753623188	1.0821256038647342	119.0
1.0483516483516484	1.0747252747252747	1.065934065934066	142.0
0.7037037037037037	0.8148148148148148	0.7777777777777778	13.0
1.0744827586206898	1.08	1.1020689655172413	173.0
1.1123595505617978	1.1123595505617978	1.1438202247191012	132.0
1.0462287104622872	1.0559610705596107	1.0632603406326033	129.0
1.0806451612903225	1.064516129032258	1.1088709677419355	129.0
1.0251046025104602	1.00836820083682	1.0334728033472804	62.0
1.0758426966292134	1.0393258426966292	1.0786516853932584	164.0
1.0165425971877584	1.0479735318444996	1.0727874276261373	232.0
1.0503597122302157	1.0071942446043165	1.0503597122302157	80.0
1.0786610878661087	1.088702928870293	1.1255230125523012	232.0
1.0	0.9219512195121952	0.9707317073170731	69.0
1.0606060606060606	1.0745920745920745	1.097902097902098	124.0
1.0498753117206983	1.0698254364089776	1.0947630922693268	123.0
0.7948717948717948	0.8974358974358975	0.8974358974358975	38.0
1.0181347150259068	1.0259067357512954	1.0803108808290156	193.0
0.8529411764705882	0.9411764705882353	0.8529411764705882	18.0
1.067632850241546	1.077294685990338	1.0724637681159421	125.0
1.0	1.3333333333333333	1.3333333333333333	18.0
1.0797227036395147	1.0797227036395147	1.0935875216637783	109.0
1.0751879699248121	1.0751879699248121	1.0776942355889725	195.0
1.041237113402062	1.0206185567010309	1.0701030927835051	122.0
1.0273972602739727	1.0328767123287672	1.0383561643835617	85.0
1.0723404255319149	1.0595744680851065	1.0638297872340425	121.0
1.0626631853785902	1.08355091383812	1.0939947780678851	235.0


==> nbpCM_praline-package-2020-05-18.tex <==
mixed/kieler	ports/kieler	nodes/kieler	vtcs
1.118491921005386	1.0969479353680431	1.125673249551167	114.0
1.0404217926186292	1.0369068541300528	1.0369068541300528	237.0
0.9617834394904459	0.9363057324840764	1.0509554140127388	54.0
1.1209068010075567	1.0906801007556675	1.105793450881612	123.0
0.8954248366013072	0.8562091503267973	0.8562091503267973	67.0
0.9578947368421052	0.8947368421052632	1.0210526315789474	40.0
1.051107325383305	1.0885860306643953	1.0885860306643953	190.0
1.0425531914893618	1.0297872340425531	1.0553191489361702	122.0
1.0698689956331877	1.0873362445414847	1.0698689956331877	70.0
1.0507399577167018	1.0591966173361522	1.0338266384778012	135.0
1.0745454545454545	1.0618181818181818	1.1236363636363635	244.0
1.0844155844155845	1.0811688311688312	1.12987012987013	169.0
0.9186046511627907	0.8604651162790697	0.9534883720930233	110.0
0.9685393258426966	0.9280898876404494	0.9820224719101124	121.0
0.782608695652174	0.782608695652174	0.782608695652174	31.0
1.0392156862745099	0.8431372549019608	0.9215686274509803	15.0
0.9197707736389685	0.9828080229226361	1.0	93.0
1.0	1.0	1.0	8.0
0.7333333333333333	0.7333333333333333	1.0	21.0
1.0176991150442478	0.9793510324483776	0.9970501474926253	168.0
0.9754098360655737	0.9508196721311475	1.0	133.0
1.0073394495412844	1.003669724770642	1.0293577981651376	145.0
1.0576671035386631	1.055045871559633	1.0838794233289646	149.0
1.0286298568507157	1.016359918200409	1.0	147.0
1.0593220338983051	1.0254237288135593	1.076271186440678	60.0
1.0	1.0209424083769634	1.036649214659686	91.0
0.9744408945686901	0.9552715654952076	1.0	102.0
1.0651162790697675	1.0883720930232559	1.0930232558139534	134.0
1.0	1.0	1.0	13.0
0.8837209302325582	0.7906976744186046	0.9302325581395349	24.0
1.0359116022099448	1.058011049723757	1.0966850828729282	153.0
0.9536231884057971	0.9420289855072463	0.8956521739130435	86.0
1.078078078078078	1.042042042042042	1.078078078078078	164.0
1.058252427184466	1.0776699029126213	1.0533980582524272	134.0
0.8928571428571429	0.9642857142857143	0.8214285714285714	31.0
0.9466666666666667	1.0	0.9786666666666667	100.0
1.0597014925373134	1.0786974219810042	1.1031207598371777	186.0
1.0	1.0	1.0	8.0
1.0	1.027027027027027	1.0	47.0
1.0836501901140685	1.0760456273764258	1.0608365019011408	139.0
1.0079617834394905	1.0286624203821657	1.0509554140127388	241.0
1.1346153846153846	1.0576923076923077	1.0961538461538463	58.0
1.0446650124069479	1.0446650124069479	1.0099255583126552	122.0
1.0698689956331877	1.0698689956331877	1.098981077147016	169.0
1.0636363636363637	1.0136363636363637	1.0863636363636364	126.0
1.0253164556962024	1.0911392405063292	1.1265822784810127	120.0
0.9849056603773585	0.969811320754717	1.0150943396226415	138.0
1.010752688172043	1.025089605734767	1.007168458781362	144.0
1.005050505050505	0.9949494949494949	1.0101010101010102	102.0
0.9424920127795527	0.9424920127795527	0.9808306709265175	109.0
0.8181818181818182	0.8181818181818182	0.8181818181818182	14.0
1.0806794055201698	1.0339702760084926	1.089171974522293	133.0
0.9344262295081968	0.9754098360655737	1.0163934426229508	113.0
0.9285714285714286	0.8571428571428571	0.8571428571428571	32.0
1.0420091324200913	1.0511415525114156	1.0748858447488585	241.0
1.068062827225131	1.1047120418848169	1.068062827225131	105.0
0.9967051070840197	0.9769357495881383	0.9934102141680395	159.0
0.9344262295081968	0.8797814207650273	0.9672131147540983	107.0
1.0384615384615385	1.047008547008547	1.0598290598290598	194.0
0.9119496855345912	0.8679245283018868	0.8742138364779874	99.0
0.9878048780487805	0.9878048780487805	0.9512195121951219	60.0
1.0256410256410255	1.0598290598290598	1.1111111111111112	76.0
1.0431266846361187	1.0377358490566038	1.005390835579515	92.0
1.0588235294117647	1.0374331550802138	1.0962566844919786	97.0
1.125	0.8571428571428571	1.0178571428571428	47.0
1.0	1.0	1.0	10.0
1.061764705882353	1.0852941176470587	1.0852941176470587	164.0
1.0357142857142858	1.0029761904761905	1.005952380952381	168.0
0.9325301204819277	0.9710843373493976	0.9710843373493976	115.0
1.0788177339901477	0.9802955665024631	1.0098522167487685	63.0
0.9628482972136223	0.9256965944272446	0.9690402476780186	80.0
1.0240343347639485	1.0326180257510729	1.0532188841201717	234.0
0.8759305210918115	0.9503722084367245	0.9751861042183623	119.0
1.0745341614906831	1.0745341614906831	1.0559006211180124	107.0
1.0733333333333333	1.0033333333333334	1.0833333333333333	165.0
0.92	1.08	1.08	21.0
1.0921658986175116	1.055299539170507	1.0737327188940091	117.0
1.0112359550561798	1.0224719101123596	1.0786516853932584	97.0
0.9575757575757575	1.018181818181818	0.9575757575757575	82.0
0.9753846153846154	0.9261538461538461	0.9753846153846154	98.0
0.9636363636363636	0.9090909090909091	0.9272727272727272	40.0
1.0541455160744502	1.0879864636209813	1.0947546531302876	154.0
0.863013698630137	0.8356164383561644	0.9452054794520548	27.0
0.9744136460554371	0.9957356076759062	1.0	115.0
1.0674157303370786	1.0112359550561798	1.0898876404494382	49.0
1.0	1.0	1.0	7.0
1.0964630225080385	1.0707395498392283	1.0321543408360128	105.0
1.0361663652802893	1.0072332730560578	1.0506329113924051	148.0
1.1063829787234043	1.148936170212766	1.127659574468085	43.0
1.025089605734767	0.982078853046595	1.003584229390681	142.0
1.0	1.0	1.0	14.0
1.110091743119266	1.018348623853211	1.036697247706422	40.0
1.1011560693641618	1.0953757225433527	1.0809248554913296	123.0
0.9393939393939394	1.0	1.0	36.0
1.125	1.125	1.25	22.0
1.05625	1.09375	1.0875	102.0
1.0513478818998716	1.0410783055198973	1.0616174582798459	194.0
1.0332541567695963	1.0380047505938241	1.0285035629453683	128.0
0.9698216735253772	0.9780521262002744	1.027434842249657	157.0
1.0089020771513353	1.0267062314540059	1.0356083086053411	174.0
1.0655066530194472	1.0532241555783008	1.1003070624360287	199.0
1.062015503875969	1.0930232558139534	1.124031007751938	55.0
1.1547619047619047	1.0793650793650793	1.0873015873015872	112.0
1.1182266009852218	1.1083743842364533	1.1083743842364533	111.0
0.9036144578313253	1.0481927710843373	1.0963855421686748	25.0
1.0348837209302326	1.065891472868217	1.0813953488372092	105.0
0.9532163742690059	0.9298245614035088	0.9415204678362573	58.0
0.9811320754716981	0.9622641509433962	1.0377358490566038	55.0
0.9743119266055046	0.9889908256880734	1.018348623853211	131.0
1.0	1.0	1.0	11.0
1.037313432835821	0.8432835820895522	1.0746268656716418	84.0
0.9847328244274809	1.0916030534351144	1.0763358778625953	43.0
0.9909638554216867	1.0180722891566265	1.0301204819277108	168.0
1.0208333333333333	0.9375	1.0208333333333333	41.0
1.08675799086758	1.0547945205479452	1.1004566210045663	133.0
0.8148148148148148	0.8518518518518519	1.0740740740740742	28.0
0.9876160990712074	1.0	0.9566563467492261	91.0
1.0	1.0178571428571428	1.0803571428571428	61.0
1.0576923076923077	1.123076923076923	1.0884615384615384	129.0
1.0493273542600896	1.0762331838565022	1.0762331838565022	150.0
1.101644245142003	1.0687593423019432	1.0896860986547086	187.0
1.0985221674876848	1.1133004926108374	1.1330049261083743	118.0
1.0808510638297872	1.0085106382978724	1.0808510638297872	115.0
1.121654501216545	1.1167883211678833	1.1265206812652069	104.0
1.0315789473684212	1.0473684210526315	1.0578947368421052	113.0
1.055299539170507	1.0460829493087558	1.1105990783410138	132.0
1.0	1.0	1.0	17.0
1.064516129032258	1.096774193548387	1.0591397849462365	113.0
0.6	1.0	0.6	11.0
0.9695121951219512	1.0426829268292683	1.0975609756097562	94.0
1.0556962025316456	1.0506329113924051	1.0607594936708862	122.0
0.75	1.0	1.0833333333333333	14.0
1.0397350993377483	1.0264900662251655	1.0927152317880795	37.0
1.0576631259484066	1.069802731411229	1.069802731411229	178.0
0.9797297297297297	1.0	1.0405405405405406	66.0
1.0485115766262403	1.0441014332965821	1.0661521499448732	217.0
1.0638297872340425	1.0372340425531914	1.053191489361702	79.0
1.0975609756097562	0.9024390243902439	1.146341463414634	13.0
1.0592592592592593	1.0493827160493827	1.0592592592592593	111.0
1.0847953216374269	1.0789473684210527	1.0818713450292399	170.0
1.0854368932038836	1.0854368932038836	1.0737864077669903	152.0
1.0078125	1.0	1.01171875	131.0
0.950920245398773	0.9570552147239264	0.9877300613496932	134.0
0.9714765100671141	0.9966442953020134	1.0369127516778522	202.0
1.0191780821917809	0.9917808219178083	1.021917808219178	169.0
1.0524344569288389	1.0730337078651686	1.0599250936329587	254.0
1.070298769771529	1.070298769771529	1.0492091388400704	113.0
1.0548780487804879	1.079268292682927	1.0182926829268293	107.0
1.0754716981132075	1.0781671159029649	1.0889487870619947	194.0
1.0946969696969697	1.0795454545454546	1.1022727272727273	128.0
1.0544502617801048	1.0586387434554974	1.0586387434554974	226.0
0.9741379310344828	1.0517241379310345	1.0344827586206897	87.0
0.92	0.92	1.0	30.0
1.0056022408963585	1.0168067226890756	1.0560224089635855	187.0
0.9611650485436893	0.9611650485436893	0.941747572815534	92.0
1.0588235294117647	1.0294117647058822	0.9705882352941176	50.0
1.0575539568345325	0.9856115107913669	1.064748201438849	93.0
1.0	1.0	1.0	8.0
0.8	0.6	0.6	14.0
1.0506329113924051	1.0683544303797468	1.081012658227848	201.0
1.0825242718446602	1.0533980582524272	1.1262135922330097	112.0
1.1777777777777778	1.0666666666666667	1.1	53.0
1.0724637681159421	1.077294685990338	1.0821256038647342	131.0
1.0683506686478454	1.0683506686478454	1.074294205052006	184.0
1.5	1.5	1.1666666666666667	15.0
0.7647058823529411	0.6470588235294118	0.7647058823529411	18.0
1.0363636363636364	1.084848484848485	1.096969696969697	50.0
1.0	0.9630390143737166	1.0123203285420945	126.0
1.0847457627118644	1.152542372881356	1.1355932203389831	99.0
1.10752688172043	1.064516129032258	1.10752688172043	55.0
1.25	0.75	0.75	5.0
0.9777777777777777	0.9866666666666667	1.0444444444444445	111.0
0.9865771812080537	1.0	1.0402684563758389	44.0
1.2272727272727273	1.3636363636363635	1.3181818181818181	27.0
1.0600193610842208	1.0387221684414327	1.0058083252662149	209.0
0.9090909090909091	1.0	1.0	18.0
0.9615384615384616	1.0384615384615385	1.0769230769230769	27.0
1.075268817204301	1.021505376344086	1.0465949820788532	230.0
0.9766536964980544	0.9377431906614786	0.9766536964980544	73.0
1.0	0.8940397350993378	1.0	78.0
1.1	1.1	1.0	18.0
1.0912162162162162	1.0675675675675675	1.1013513513513513	190.0
0.9701492537313433	0.9701492537313433	1.0298507462686568	49.0
0.7142857142857143	0.7142857142857143	0.7142857142857143	11.0
1.0057142857142858	1.002857142857143	1.04	188.0
0.8898071625344353	0.9614325068870524	0.9889807162534435	104.0
1.0894941634241244	1.0778210116731517	1.0155642023346303	202.0
1.0930232558139534	1.083720930232558	1.083720930232558	141.0
1.0566572237960339	1.0509915014164306	1.081208687440982	235.0
1.0300751879699248	1.0620300751879699	1.0845864661654134	224.0
1.0	1.0	1.0	2.0
1.034934497816594	1.091703056768559	1.0960698689956332	145.0
1.0	1.08	1.0	33.0
1.121212121212121	0.9393939393939394	1.0606060606060606	38.0
1.0152542372881357	0.9932203389830508	1.0423728813559323	230.0
0.8851963746223565	0.9516616314199395	0.9697885196374623	93.0
0.967741935483871	0.9032258064516129	1.032258064516129	35.0
0.9227799227799228	0.9922779922779923	0.9613899613899614	97.0
1.0327868852459017	1.030054644808743	1.0737704918032787	170.0
0.972027972027972	0.8741258741258742	0.965034965034965	84.0
1.0044247787610618	1.1194690265486726	1.0442477876106195	113.0
1.0246913580246915	1.0617283950617284	1.0740740740740742	102.0
1.0934579439252337	1.0560747663551402	1.2616822429906542	47.0
0.995260663507109	1.0	1.033175355450237	133.0
1.0826666666666667	1.0693333333333332	1.0853333333333333	197.0
1.0837988826815643	1.111731843575419	1.106145251396648	95.0
1.092063492063492	1.0793650793650793	1.092063492063492	171.0
1.0326530612244897	1.0571428571428572	1.0506122448979591	239.0
1.065359477124183	1.091503267973856	1.056644880174292	99.0
0.9905660377358491	0.9905660377358491	0.9716981132075472	44.0
1.0242424242424242	1.1454545454545455	1.084848484848485	44.0
1.0184119677790564	1.0437284234752588	1.0575373993095512	186.0
1.0209205020920502	1.0251046025104602	0.9874476987447699	119.0
1.0558659217877095	1.0782122905027933	1.089385474860335	95.0
1.0380952380952382	1.1333333333333333	1.1714285714285715	45.0
1.0608365019011408	1.091254752851711	1.0608365019011408	69.0
0.9264214046822743	0.939799331103679	0.959866220735786	89.0
1.0669344042838018	1.0428380187416333	1.0321285140562249	148.0
0.8620689655172413	0.9363395225464191	0.9151193633952255	107.0
0.8375	0.825	0.975	67.0
0.9024390243902439	1.016260162601626	0.967479674796748	41.0
0.9340659340659341	0.8681318681318682	0.9560439560439561	55.0
0.94	0.92	0.94	41.0
0.0	0.0	0.0	10.0
1.0	0.8	1.0	7.0
1.0	0.9966442953020134	1.0201342281879195	143.0
1.0249776984834968	1.0446030330062444	1.0660124888492417	245.0
1.046685340802988	1.072829131652661	1.0373482726423904	241.0
0.9411764705882353	0.9327731092436975	0.9495798319327731	62.0
1.0796019900497513	1.064676616915423	1.0696517412935322	122.0
1.0930232558139534	1.0775193798449612	1.073643410852713	142.0
1.0346320346320346	1.0346320346320346	1.0346320346320346	87.0
1.0	0.7575757575757576	1.0	18.0
1.032967032967033	1.0769230769230769	1.065934065934066	37.0
1.1095890410958904	1.1461187214611872	1.1187214611872147	86.0
1.0955315870570108	1.0677966101694916	1.12326656394453	156.0
0.9481865284974094	0.9896373056994818	0.9481865284974094	80.0
0.9875	1.175	1.15	69.0
1.0	1.3	0.9	18.0
1.0575815738963532	1.0652591170825336	1.1036468330134357	156.0
1.0	0.9894179894179894	1.0105820105820107	53.0
1.0654545454545454	1.0581818181818181	1.0072727272727273	80.0
1.087323943661972	1.0704225352112675	1.095774647887324	193.0
1.072112676056338	1.0833802816901408	1.0698591549295775	313.0
1.0650054171180932	1.0260021668472372	1.0411700975081257	241.0
1.0	1.0	1.0	5.0
1.0515463917525774	1.041237113402062	1.0154639175257731	114.0
1.1015873015873017	1.0444444444444445	1.1015873015873017	80.0
1.0701754385964912	0.9298245614035088	1.105263157894737	34.0
1.0802919708029197	1.0802919708029197	1.0802919708029197	130.0
0.9388379204892966	0.9571865443425076	0.8654434250764526	91.0
1.2325581395348837	1.2325581395348837	1.2325581395348837	43.0
1.1181434599156117	1.0928270042194093	1.1012658227848102	122.0
1.1167608286252355	1.0941619585687383	1.0225988700564972	141.0
1.0447154471544715	1.0406504065040652	1.032520325203252	130.0
1.0952380952380953	0.9365079365079365	1.1587301587301588	27.0
1.0138888888888888	1.0231481481481481	1.0324074074074074	130.0
1.0165745856353592	1.0607734806629834	1.0828729281767955	120.0
0.9494584837545126	1.0216606498194947	1.0144404332129964	86.0
1.0410958904109588	0.9041095890410958	0.958904109589041	51.0
1.0521739130434782	0.9478260869565217	1.0521739130434782	60.0
1.1096491228070176	1.0921052631578947	1.1228070175438596	134.0
1.1007957559681698	1.1007957559681698	1.129973474801061	127.0
1.043282236248873	1.0450856627592426	1.036068530207394	245.0
1.0417457305502846	1.0379506641366223	1.0986717267552182	163.0
0.9761904761904762	1.010204081632653	1.0136054421768708	157.0
1.0	1.0	1.0	2.0
0.9473684210526315	0.9736842105263158	1.105263157894737	26.0
1.056420233463035	1.038910505836576	1.0856031128404668	212.0
1.4	0.8	1.0	21.0
1.0521739130434782	1.0347826086956522	1.0869565217391304	60.0
1.0301974448315911	1.0766550522648084	1.051103368176539	170.0
1.0143198090692125	0.9952267303102625	0.9761336515513126	115.0
1.0246913580246915	1.0740740740740742	1.0603566529492456	121.0
1.0	0.9655172413793104	0.9425287356321839	56.0
1.0	0.9895287958115183	1.0	71.0
0.9743589743589743	0.8717948717948718	0.9743589743589743	26.0
1.0769230769230769	1.0	1.1538461538461537	28.0
1.032	1.048	1.048	48.0
1.036939313984169	0.9736147757255936	1.0633245382585752	107.0
1.0918367346938775	1.066326530612245	1.114795918367347	132.0
1.1081081081081081	1.018018018018018	1.1081081081081081	37.0
0.8709677419354839	0.8573853989813243	0.966044142614601	117.0
1.0486223662884928	1.0551053484602917	1.0907617504051863	147.0
1.0069444444444444	0.9791666666666666	0.9861111111111112	157.0
1.1818181818181819	1.0	1.4545454545454546	8.0
1.0579710144927537	1.1014492753623188	1.0724637681159421	131.0
0.9736842105263158	0.9868421052631579	1.0526315789473684	89.0
1.08	1.056	1.072	95.0
1.0677290836653386	1.047808764940239	1.0677290836653386	147.0
1.0531645569620254	1.0151898734177216	1.058227848101266	159.0
1.0989583333333333	1.1041666666666667	1.0677083333333333	113.0
0.9162790697674419	1.0	1.027906976744186	77.0
0.96875	0.875	1.25	40.0
1.0185185185185186	1.0185185185185186	1.0308641975308641	101.0
1.076086956521739	1.1358695652173914	1.0978260869565217	86.0
1.0686868686868687	1.0646464646464646	1.0747474747474748	219.0
1.08	1.1	1.07	62.0
1.07909604519774	1.0847457627118644	1.0819209039548023	130.0
1.0425531914893618	1.060790273556231	1.0547112462006079	112.0
1.080188679245283	1.070754716981132	1.070754716981132	126.0
1.0322981366459627	1.0422360248447204	1.0198757763975155	182.0
0.9834710743801653	1.0495867768595042	1.0110192837465564	172.0
1.0226757369614512	0.9773242630385488	1.0453514739229024	124.0
1.0728744939271255	1.0512820512820513	1.0890688259109311	121.0
0.9254237288135593	0.9593220338983051	1.0	100.0
1.0	1.0	1.0	5.0
1.036617262423714	1.02615518744551	1.059285091543156	234.0
1.0538720538720538	1.0650953984287317	1.0606060606060606	225.0
1.0888888888888888	1.0777777777777777	1.0333333333333334	63.0
1.0555555555555556	1.0648148148148149	1.0694444444444444	126.0
1.009546539379475	1.0047732696897376	0.9809069212410502	115.0
1.0234375	1.0651041666666667	1.1119791666666667	171.0
0.9290465631929047	1.0133037694013303	1.0221729490022173	122.0
0.9744525547445255	1.010948905109489	1.0547445255474452	139.0
1.0505050505050506	1.0378787878787878	1.0656565656565657	197.0
1.0205479452054795	1.0753424657534247	1.1027397260273972	105.0
1.0	1.3333333333333333	1.1666666666666667	11.0
1.0562130177514792	1.0532544378698225	1.0236686390532543	173.0
1.0588235294117647	0.9803921568627451	0.9607843137254902	65.0
1.050909090909091	1.050909090909091	1.0727272727272728	69.0
1.1419354838709677	1.0903225806451613	1.0903225806451613	27.0
0.8018575851393189	0.7585139318885449	0.9195046439628483	92.0
1.0735294117647058	1.0588235294117647	1.1323529411764706	68.0
1.2	1.2	1.2	20.0
1.0691358024691358	1.054320987654321	1.1135802469135803	130.0
1.047872340425532	1.0212765957446808	1.0425531914893618	96.0
0.9230769230769231	1.0	1.0	14.0
0.9406880189798339	0.9620403321470937	1.0094899169632265	166.0
1.0968586387434556	1.0863874345549738	1.1151832460732984	180.0
1.0	1.032258064516129	1.0483870967741935	63.0
1.0678642714570858	1.0399201596806387	1.0638722554890219	156.0
1.0576923076923077	0.9807692307692307	1.0769230769230769	120.0
1.0114942528735633	1.0114942528735633	1.0666666666666667	162.0
1.0587371512481645	1.0293685756240822	1.0939794419970632	205.0
1.0859504132231406	1.1024793388429752	1.0760330578512396	168.0
1.103448275862069	0.9655172413793104	0.9827586206896551	62.0
1.099502487562189	1.1592039800995024	1.1194029850746268	85.0
1.021341463414634	1.0152439024390243	1.0335365853658536	163.0
1.0718954248366013	1.0555555555555556	1.0620915032679739	153.0
1.0028301886792452	1.0	1.019811320754717	354.0
1.2222222222222223	0.8888888888888888	1.1111111111111112	17.0
1.055393586005831	1.0495626822157433	1.075801749271137	156.0
1.015	0.9975	1.0475	218.0
0.9464882943143813	0.8996655518394648	0.9331103678929766	85.0
1.056338028169014	1.0704225352112675	1.0422535211267605	66.0
1.082324455205811	1.1016949152542372	1.0968523002421307	131.0
0.9924812030075187	1.0338345864661653	1.0112781954887218	160.0
0.984251968503937	0.889763779527559	1.062992125984252	54.0
1.010840108401084	1.016260162601626	1.024390243902439	168.0
1.0385852090032155	1.0814576634512325	1.07502679528403	231.0
0.8727272727272727	0.8909090909090909	0.8545454545454545	48.0
2.0	2.0	2.0	8.0
1.096026490066225	1.0629139072847682	1.0794701986754967	169.0
0.963076923076923	0.92	0.9876923076923076	91.0
1.0070422535211268	1.0140845070422535	0.9929577464788732	144.0
1.0053333333333334	1.0533333333333332	0.9946666666666667	105.0
1.0804597701149425	0.9885057471264368	1.0804597701149425	87.0
1.1	1.2	1.1	18.0
0.9625468164794008	0.8951310861423221	0.9550561797752809	82.0
0.9891304347826086	1.076086956521739	1.0434782608695652	52.0
2.0	2.0	2.0	8.0
0.9702602230483272	1.0	1.0185873605947955	127.0
0.8771929824561403	0.8245614035087719	0.7543859649122807	39.0
0.9130434782608695	0.9347826086956522	0.8768115942028986	79.0
1.0192307692307692	1.0961538461538463	1.0769230769230769	39.0
1.0176730486008836	1.0618556701030928	1.0206185567010309	170.0
1.0034423407917383	0.9896729776247849	1.0654044750430292	146.0
1.0980392156862746	1.0784313725490196	1.1372549019607843	50.0
0.8857142857142857	0.8285714285714286	0.9428571428571428	35.0
1.0802620802620804	1.0458640458640458	1.058968058968059	246.0
1.103359173126615	1.0981912144702843	1.0723514211886305	123.0
0.9027027027027027	1.0	1.0324324324324323	38.0
1.0091533180778032	1.0091533180778032	1.0594965675057209	105.0
1.021505376344086	1.0573476702508962	0.996415770609319	144.0
1.1278772378516624	1.1074168797953965	1.1125319693094629	120.0
1.0561122244488979	1.0440881763527055	1.0681362725450902	144.0
1.1026548672566372	1.08141592920354	1.0849557522123894	113.0
1.0367534456355283	0.996937212863706	1.0336906584992342	158.0
1.087378640776699	1.029126213592233	1.0485436893203883	77.0


==> nbpDA_generated_2021-08-06_17-27-03.tex <==
fd/rand	bfs/rand	vtcs
0.9822222222222222	1.08	68.0
0.9678942398489141	0.9641170915958451	182.0
0.8969072164948454	1.041237113402062	33.0
0.947565543071161	1.0024968789013733	172.0
0.987987987987988	1.0360360360360361	145.0
0.8963414634146342	1.0426829268292683	81.0
1.157377049180328	1.118032786885246	90.0
0.9847094801223242	0.963302752293578	142.0
0.9952718676122931	0.9858156028368794	224.0
0.9393939393939394	0.8787878787878788	41.0
1.0087336244541485	1.034934497816594	150.0
0.9178515007898894	0.9273301737756714	142.0
0.9584569732937686	0.9940652818991098	96.0
0.9799691833590138	0.9984591679506933	204.0
0.8348623853211009	0.981651376146789	48.0
0.9831223628691983	1.0056258790436006	134.0
0.9646365422396856	1.0	139.0
1.0172413793103448	0.9827586206896551	41.0
0.944954128440367	0.9596330275229358	145.0
0.9613899613899614	1.0205920205920207	169.0
0.9595959595959596	1.0	23.0
1.0015060240963856	0.9954819277108434	228.0
0.9398998330550918	1.003338898163606	127.0
0.9542947202521671	0.9968479117415288	236.0
0.9904306220095693	1.0095693779904307	100.0
0.8700696055684455	0.9489559164733179	109.0
1.0930232558139534	1.0930232558139534	32.0
0.9739413680781759	0.9804560260586319	75.0
0.9509632224168126	0.9544658493870403	133.0
0.8904109589041096	0.9452054794520548	111.0
0.9041533546325878	0.9808306709265175	84.0
0.9662162162162162	1.0067567567567568	134.0
0.9602977667493796	0.9875930521091811	174.0
0.9964028776978417	0.9784172661870504	143.0
0.976878612716763	1.0423892100192678	126.0
0.983065198983912	1.0304826418289585	213.0
0.9102564102564102	0.9358974358974359	89.0
0.9565217391304348	1.0108695652173914	43.0
1.0	0.9829787234042553	49.0
0.9774647887323944	1.0394366197183098	78.0
1.0157977883096367	1.0221169036334914	115.0
1.0031298904538342	1.050078247261346	142.0
0.9539295392953929	0.9701897018970189	156.0
0.9806629834254144	1.0165745856353592	158.0
1.017391304347826	1.0521739130434782	68.0
1.0	1.6666666666666667	9.0
0.9712230215827338	0.9856115107913669	39.0
1.0	1.0	11.0
0.978401727861771	1.038876889848812	128.0
0.991304347826087	1.0260869565217392	131.0
1.0	0.8	20.0
0.0	0.0	12.0
0.934640522875817	1.0	40.0
0.9724655819774718	0.9899874843554443	179.0
0.9770114942528736	0.967816091954023	91.0
0.9863013698630136	1.0410958904109588	71.0
1.005181347150259	1.0336787564766838	205.0
1.0350877192982457	0.9766081871345029	36.0
0.9916317991631799	0.9748953974895398	126.0
0.890625	0.890625	58.0
0.970873786407767	1.0436893203883495	99.0
0.9953379953379954	1.006993006993007	150.0
0.9491916859122402	1.0	91.0
0.9074550128534704	0.9074550128534704	105.0
0.926829268292683	0.9902439024390244	105.0
0.9659090909090909	1.0	52.0
1.0151515151515151	1.0151515151515151	104.0
1.0114285714285713	1.1257142857142857	68.0
0.9451476793248945	0.9746835443037974	129.0
0.9397260273972603	0.9753424657534246	189.0
0.8764478764478765	0.9768339768339769	61.0
0.9524564183835182	0.9334389857369255	157.0
0.7894736842105263	0.8947368421052632	8.0
1.6666666666666667	1.6666666666666667	7.0
0.9722675367047309	0.9690048939641109	213.0
1.0	1.0	4.0
0.8943894389438944	0.9570957095709571	154.0
0.5555555555555556	0.5555555555555556	16.0
0.9571734475374732	0.9593147751605996	169.0
0.9467787114845938	0.9467787114845938	132.0
0.9832985386221295	0.9916492693110647	126.0
0.9291635267520724	0.9608138658628486	203.0
0.9959266802443992	1.0040733197556009	109.0
0.9680851063829787	1.0319148936170213	79.0
1.0655737704918034	1.1366120218579234	50.0
0.9598393574297188	1.0401606425702812	46.0
0.9069767441860465	0.9948320413436692	105.0
0.9032258064516129	0.8870967741935484	57.0
0.9456118665018541	0.9950556242274413	143.0
0.9554140127388535	0.9872611464968153	96.0
0.9618055555555556	0.9930555555555556	131.0
0.9692307692307692	0.9230769230769231	47.0
1.0043668122270741	1.017467248908297	117.0
0.8962264150943396	0.9575471698113207	90.0
0.8360655737704918	0.9016393442622951	24.0
1.0156657963446476	1.052219321148825	98.0
1.1176470588235294	1.3529411764705883	15.0
1.0	1.0	4.0
0.9656786271450858	0.9875195007800313	129.0
0.9719887955182073	0.9663865546218487	81.0
0.9396825396825397	0.9333333333333333	139.0
0.9267399267399268	1.0	92.0
0.9948652118100129	1.0154043645699615	168.0
0.9953917050691244	1.0138248847926268	117.0
1.0	1.0	7.0
0.9641379310344828	0.9972413793103448	158.0
1.0477064220183485	1.073394495412844	136.0
0.8924731182795699	0.978494623655914	34.0
0.8971553610503282	1.013129102844639	162.0
1.0975609756097562	1.1951219512195121	34.0
0.9812865497076023	1.0116959064327486	177.0
0.9682539682539683	0.9126984126984127	76.0
0.9972862957937585	1.0597014925373134	164.0
1.0957446808510638	1.0319148936170213	55.0
0.9485981308411215	0.9813084112149533	122.0
0.9315589353612167	0.9746514575411914	180.0
1.0	1.0	6.0
0.972972972972973	0.9831081081081081	127.0
1.0056258790436006	1.0056258790436006	140.0
0.938375350140056	0.9719887955182073	78.0
0.8770226537216829	0.941747572815534	69.0
0.9737856592135697	1.0030840400925212	243.0
1.0	1.163265306122449	34.0
0.7777777777777778	0.7777777777777778	28.0
0.9725274725274725	1.0384615384615385	87.0
0.75	0.7272727272727273	22.0
0.9561551433389545	1.0101180438448567	142.0
0.9866412213740458	0.9809160305343512	219.0
0.875	1.0	29.0
0.9701492537313433	1.1194029850746268	17.0
0.9518459069020867	1.0224719101123596	120.0
0.9681762545899633	1.0195838433292534	168.0
0.9796334012219959	0.9633401221995926	114.0
0.9135802469135802	1.037037037037037	93.0
0.7777777777777778	1.0	15.0
1.0	1.0588235294117647	14.0
1.0169491525423728	1.0932203389830508	64.0
1.030967741935484	1.0464516129032257	120.0
0.9619909502262444	1.0036199095022624	219.0
0.9523809523809523	0.8888888888888888	56.0
0.9098360655737705	0.9262295081967213	94.0
0.9507908611599297	1.0140597539543057	132.0
1.007843137254902	1.0392156862745099	115.0
0.8502994011976048	0.9161676646706587	82.0
1.0	1.0	5.0
0.9547325102880658	0.9711934156378601	127.0
0.9428571428571428	0.9936507936507937	145.0
0.9846153846153847	1.0131868131868131	195.0
0.9571209800918836	1.003062787136294	150.0
1.0	0.9856115107913669	32.0
0.9316546762589928	0.9748201438848921	120.0
0.9472573839662447	0.9493670886075949	155.0
0.9292035398230089	0.911504424778761	40.0
0.9745222929936306	1.0286624203821657	108.0
0.9823008849557522	1.0353982300884956	41.0
1.0222222222222221	1.0888888888888888	24.0
0.9354838709677419	0.9354838709677419	29.0
0.9183673469387755	0.9727891156462585	135.0
0.9619883040935673	0.97953216374269	146.0
0.9688195991091314	0.9732739420935412	200.0
0.9617834394904459	0.9787685774946921	129.0
0.9954954954954955	1.009009009009009	105.0
0.9398496240601504	0.9548872180451128	81.0
0.9691119691119691	1.0038610038610039	134.0
0.8562628336755647	0.8685831622176592	103.0
1.0100502512562815	0.9949748743718593	98.0
1.0987654320987654	1.1975308641975309	36.0
0.9559902200488998	0.9657701711491442	78.0
0.9744680851063829	1.0198581560283688	169.0
0.9119496855345912	1.0125786163522013	113.0
0.8705035971223022	0.9376498800959233	119.0
0.8260869565217391	1.0072463768115942	76.0
0.9558359621451105	0.9968454258675079	251.0
1.023972602739726	1.0308219178082192	157.0
0.9631490787269682	1.0083752093802345	208.0
0.9314128943758574	0.9835390946502057	154.0
0.946927374301676	0.9692737430167597	190.0
0.9690844233055886	0.9785969084423306	124.0
0.8292682926829268	0.8536585365853658	39.0
0.9256965944272446	0.9628482972136223	92.0
1.0244648318042813	1.055045871559633	98.0
0.9279588336192109	0.9965694682675815	138.0
0.94	0.96	53.0
0.9985984583041345	1.0112123335669236	250.0
0.9782608695652174	0.9782608695652174	40.0
0.9356321839080459	1.0229885057471264	112.0
0.9211822660098522	0.9802955665024631	86.0
0.6923076923076923	0.8461538461538461	21.0
1.0	0.8181818181818182	30.0
0.998390989541432	1.0273531777956557	226.0
0.927536231884058	0.9468599033816425	103.0
0.9122401847575058	0.9815242494226328	97.0
0.95822454308094	0.9112271540469974	106.0
0.9488721804511279	0.9759398496240601	140.0
1.0062893081761006	1.0125786163522013	87.0
0.9561290322580646	0.9509677419354838	183.0
0.9656946826758147	0.9725557461406518	139.0
0.9587155963302753	1.0045871559633028	118.0
0.9746835443037974	1.0	41.0
0.9686888454011742	1.0313111545988258	143.0
0.8181818181818182	1.0	15.0
0.8305084745762712	0.9152542372881356	57.0
1.0090702947845804	1.0272108843537415	113.0
1.0309278350515463	1.0206185567010309	45.0
0.9230769230769231	0.9038461538461539	107.0
0.8908045977011494	0.8735632183908046	88.0
0.8666666666666667	0.9333333333333333	34.0
0.9665442676458589	0.9787841697266422	352.0
1.0016611295681064	0.9933554817275747	247.0
0.9231664726426076	0.9557625145518044	158.0
0.6666666666666666	0.8333333333333334	20.0
0.9560439560439561	0.8901098901098901	23.0
0.9523809523809523	0.9761904761904762	122.0
1.0	1.0	10.0
0.8461538461538461	0.8461538461538461	18.0
0.9629005059021922	1.0101180438448567	146.0
1.0	1.0	6.0
0.954070981210856	0.9624217118997912	127.0
0.9540636042402827	1.028268551236749	107.0
0.9120095124851367	0.9690844233055886	189.0
1.0368098159509203	1.0368098159509203	42.0
0.9471228615863142	0.9657853810264385	167.0
0.9923175416133163	0.9667093469910372	133.0
1.0182648401826484	1.0882800608828007	140.0
0.9	1.0	52.0
0.9446640316205533	0.9881422924901185	103.0
0.9841688654353562	0.9718557607739666	203.0
0.9407407407407408	1.0296296296296297	55.0
0.8867924528301887	0.9716981132075472	49.0
0.9670658682634731	1.0119760479041917	143.0
0.9256198347107438	0.9628099173553719	118.0
0.9203539823008849	0.995575221238938	97.0
0.9759562841530055	0.9650273224043716	183.0
0.9344262295081968	0.9344262295081968	22.0
0.9512195121951219	1.146341463414634	38.0
0.9643564356435643	0.9683168316831683	191.0
1.0056657223796035	0.9886685552407932	103.0
0.915625	0.965625	112.0
1.0724637681159421	1.0144927536231885	66.0
0.947242206235012	0.9808153477218226	89.0
0.9604743083003953	1.0158102766798418	252.0
0.9335624284077892	0.9656357388316151	154.0
0.9821029082774049	1.0178970917225951	174.0
0.9841269841269841	1.0132275132275133	156.0
0.9751972942502819	0.9887260428410372	197.0
0.9696969696969697	0.9952153110047847	233.0
0.875	0.8125	38.0
0.9956043956043956	1.0087912087912088	127.0
0.9770114942528736	1.0402298850574712	99.0
0.9656829100892245	0.9629375428963624	245.0
0.9175257731958762	0.9175257731958762	69.0
0.956989247311828	0.9827956989247312	128.0
0.9279588336192109	0.9210977701543739	145.0
0.9590443686006825	0.9726962457337884	120.0
0.9676025917926566	1.0064794816414686	178.0
0.9476861167002012	1.0241448692152917	93.0
0.9907763259031515	0.98923904688701	243.0
0.9627906976744186	0.9627906976744186	122.0
0.957983193277311	0.9411764705882353	59.0
0.8765822784810127	0.930379746835443	112.0
0.9583333333333334	0.9583333333333334	28.0
0.9450867052023122	1.0144508670520231	142.0
0.9311531841652324	0.9483648881239243	121.0
0.8285714285714286	0.8285714285714286	24.0
0.9972862957937585	0.989145183175034	157.0
0.9801980198019802	0.995049504950495	161.0
0.9090909090909091	1.0545454545454545	31.0
0.8735362997658079	0.9484777517564403	108.0
0.8842105263157894	0.9631578947368421	104.0
0.9753086419753086	0.9938271604938271	94.0
0.9644549763033176	1.0071090047393365	122.0
1.0112994350282485	1.0338983050847457	42.0
0.9451612903225807	0.964516129032258	145.0
0.9750623441396509	0.9850374064837906	88.0
1.0	1.011350737797957	190.0
0.8122448979591836	0.9428571428571428	74.0
0.9473684210526315	0.9210526315789473	63.0
1.0	0.9568345323741008	50.0
0.801980198019802	1.0198019801980198	68.0
1.0138169257340242	1.0345423143350605	158.0
0.9636627906976745	1.0406976744186047	240.0
0.9178082191780822	0.9921722113502935	102.0
0.9627039627039627	0.986013986013986	97.0
0.8888888888888888	0.8888888888888888	28.0
0.9069767441860465	0.8604651162790697	36.0
0.9544303797468354	0.9949367088607595	89.0
0.9797979797979798	0.9884559884559885	165.0
1.0	0.9768339768339769	152.0
0.8518518518518519	0.9259259259259259	28.0
1.0	0.9716981132075472	52.0
0.941656942823804	0.9719953325554259	187.0
1.03	1.075	90.0
0.9316239316239316	1.0	60.0
0.4666666666666667	0.8666666666666667	13.0
0.9634146341463414	0.975609756097561	94.0
0.9738863287250384	0.9846390168970814	233.0
0.963531669865643	1.0057581573896353	227.0
1.0	1.0	6.0
1.0125	1.0625	135.0
0.990990990990991	1.009009009009009	152.0
0.7837837837837838	0.7297297297297297	38.0
1.0	1.0	6.0
0.9315789473684211	0.9947368421052631	93.0
0.9032258064516129	0.9935483870967742	85.0
0.9370629370629371	0.986013986013986	63.0
0.9512195121951219	1.048780487804878	36.0
0.9402173913043478	0.9836956521739131	98.0
1.1379310344827587	1.0689655172413792	23.0
0.9975520195838433	0.98531211750306	169.0
0.9304347826086956	1.0	42.0
1.0408163265306123	1.0816326530612246	14.0
0.9685863874345549	0.9738219895287958	79.0
0.9230769230769231	0.9846153846153847	49.0
1.2571428571428571	0.9142857142857143	33.0
1.0	1.2	13.0
0.9659367396593674	0.9708029197080292	109.0
0.8585858585858586	0.9393939393939394	24.0
0.9432098765432099	0.9851851851851852	190.0
0.9478957915831663	0.9959919839679359	111.0
0.9621451104100947	0.9873817034700315	144.0
0.9487179487179487	1.0512820512820513	26.0
0.9333333333333333	0.9	58.0
0.9757085020242915	0.9433198380566802	115.0
0.9750566893424036	0.9705215419501134	198.0
0.979381443298969	0.979381443298969	239.0
0.979002624671916	0.968503937007874	87.0
0.9929947460595446	0.9754816112084063	110.0
0.940959409594096	1.007380073800738	85.0
0.9449225473321858	1.0172117039586919	143.0
0.9090909090909091	0.9318181818181818	134.0
0.926829268292683	0.975609756097561	117.0
0.9440820130475303	0.9869524697110904	186.0
0.9930875576036866	1.0069124423963134	156.0
0.9464285714285714	1.0357142857142858	36.0
0.9712460063897763	0.987220447284345	140.0
0.970856102003643	0.9908925318761385	233.0
0.9755283648498332	1.0244716351501668	161.0
1.0210084033613445	1.0084033613445378	122.0
1.0080645161290323	1.0	57.0
0.8651685393258427	0.8576779026217228	68.0
0.9310344827586207	1.0	37.0
0.9539641943734015	1.0153452685421995	202.0
0.8245614035087719	0.9181286549707602	56.0
1.1333333333333333	1.1333333333333333	8.0
0.9696969696969697	1.018181818181818	74.0
0.9774011299435028	1.0112994350282485	128.0
0.9310344827586207	0.9540229885057471	118.0
1.0	1.0	6.0
1.0	1.0	4.0
0.8760330578512396	0.9669421487603306	39.0
0.9424836601307189	1.0366013071895426	163.0
0.8181818181818182	1.0	14.0
1.0147058823529411	1.0	92.0
0.9210526315789473	1.0789473684210527	20.0
0.9712230215827338	0.9913669064748202	239.0
0.9421841541755889	0.987152034261242	186.0
0.9817470664928292	1.0417209908735332	161.0
0.9370786516853933	1.0	123.0
0.7254901960784313	0.8431372549019608	32.0
0.8709677419354839	0.9354838709677419	24.0
0.951310861423221	0.9438202247191011	142.0
0.9797160243407708	0.9716024340770791	139.0
1.0	1.1142857142857143	22.0
0.9741518578352181	0.9612277867528272	124.0
0.8333333333333334	0.8333333333333334	11.0
0.9730799683293745	1.0190023752969122	245.0
1.0	1.5714285714285714	8.0
0.9460269865067467	1.0	152.0
0.956140350877193	0.9736842105263158	60.0
0.9679358717434869	0.9639278557114228	131.0
0.9387186629526463	0.9805013927576601	108.0
1.0089887640449438	1.002247191011236	216.0
0.8	0.98	30.0
0.9209876543209876	0.9506172839506173	103.0
0.9664670658682635	1.007185628742515	186.0
0.9264	0.9648	129.0
1.0158730158730158	1.0158730158730158	85.0
0.9310344827586207	0.9655172413793104	61.0
1.1666666666666667	1.3333333333333333	18.0
0.8945054945054945	1.0	130.0
1.010126582278481	1.0329113924050632	171.0
0.9670588235294117	1.0015686274509803	237.0
1.0	1.0	14.0
0.9781818181818182	0.9636363636363636	99.0
0.9305019305019305	0.972972972972973	135.0
0.9210526315789473	0.9605263157894737	88.0
0.901840490797546	0.8282208588957055	47.0
0.9802581624905087	1.0197418375094913	244.0
0.8214285714285714	0.8333333333333334	52.0
0.9444444444444444	1.0555555555555556	34.0
0.9252336448598131	0.9626168224299065	113.0
0.9933407325194229	1.0244173140954496	202.0
0.9842271293375394	1.0410094637223974	135.0
0.9875776397515528	1.0248447204968945	177.0
0.9683168316831683	1.0316831683168317	195.0
0.8333333333333334	0.9242424242424242	47.0
1.0	1.0	12.0
0.9669421487603306	1.0082644628099173	85.0
0.9883466860888566	1.0320466132556445	240.0
0.9608433734939759	1.0150602409638554	157.0
0.9286367795059469	0.9505946935041171	191.0
1.1025641025641026	1.0	22.0
0.9701046337817638	0.9880418535127056	147.0
1.0377358490566038	1.070754716981132	116.0
0.9736263736263736	0.9736263736263736	114.0
1.0	0.9804878048780488	84.0
0.9092783505154639	0.9670103092783505	118.0
0.9516129032258065	0.9953917050691244	183.0
0.9884125144843569	1.0231749710312863	151.0
0.9261538461538461	0.9835897435897436	154.0
0.9875518672199171	1.0	105.0
0.9765625	0.953125	51.0
0.9238095238095239	0.9301587301587302	82.0
0.9639810426540284	1.0056872037914693	244.0
0.8746268656716418	0.8686567164179104	86.0
0.9721115537848606	0.9721115537848606	137.0
0.8645833333333334	0.9270833333333334	81.0
0.9012875536480687	0.9399141630901288	108.0
0.9502196193265008	0.95900439238653	160.0
0.9	0.9470588235294117	101.0
1.0301507537688441	1.065326633165829	97.0
0.8706467661691543	0.9701492537313433	65.0
0.8797595190380761	0.935871743486974	130.0
0.92046783625731	0.9742690058479532	148.0
1.0	0.6666666666666666	13.0
1.0093896713615023	1.0093896713615023	53.0
0.9104477611940298	1.044776119402985	69.0
0.9319727891156463	1.054421768707483	39.0
0.9463806970509383	0.9785522788203753	107.0
0.8814814814814815	0.9259259259259259	84.0
0.9628865979381444	0.9711340206185567	113.0
0.9521988527724665	1.0038240917782026	229.0
0.9524348810872028	0.9796149490373726	200.0
0.9605633802816902	0.9774647887323944	91.0
0.9656652360515021	0.9914163090128756	63.0
0.9802197802197802	1.0175824175824175	163.0
0.9382113821138212	0.9447154471544715	120.0
1.0086580086580086	1.0346320346320346	71.0
0.9503105590062112	0.9544513457556936	138.0
0.9940476190476191	0.9880952380952381	98.0
1.064	1.0	43.0
0.9033816425120773	0.9710144927536232	73.0
0.7142857142857143	0.6190476190476191	22.0
0.9917184265010351	0.9544513457556936	112.0
0.9696485623003195	1.0287539936102237	240.0
0.978494623655914	1.0	73.0
0.8927738927738927	0.9533799533799534	95.0
0.9195402298850575	0.9655172413793104	73.0
0.9393939393939394	1.0	103.0
0.9324894514767933	1.0063291139240507	179.0
0.9599383667180277	1.0	142.0
0.8457583547557841	0.8817480719794345	99.0
0.9407407407407408	0.9950617283950617	190.0
0.9691629955947136	0.9911894273127754	115.0
0.9688995215311005	0.992822966507177	176.0
1.012	1.028	118.0
0.975051975051975	1.0332640332640333	133.0
0.9141104294478528	0.9550102249488752	126.0
0.8507462686567164	0.8059701492537313	45.0
1.0613496932515338	1.0245398773006136	53.0
0.9647798742138365	1.0	161.0
0.0	0.0	12.0
0.9815789473684211	1.0078947368421052	115.0
0.8674698795180723	0.9036144578313253	41.0
0.7798165137614679	0.8899082568807339	59.0
0.9115913555992141	0.9449901768172888	166.0
0.8290598290598291	0.8974358974358975	39.0
0.9700374531835206	0.9625468164794008	96.0
0.9536231884057971	0.9884057971014493	79.0
0.9974126778783958	1.0129366106080206	118.0
0.9790849673202614	1.0339869281045753	177.0
0.8888888888888888	1.0	17.0
0.9442231075697212	1.0	121.0
0.9664429530201343	0.9798657718120806	133.0
0.8947368421052632	0.961218836565097	93.0
0.965166908563135	0.9796806966618288	149.0
1.1818181818181819	1.1818181818181819	13.0
0.9686369119420989	1.0	170.0
0.9891156462585035	0.9836734693877551	165.0
1.0	1.0	6.0
0.841688654353562	0.9313984168865436	95.0
1.0	0.968	48.0
0.8918918918918919	0.8918918918918919	94.0
0.9071729957805907	1.0	57.0
0.9559585492227979	1.0025906735751295	159.0
0.9385964912280702	0.956140350877193	62.0
0.9856410256410256	0.9856410256410256	221.0
0.8982188295165394	0.9491094147582697	112.0
0.8311688311688312	0.7922077922077922	51.0
0.9372549019607843	1.007843137254902	64.0
0.983402489626556	1.049792531120332	59.0
0.9680608365019011	1.0136882129277567	232.0
0.9688826025459689	0.9915134370579916	149.0
0.978021978021978	0.9843014128728415	129.0
0.9364161849710982	0.9653179190751445	89.0
1.0325865580448066	1.0325865580448066	104.0
1.0	1.0307692307692307	75.0
0.9820224719101124	0.9730337078651685	115.0
0.8923395445134575	0.9544513457556936	133.0
0.9265536723163842	0.9717514124293786	90.0
0.9883585564610011	0.9813736903376019	199.0
0.9944559944559944	1.0097020097020097	252.0
0.9959919839679359	1.0	141.0
0.8976109215017065	0.9931740614334471	148.0
0.8565022421524664	0.9103139013452914	84.0
0.9358974358974359	0.9487179487179487	123.0
0.9806094182825484	0.997229916897507	147.0
0.8695652173913043	0.8913043478260869	62.0
0.9198396793587175	0.9779559118236473	162.0
0.9253333333333333	0.9466666666666667	171.0
0.9558823529411765	0.9754901960784313	97.0
0.935064935064935	0.961038961038961	113.0
0.9404255319148936	0.948936170212766	141.0
0.9626168224299065	0.9813084112149533	168.0
1.0	1.0494791666666667	130.0
0.9817073170731707	0.9786585365853658	127.0
1.0	1.0	8.0
0.8646616541353384	0.924812030075188	57.0
0.9310344827586207	0.9408866995073891	40.0
0.9396984924623115	0.9824120603015075	184.0
1.0059701492537314	1.0328358208955224	164.0
0.9269183922046285	1.0121802679658953	165.0
0.8454106280193237	0.9130434782608695	56.0
0.9489795918367347	1.030612244897959	86.0
0.971342383107089	1.0060331825037707	240.0
0.9436008676789588	1.017353579175705	109.0
1.0045402951191829	1.006810442678774	215.0
0.8947368421052632	0.868421052631579	25.0
1.0606060606060606	1.1818181818181819	25.0
0.9590909090909091	1.0	201.0
0.982414068745004	1.017585931254996	237.0
0.9943100995732574	1.0256045519203414	156.0
1.0	1.0302171860245515	217.0
0.9400749063670412	0.9775280898876404	91.0
0.9419191919191919	0.98989898989899	185.0
0.9562043795620438	1.0145985401459854	103.0
1.0128102481985588	1.022417934347478	244.0
0.996551724137931	1.0379310344827586	124.0
2.3333333333333335	2.3333333333333335	5.0
0.9683544303797469	1.0031645569620253	142.0
0.8620689655172413	0.6551724137931034	16.0
0.9868995633187773	0.9912663755458515	121.0
0.9681528662420382	1.017515923566879	247.0
1.0256410256410255	1.054945054945055	149.0
1.0	1.0	12.0
1.5	1.5	8.0
0.9111111111111111	0.7777777777777778	47.0
0.9934138309549945	1.0065861690450055	176.0
0.9710669077757685	1.0	149.0
1.0909090909090908	1.2727272727272727	13.0
0.9530026109660574	0.95822454308094	116.0
0.8	0.8	14.0
0.9817813765182186	0.9959514170040485	127.0
0.9047619047619048	0.9523809523809523	19.0
0.9927536231884058	0.9855072463768116	127.0
1.0	1.03125	22.0
0.9564032697547684	0.9564032697547684	80.0
0.9599198396793587	0.9679358717434869	119.0
0.9707317073170731	1.0195121951219512	54.0
0.9676232523914643	1.0014716703458426	231.0
0.9539473684210527	1.013157894736842	65.0
0.9477124183006536	1.0	110.0
0.9544592030360531	0.9772296015180265	135.0
0.9449901768172888	1.0078585461689586	125.0
0.8181818181818182	0.8181818181818182	16.0
0.9881481481481481	1.002962962962963	165.0
0.9537815126050421	0.9831932773109243	111.0
1.0118694362017804	1.0118694362017804	94.0
1.013840830449827	1.0346020761245676	164.0
0.8709677419354839	0.967741935483871	25.0
0.8163265306122449	0.9183673469387755	34.0
0.896969696969697	0.9787878787878788	139.0
0.9389140271493213	0.9932126696832579	132.0
0.9461538461538461	1.0	67.0
0.7142857142857143	0.7142857142857143	19.0
1.0	1.0	9.0
0.954337899543379	1.0114155251141552	200.0
0.9870550161812298	0.9741100323624595	89.0
0.9145907473309609	1.0	97.0
0.9912280701754386	1.0175438596491229	191.0
0.9620853080568721	1.028436018957346	53.0
1.0105263157894737	0.9578947368421052	53.0
0.7452229299363057	0.9363057324840764	36.0
1.0	1.0	7.0
1.0154142581888246	0.9884393063583815	121.0
0.9368421052631579	0.9326315789473684	131.0
0.986013986013986	1.0	107.0
0.9295154185022027	0.947136563876652	63.0
0.9082969432314411	1.0218340611353711	123.0
1.003883495145631	1.0737864077669903	107.0
0.9137380191693291	0.9744408945686901	157.0
0.9446153846153846	0.9507692307692308	90.0
0.953757225433526	0.9653179190751445	103.0
0.964	0.936	122.0
0.922077922077922	1.0	48.0
0.9924050632911392	1.0050632911392405	162.0
1.0239234449760766	1.0526315789473684	118.0
0.9641025641025641	0.9692307692307692	88.0
0.9578163771712159	0.9851116625310173	171.0
1.0032414910858996	1.0713128038897892	117.0
0.8554216867469879	0.8554216867469879	38.0
0.933649289099526	0.981042654028436	70.0
1.0129198966408268	1.049095607235142	159.0
0.875	0.9166666666666666	29.0
0.898989898989899	0.8383838383838383	34.0
0.9701492537313433	1.0298507462686568	43.0
1.0740740740740742	1.1481481481481481	19.0
1.0050377833753148	1.0629722921914357	121.0
0.9851714550509731	1.0018535681186285	226.0
1.0418848167539267	1.0157068062827226	99.0
0.9957446808510638	1.0297872340425531	112.0
0.9534450651769087	0.9925512104283054	220.0
0.9672131147540983	0.9344262295081968	43.0
0.9695431472081218	0.9661590524534687	148.0
1.033167495854063	0.9767827529021559	130.0
0.8853503184713376	0.9235668789808917	49.0
1.0024844720496895	1.0372670807453417	119.0
0.8888888888888888	0.8148148148148148	36.0
0.9565217391304348	1.0434782608695652	64.0
0.976545842217484	0.997867803837953	175.0
1.1261261261261262	1.1261261261261262	49.0
0.9501557632398754	0.9875389408099688	145.0
0.9012345679012346	0.9506172839506173	22.0
1.2222222222222223	1.4444444444444444	14.0
1.105263157894737	1.0382775119617225	53.0
1.0	1.0	5.0
0.9693654266958425	1.0043763676148796	110.0
0.9177377892030848	0.9280205655526992	105.0
0.9849056603773585	0.9886792452830189	192.0
0.9646017699115044	1.0265486725663717	66.0
0.9487179487179487	0.9230769230769231	49.0
0.9632352941176471	1.0098039215686274	170.0
0.8947368421052632	1.0150375939849625	57.0
0.8960396039603961	1.0	94.0
0.8781163434903048	0.9279778393351801	94.0
0.9587878787878787	1.0	169.0
0.8620689655172413	1.0	22.0
0.990990990990991	1.0202702702702702	203.0
1.0073260073260073	1.0146520146520146	90.0
0.8518518518518519	1.0740740740740742	22.0
0.9729064039408867	0.9901477832512315	176.0
0.9864559819413092	1.0135440180586908	120.0
0.9115281501340483	0.9410187667560321	116.0
1.0857142857142856	1.1	63.0
0.9644670050761421	0.9822335025380711	182.0
0.9885714285714285	1.0571428571428572	50.0
0.9577464788732394	0.9859154929577465	119.0
0.9629927594529365	0.9935639581657281	241.0
0.9815590947191953	1.0184409052808048	206.0
0.9967611336032388	1.0064777327935224	220.0
0.9657142857142857	0.9885714285714285	56.0
1.0024721878862795	1.0321384425216316	126.0
0.9736263736263736	0.9736263736263736	119.0
0.9069767441860465	0.9534883720930233	75.0
0.971875	0.984375	153.0
0.9705882352941176	0.9640522875816994	140.0
0.9767441860465116	0.9488372093023256	112.0
0.9800613496932515	1.0122699386503067	244.0
0.9722108704536166	0.9844707805476093	356.0
0.9649122807017544	0.9122807017543859	42.0
1.027027027027027	0.9864864864864865	47.0
0.9600570613409415	1.0114122681883024	150.0
1.0	1.0666666666666667	31.0
0.9448698315467075	0.9693721286370597	140.0
0.9502487562189055	0.9601990049751243	51.0
0.9333333333333333	0.6	12.0
0.9798994974874372	1.0603015075376885	48.0
0.955719557195572	0.992619926199262	191.0
1.0336134453781514	1.0672268907563025	39.0
1.0	1.0	5.0
0.9380530973451328	0.9778761061946902	141.0
0.9766718506998445	0.995334370139969	249.0
0.9913793103448276	1.0603448275862069	37.0
0.95	0.9333333333333333	34.0
1.0	1.0	15.0
1.047197640117994	1.064896755162242	90.0
1.028397565922921	1.0121703853955375	120.0
0.986644407345576	0.9732888146911519	117.0
0.9541984732824428	0.9541984732824428	40.0
0.8962264150943396	0.9150943396226415	65.0
1.0076045627376427	1.0329531051964511	167.0
0.9532846715328467	0.9708029197080292	155.0
0.9792099792099792	1.004158004158004	128.0
0.9775280898876404	1.0074906367041199	171.0
0.9695652173913043	0.9869565217391304	108.0
0.9491525423728814	0.9491525423728814	76.0
1.0	1.0	6.0
0.9832602630530092	1.0199282582702272	357.0
1.0	0.5555555555555556	18.0
0.9736842105263158	0.9962406015037594	109.0
0.964221824686941	0.9928443649373881	116.0
0.9486238532110092	0.9963302752293578	137.0
0.9388235294117647	1.0847058823529412	100.0
0.9924050632911392	1.0	166.0
1.0063291139240507	1.0316455696202531	86.0
1.0	0.9523809523809523	27.0
1.0051948051948052	1.0285714285714285	116.0
0.9876543209876543	1.0354938271604939	229.0
0.9872611464968153	1.0	113.0
0.946524064171123	1.0213903743315509	48.0
0.9886039886039886	0.9886039886039886	82.0
1.0	0.9922480620155039	87.0
0.9259259259259259	1.1481481481481481	20.0
0.9558282208588957	0.9901840490797545	129.0
0.7560975609756098	0.7560975609756098	31.0
0.8728813559322034	0.9830508474576272	65.0
0.9492753623188406	0.9879227053140096	190.0
0.9698239731768651	0.9798826487845766	203.0
1.0	1.0341614906832297	140.0
0.8566037735849057	0.9622641509433962	84.0
1.0623052959501558	1.0934579439252337	80.0
1.0094117647058825	1.0611764705882354	104.0
0.9681978798586572	0.9823321554770318	108.0
0.9285714285714286	0.8809523809523809	49.0
0.9	1.0833333333333333	40.0
0.9578651685393258	0.9915730337078652	148.0
0.8787878787878788	1.0606060606060606	22.0
0.9322533136966127	0.9911634756995582	144.0
0.9530201342281879	1.0134228187919463	71.0
0.9589442815249267	0.9706744868035191	97.0
0.9911504424778761	1.0353982300884956	106.0
0.9557522123893806	0.9601769911504425	115.0
0.9808087731322824	1.0150788211103496	247.0
0.9802955665024631	0.9605911330049262	70.0
0.8716577540106952	0.8609625668449198	80.0
1.0	1.0	27.0
1.0211640211640212	0.9153439153439153	41.0
0.926829268292683	1.0406504065040652	88.0
1.0	1.0	9.0
1.0107962213225372	1.0242914979757085	147.0
0.8411552346570397	0.9061371841155235	91.0
0.9684647302904564	0.9933609958506224	204.0
1.0363636363636364	1.0545454545454545	50.0
0.9380952380952381	0.9619047619047619	90.0
0.8823529411764706	0.8823529411764706	18.0
0.9823529411764705	1.0127450980392156	320.0
0.9898255813953488	1.0377906976744187	241.0
0.9927536231884058	1.0253623188405796	132.0
0.8410041841004184	0.9497907949790795	77.0
0.8676470588235294	0.9558823529411765	45.0
0.9491525423728814	1.0	60.0
0.9663865546218487	0.9831932773109243	30.0
0.9689655172413794	0.9724137931034482	150.0
1.028436018957346	1.04739336492891	61.0
0.9333333333333333	0.9333333333333333	26.0
0.9813302217036173	0.9953325554259043	167.0
0.9948586118251928	1.025706940874036	121.0
0.9889908256880734	1.0091743119266054	224.0
0.9461077844311377	0.9880239520958084	83.0
0.8879310344827587	0.9396551724137931	104.0
1.5	1.5	6.0
0.9708222811671088	1.0079575596816976	162.0
1.0438356164383562	1.0547945205479452	103.0
0.8901098901098901	1.021978021978022	30.0
0.9697802197802198	0.9945054945054945	131.0
0.9347079037800687	0.9484536082474226	139.0
0.9853747714808044	0.9890310786106032	242.0
0.7916666666666666	0.8333333333333334	33.0
0.8717948717948718	0.9487179487179487	78.0
0.9439906651108518	1.0116686114352391	155.0
0.9628252788104089	0.990086741016109	205.0
0.9418803418803419	0.9863247863247864	130.0
0.8102189781021898	0.8978102189781022	58.0
0.9627749576988156	1.0101522842639594	118.0
0.8181818181818182	0.948051948051948	54.0
0.9774266365688488	1.0225733634311513	204.0
0.9555555555555556	0.9185185185185185	76.0
1.0213219616204692	1.0255863539445629	106.0
0.960880195599022	0.980440097799511	101.0
0.9545454545454546	1.0075757575757576	66.0
1.0748299319727892	1.054421768707483	74.0
0.9628040057224606	0.9971387696709585	190.0
0.9166666666666666	1.0	22.0
1.003125	1.0171875	241.0
0.9471947194719472	1.023102310231023	126.0
0.9791304347826087	0.9686956521739131	104.0
1.0023148148148149	1.025462962962963	150.0
0.9223744292237442	0.9908675799086758	109.0
0.972027972027972	1.013986013986014	38.0
0.92	0.92	24.0
0.9879518072289156	1.0120481927710843	220.0
0.9911971830985915	1.0211267605633803	195.0
1.0	1.0	9.0
0.9767981438515081	1.0278422273781902	98.0
0.9844961240310077	1.0	67.0
0.9893617021276596	1.0151975683890577	229.0
0.9444444444444444	0.9673202614379085	157.0
0.9148936170212766	0.9513677811550152	82.0
0.95	0.9818181818181818	95.0
0.974025974025974	1.077922077922078	28.0
0.8947368421052632	1.0175438596491229	35.0
0.9771754636233951	0.9771754636233951	150.0
1.0	1.054945054945055	51.0
0.9352380952380952	0.9809523809523809	124.0
0.956989247311828	1.086021505376344	53.0
0.7590361445783133	0.9156626506024096	43.0
0.9206349206349206	0.9206349206349206	42.0
0.9947229551451188	0.9736147757255936	90.0
0.9975816203143894	1.0386940749697702	170.0
1.0180831826401446	1.0180831826401446	110.0
1.0755667506297228	1.0302267002518892	93.0
0.972027972027972	0.9766899766899767	108.0
0.9497142857142857	0.9817142857142858	194.0
1.0	1.0	9.0
0.7857142857142857	0.9285714285714286	15.0
0.9840255591054313	1.0047923322683705	244.0
0.9352941176470588	0.9088235294117647	120.0
0.9798387096774194	0.9919354838709677	140.0
0.9772727272727273	0.9772727272727273	172.0
0.9568345323741008	1.0215827338129497	80.0
0.9894179894179894	0.9894179894179894	67.0
1.0	1.1176470588235294	16.0
0.958041958041958	0.986013986013986	117.0
0.9603174603174603	0.9920634920634921	128.0
0.9847328244274809	0.9083969465648855	58.0
0.9775280898876404	1.0224719101123596	52.0
0.9262672811059908	0.9447004608294931	96.0
1.0	0.9907407407407407	84.0
0.9512195121951219	1.1951219512195121	49.0
0.9651567944250871	0.967479674796748	173.0
0.937888198757764	0.979296066252588	113.0
1.0892857142857142	1.0714285714285714	42.0
0.6	0.6	13.0
0.9662337662337662	1.0077922077922077	179.0
0.8181818181818182	0.8585858585858586	28.0
1.4	1.4	10.0
0.8802992518703242	0.9451371571072319	110.0
0.9489795918367347	0.9489795918367347	35.0
1.0	1.0	7.0
0.8133333333333334	0.8666666666666667	51.0
0.9799749687108886	1.0050062578222778	167.0
0.9520958083832335	1.0079840319361277	120.0
0.9652173913043478	1.0024844720496895	187.0
0.9590316573556797	0.9739292364990689	213.0
1.0	1.0	10.0
0.9921073401736386	1.0552486187845305	236.0
0.8817204301075269	0.8602150537634409	68.0
1.0	1.0	1.0
0.9848975188781014	0.9978425026968716	134.0
0.9927797833935018	1.0469314079422383	121.0
0.9925925925925926	1.037037037037037	87.0
0.9660297239915074	1.0212314225053079	132.0
0.9723502304147466	0.9585253456221198	101.0
0.8648648648648649	0.972972972972973	64.0
0.9464720194647201	0.9318734793187348	100.0
1.0326975476839237	1.0463215258855585	162.0
0.9657631954350927	1.0085592011412268	169.0
0.8305084745762712	0.9096045197740112	88.0
0.9	0.9555555555555556	63.0
0.9305210918114144	0.9702233250620348	93.0
0.9797979797979798	0.9797979797979798	230.0
1.011881188118812	1.0792079207920793	126.0
1.0301507537688441	0.9949748743718593	93.0
0.9587020648967551	1.0353982300884956	151.0
0.9131483715319663	0.9372738238841978	153.0
0.9538784067085954	0.9664570230607966	134.0
1.0	1.003062787136294	121.0
0.9927272727272727	1.029090909090909	146.0
0.9881364310430054	1.0533860603064755	320.0
0.9599578503688093	0.9957850368809273	156.0
0.6923076923076923	0.6923076923076923	13.0
0.9548306148055207	0.9698870765370138	183.0
0.9773371104815864	0.9905571293673276	243.0
0.9379407616361072	1.002820874471086	151.0
0.9494163424124513	0.9883268482490273	128.0
0.8675496688741722	0.8278145695364238	51.0
0.9779353821907013	1.0	240.0
0.7878787878787878	1.0303030303030303	24.0
0.9330143540669856	0.9425837320574163	92.0
0.898989898989899	0.9393939393939394	46.0
0.9551886792452831	1.0070754716981132	170.0
0.9775280898876404	0.9775280898876404	47.0
0.9693165969316597	1.00278940027894	156.0
0.9254658385093167	1.0124223602484472	50.0
0.8804597701149425	0.9172413793103448	111.0
0.9292701279157262	0.9939804364183596	203.0
0.9875130072840791	1.0228928199791882	172.0
0.9595959595959596	0.9966329966329966	144.0
0.900497512437811	0.9303482587064676	64.0
1.0045045045045045	0.990990990990991	99.0
0.9469387755102041	0.9959183673469387	113.0
0.9922879177377892	1.0154241645244215	96.0
1.0091954022988505	1.0298850574712644	127.0
0.7936507936507936	0.9841269841269841	39.0
0.9751861042183623	0.9900744416873449	90.0
0.936	0.9413333333333334	103.0
0.9230769230769231	0.9615384615384616	91.0
0.9233449477351916	0.9442508710801394	150.0
0.9116022099447514	0.9005524861878453	58.0
0.9952718676122931	1.0472813238770686	108.0
0.9628378378378378	0.9932432432432432	147.0
0.9634369287020109	0.9744058500914077	114.0
0.9747292418772563	0.9711191335740073	115.0
0.9413333333333334	1.0053333333333334	101.0
1.0	1.0	11.0
0.9785604900459418	1.006125574272588	114.0
0.8961038961038961	0.987012987012987	59.0
0.9615384615384616	0.8974358974358975	47.0
0.9877551020408163	1.0285714285714285	113.0
0.8571428571428571	0.8809523809523809	21.0
0.8888888888888888	0.9074074074074074	47.0
0.983640081799591	0.9795501022494888	131.0
0.9880546075085325	0.9914675767918089	210.0
0.9133574007220217	0.9530685920577617	135.0
0.9336099585062241	0.9585062240663901	62.0
1.0	1.0502793296089385	83.0
0.8473282442748091	0.9083969465648855	61.0
0.9631205673758865	1.0312056737588653	165.0
1.0285035629453683	1.0593824228028503	140.0
0.9	0.9583333333333334	48.0
0.9027237354085603	1.0077821011673151	109.0
0.9203980099502488	0.9369817578772802	160.0
0.875	0.875	30.0
1.0	0.9656357388316151	88.0
0.9672131147540983	1.0081967213114753	89.0
1.0	1.0	13.0
0.9961389961389961	1.0154440154440154	133.0
0.875	0.875	23.0
0.9637243047158404	0.992744860943168	164.0
0.9661016949152542	0.9661016949152542	36.0
1.010958904109589	0.9726027397260274	80.0
0.9822222222222222	0.9422222222222222	119.0
0.975609756097561	0.9786585365853658	152.0
1.0	1.0	8.0
0.958904109589041	0.9863013698630136	123.0
1.0	1.2222222222222223	13.0
0.7795275590551181	0.9212598425196851	46.0
0.9629629629629629	0.9629629629629629	82.0
1.0	1.007936507936508	127.0
0.9097387173396675	1.004750593824228	93.0
0.9687174139728885	1.018769551616267	167.0
0.9395465994962217	0.9622166246851386	189.0
0.8823529411764706	0.7983193277310925	26.0
0.8662420382165605	0.9745222929936306	84.0
0.9753086419753086	1.0049382716049382	93.0
0.9851851851851852	1.0	47.0
0.9134615384615384	0.8365384615384616	39.0
0.976401179941003	1.0	164.0
0.8021978021978022	0.7802197802197802	26.0
0.8235294117647058	1.0	18.0
0.8160919540229885	0.9310344827586207	54.0
0.9660056657223796	0.9773371104815864	79.0
1.005449591280654	1.0708446866485013	104.0
0.9950556242274413	1.0222496909765142	171.0
0.9652605459057072	0.9801488833746899	129.0
0.9847638395124428	1.026409344845099	309.0
1.6666666666666667	1.0	4.0
0.9839034205231388	0.9637826961770624	131.0
1.0	0.9358974358974359	96.0
0.9887459807073955	1.0209003215434083	244.0
0.9716494845360825	0.9664948453608248	163.0
0.9090909090909091	1.0	25.0
0.94375	0.9895833333333334	165.0
1.0	1.0315789473684212	161.0
0.9440559440559441	1.0186480186480187	103.0
0.9904306220095693	1.0334928229665072	113.0
0.8805970149253731	0.8805970149253731	57.0
0.9379042690815006	1.0258732212160413	174.0
0.9967689822294022	1.0323101777059773	143.0
0.9795918367346939	0.9846938775510204	164.0
0.84	1.0	25.0
0.9861751152073732	1.0092165898617511	130.0
1.0509554140127388	1.0382165605095541	79.0
0.8815489749430524	0.8724373576309795	109.0
0.958041958041958	1.017982017982018	163.0
1.0165562913907285	1.0695364238410596	113.0
0.9737991266375546	0.9934497816593887	213.0
0.9977064220183486	1.0298165137614679	176.0
1.0	1.0	6.0
1.6	1.2	2.0
0.6363636363636364	0.9090909090909091	20.0
0.9977703455964325	1.0178372352285396	195.0
0.9507186858316222	1.0082135523613962	133.0
0.9902755267423015	1.032414910858995	139.0
1.0042194092827004	1.0084388185654007	102.0
1.0235081374321882	1.0379746835443038	230.0
0.9491916859122402	1.046189376443418	87.0
0.8	0.9	20.0
1.007843137254902	1.0705882352941176	59.0
0.9767441860465116	1.0155038759689923	151.0
0.9572368421052632	1.019736842105263	136.0
0.9315068493150684	0.9315068493150684	37.0
0.9385113268608414	0.9805825242718447	129.0
0.9714285714285714	0.9142857142857143	58.0
0.9880597014925373	1.0298507462686568	145.0
0.9836808703535811	1.0199456029011786	220.0
0.881104033970276	0.9490445859872612	108.0
0.9305555555555556	0.9583333333333334	89.0
0.9890510948905109	1.0	111.0
2.0	1.0	5.0
0.9545454545454546	1.0340909090909092	102.0
0.9404761904761905	0.9404761904761905	78.0
0.9395604395604396	0.9615384615384616	108.0
0.8952879581151832	0.9476439790575916	61.0
0.97	1.0	153.0
0.96996996996997	0.993993993993994	86.0
0.9639097744360903	0.9939849624060151	186.0
1.077922077922078	0.948051948051948	28.0
0.9285714285714286	1.0	46.0
0.8917647058823529	0.9576470588235294	112.0
0.9402560455192034	0.9857752489331437	188.0
0.9101654846335697	0.9290780141843972	90.0
1.0057971014492753	1.0231884057971015	96.0
0.9576271186440678	0.9957627118644068	164.0
0.9738317757009346	0.9962616822429906	118.0
0.9701492537313433	0.9751243781094527	92.0
0.9921414538310412	1.0039292730844793	145.0
0.9772727272727273	0.9954545454545455	97.0
1.024390243902439	1.0	34.0
0.9506172839506173	1.0339506172839505	113.0
0.8951612903225806	0.9112903225806451	71.0
0.9744318181818182	1.0113636363636365	168.0
0.9419795221843004	1.0	159.0
0.9607201309328969	0.9705400981996727	159.0
0.9982456140350877	1.0333333333333334	201.0
0.9418803418803419	0.9418803418803419	111.0
0.8125	0.875	39.0
1.0095846645367412	1.02555910543131	137.0
0.813953488372093	1.0	17.0
0.9582753824756607	0.9777468706536857	172.0
0.9841966637401229	0.9964881474978051	196.0
1.0	1.0	5.0
0.8571428571428571	1.0	19.0
0.9540229885057471	1.0204342273307792	160.0
0.9456943366951125	1.021722265321955	239.0
0.92	0.84	18.0
1.1578947368421053	1.131578947368421	37.0
1.206896551724138	1.2758620689655173	22.0
1.0178571428571428	1.0178571428571428	30.0
0.9648682559598495	0.9874529485570891	188.0
0.9619771863117871	0.9885931558935361	140.0
0.8064516129032258	1.064516129032258	21.0
1.005	1.0175	126.0
0.9259259259259259	0.8518518518518519	25.0
0.92914653784219	1.003220611916264	160.0
1.0	1.25	20.0
1.0093896713615023	1.056338028169014	130.0
0.9730458221024259	1.0161725067385445	91.0
0.9549295774647887	0.9661971830985916	110.0
0.9722222222222222	0.9965277777777778	124.0
0.9550561797752809	0.9730337078651685	123.0
0.963963963963964	1.0	22.0
0.9631147540983607	0.9877049180327869	128.0
0.9622641509433962	0.9547169811320755	60.0
1.0	1.0	5.0
1.0092592592592593	0.9814814814814815	50.0
0.9226804123711341	1.0309278350515463	86.0
0.9166666666666666	0.9318181818181818	86.0
0.9585062240663901	0.9087136929460581	64.0
1.0133333333333334	1.02	68.0
1.08	1.08	35.0
0.968503937007874	1.031496062992126	102.0
1.0211267605633803	1.0211267605633803	91.0
0.96	0.92	37.0
0.9215686274509803	0.9738562091503268	36.0
0.9813084112149533	1.0327102803738317	112.0
0.9612334801762115	0.9647577092511013	199.0
0.8888888888888888	1.0833333333333333	29.0
0.9400544959128065	0.9673024523160763	174.0
0.988	1.0	125.0
0.9448275862068966	0.9172413793103448	67.0
0.948051948051948	0.9792207792207792	110.0
0.9090909090909091	0.8181818181818182	34.0
0.9516908212560387	1.0	142.0
0.9563492063492064	0.9722222222222222	141.0
0.8925831202046036	0.907928388746803	88.0
1.0168067226890756	1.0605042016806723	105.0
0.9444444444444444	0.9967320261437909	125.0
0.9054945054945055	0.9868131868131869	161.0
0.99375	1.003125	136.0
1.0	1.0	11.0
0.9170506912442397	1.055299539170507	86.0
1.0130081300813008	1.0	135.0
0.965034965034965	0.951048951048951	90.0
0.9769526248399488	1.030729833546735	169.0
1.078740157480315	1.062992125984252	64.0
0.9051724137931034	0.9396551724137931	76.0
1.0	1.2857142857142858	9.0
0.9368421052631579	0.8526315789473684	30.0
0.9251769464105156	0.9838220424671386	168.0
0.9463414634146341	0.9878048780487805	151.0
0.9617444529456771	0.9892884468247896	223.0
0.967741935483871	1.017921146953405	128.0
0.937007874015748	0.9763779527559056	122.0
0.0	0.0	9.0
0.9595959595959596	0.9942279942279942	157.0
0.9203640500568828	0.9726962457337884	155.0
0.9631901840490797	1.049079754601227	42.0
1.25	1.375	14.0
1.0175438596491229	1.1578947368421053	35.0
0.8769230769230769	0.8769230769230769	43.0
1.0	1.0	7.0
0.9634146341463414	1.0	41.0
0.9630996309963099	0.997539975399754	174.0
1.1111111111111112	1.1111111111111112	20.0
0.8963730569948186	0.927461139896373	87.0
0.9636363636363636	1.004040404040404	129.0
0.904	0.952	63.0
0.9712230215827338	0.9712230215827338	89.0
0.9616788321167883	1.0036496350364963	221.0
0.9047619047619048	1.0634920634920635	19.0
1.0106870229007634	1.0183206106870228	248.0
0.8181818181818182	0.7636363636363637	24.0
0.9176954732510288	0.934156378600823	118.0
0.9571428571428572	1.042857142857143	89.0
0.9307359307359307	0.9653679653679653	120.0
0.9498861047835991	1.0136674259681093	124.0
0.9968152866242038	1.0063694267515924	144.0
0.8695652173913043	1.0869565217391304	17.0
0.9912280701754386	1.0321637426900585	166.0
0.9376083188908145	0.9826689774696707	116.0
1.0389610389610389	1.0129870129870129	51.0
0.9185750636132316	0.9440203562340967	96.0
0.9711934156378601	1.0411522633744856	138.0
1.004524886877828	1.0497737556561086	119.0
1.0162932790224033	1.0040733197556009	142.0
0.92	0.92	13.0
0.9676214196762142	0.9900373599003736	173.0
0.9691714836223507	0.9845857418111753	132.0
0.9699074074074074	1.0208333333333333	129.0
1.0	1.0222222222222221	129.0
0.9409282700421941	1.0084388185654007	62.0
0.9973753280839895	1.0	164.0
0.9891388673390225	1.0418929402637704	232.0
1.0357142857142858	0.9857142857142858	80.0
1.003088803088803	1.0200772200772201	232.0
0.9441860465116279	0.9534883720930233	69.0
0.9422680412371134	0.9711340206185567	124.0
0.9824175824175824	1.0043956043956044	123.0
0.7948717948717948	0.7948717948717948	38.0
0.9878048780487805	1.0317073170731708	193.0
0.8285714285714286	1.0	18.0
0.995575221238938	1.0	125.0
0.8	0.6	18.0
0.9936	1.032	109.0
0.9488888888888889	0.9888888888888889	195.0
1.0200400801603207	1.0080160320641283	122.0
0.9584415584415584	0.974025974025974	85.0
0.9615384615384616	0.9846153846153847	121.0
1.0098119378577268	1.0179885527391659	235.0


==> nbpDA_praline-package-2020-05-18.tex <==
bfs/rand	fd/rand	vtcs
1.0265339966832505	1.0265339966832505	114.0
1.0553691275167785	0.9899328859060402	237.0
1.0516129032258064	1.0516129032258064	54.0
0.9866962305986696	0.9290465631929047	123.0
0.9319727891156463	0.9183673469387755	67.0
0.9207920792079208	0.8811881188118812	40.0
0.9791976225854383	0.9405646359583952	190.0
0.9130434782608695	0.9565217391304348	122.0
0.9310344827586207	0.89272030651341	70.0
0.980806142034549	0.8809980806142035	135.0
0.9709677419354839	0.9532258064516129	244.0
1.0214067278287462	1.0091743119266054	169.0
0.9022988505747126	0.9137931034482759	110.0
0.9602649006622517	0.9690949227373068	121.0
1.0588235294117647	1.0	31.0
1.0930232558139534	1.0	15.0
1.0695652173913044	0.9188405797101449	93.0
1.0	1.0	8.0
0.5294117647058824	0.5294117647058824	21.0
0.9859943977591037	0.9607843137254902	168.0
0.9365671641791045	0.8507462686567164	133.0
0.9964349376114082	0.9857397504456328	145.0
0.9574970484061394	0.9622195985832349	149.0
1.022944550669216	0.9923518164435946	147.0
0.9701492537313433	0.9850746268656716	60.0
0.9320388349514563	0.9563106796116505	91.0
0.9145299145299145	0.8803418803418803	102.0
0.9915611814345991	1.0084388185654007	134.0
0.6666666666666666	0.6666666666666666	13.0
1.1081081081081081	1.027027027027027	24.0
0.9528535980148883	0.8957816377171216	153.0
0.963302752293578	0.9571865443425076	86.0
0.9655172413793104	0.9283819628647215	164.0
0.9692982456140351	0.9473684210526315	134.0
1.12	1.08	31.0
0.9794344473007712	0.9125964010282777	100.0
0.973397823458283	0.9492140266021766	186.0
1.0	1.0	8.0
0.8181818181818182	0.7954545454545454	47.0
0.9930555555555556	1.0	139.0
1.0147492625368733	0.9572271386430679	241.0
1.1304347826086956	0.9652173913043478	58.0
0.9816933638443935	0.9588100686498856	122.0
1.0053691275167784	0.9865771812080537	169.0
0.9585062240663901	0.9087136929460581	126.0
0.9528907922912205	0.9271948608137045	120.0
0.9719298245614035	0.9087719298245615	138.0
0.972318339100346	1.027681660899654	144.0
0.9090909090909091	0.9282296650717703	102.0
0.8826979472140762	0.8826979472140762	109.0
0.8181818181818182	0.8181818181818182	14.0
1.0531697341513293	1.0449897750511248	133.0
0.8856088560885609	0.8302583025830258	113.0
0.7058823529411765	0.7647058823529411	32.0
0.9851116625310173	0.9387923904052936	241.0
0.9213973799126638	0.8995633187772926	105.0
0.9726027397260274	0.8873668188736682	159.0
0.9259259259259259	0.873015873015873	107.0
0.9688796680497925	0.983402489626556	194.0
0.9276315789473685	0.8289473684210527	99.0
0.8924731182795699	0.8494623655913979	60.0
0.9384615384615385	0.9230769230769231	76.0
0.9541984732824428	0.9491094147582697	92.0
0.9282296650717703	0.9186602870813397	97.0
0.8852459016393442	0.9672131147540983	47.0
0.7142857142857143	0.7142857142857143	10.0
1.0134408602150538	0.9946236559139785	164.0
1.0349854227405249	0.9620991253644315	168.0
0.9681093394077449	0.9635535307517085	115.0
0.8683127572016461	0.9012345679012346	63.0
1.0186915887850467	0.9626168224299065	80.0
1.0099091659785302	0.9834847233691164	234.0
0.9459459459459459	0.9213759213759214	119.0
0.9619565217391305	0.9239130434782609	107.0
0.9938271604938271	0.9876543209876543	165.0
1.0	0.9259259259259259	21.0
0.9829787234042553	0.9914893617021276	117.0
0.9736842105263158	0.9526315789473684	97.0
1.0683229813664596	0.9627329192546584	82.0
0.8997050147492626	0.9174041297935103	98.0
0.8793103448275862	0.8275862068965517	40.0
1.0310077519379846	0.9844961240310077	154.0
0.9178082191780822	0.863013698630137	27.0
0.9171597633136095	0.9053254437869822	115.0
1.1071428571428572	1.1071428571428572	49.0
0.0	0.0	7.0
0.883289124668435	0.8726790450928382	105.0
1.0034662045060658	0.9722703639514731	148.0
0.896551724137931	0.8103448275862069	43.0
0.9509803921568627	0.9248366013071896	142.0
1.0	1.0	14.0
0.9548872180451128	0.7744360902255639	40.0
0.989501312335958	0.9816272965879265	123.0
0.6756756756756757	0.8378378378378378	36.0
0.8333333333333334	0.75	22.0
0.9510869565217391	0.9293478260869565	102.0
0.9815455594002307	0.9538638985005767	194.0
0.9235668789808917	0.940552016985138	128.0
0.8843788437884379	0.8523985239852399	157.0
1.0277008310249307	0.9307479224376731	174.0
1.0132450331125828	0.97918637653737	199.0
0.8940397350993378	0.8145695364238411	55.0
0.9432624113475178	0.9822695035460993	112.0
0.957983193277311	0.9411764705882353	111.0
0.956989247311828	0.956989247311828	25.0
0.9962962962962963	1.0407407407407407	105.0
0.8486486486486486	0.7837837837837838	58.0
0.7205882352941176	0.6029411764705882	55.0
0.9926605504587156	1.003669724770642	131.0
0.8	0.8	11.0
1.062015503875969	1.0465116279069768	84.0
0.9072847682119205	0.9470198675496688	43.0
0.9407008086253369	0.9137466307277629	168.0
1.0208333333333333	1.0	41.0
0.9486166007905138	0.9209486166007905	133.0
0.7666666666666667	0.8666666666666667	28.0
0.8789625360230547	0.9538904899135446	91.0
1.0163934426229508	0.9262295081967213	61.0
1.010204081632653	1.0034013605442176	129.0
0.9723320158102767	0.9367588932806324	150.0
0.9839786381842457	0.9679572763684913	187.0
0.9333333333333333	0.9458333333333333	118.0
1.0	0.9568627450980393	115.0
0.9834368530020704	0.9710144927536232	104.0
0.9348837209302325	0.9441860465116279	113.0
0.9421487603305785	0.9669421487603306	132.0
0.8823529411764706	1.0	17.0
0.9761904761904762	0.9333333333333333	113.0
1.6666666666666667	1.6666666666666667	11.0
0.9202127659574468	0.8617021276595744	94.0
1.0141176470588236	0.9764705882352941	122.0
0.9285714285714286	0.7857142857142857	14.0
0.950920245398773	1.0122699386503067	37.0
0.9496688741721855	0.9231788079470199	178.0
0.8333333333333334	0.8928571428571429	66.0
1.012012012012012	0.977977977977978	217.0
1.0	1.072538860103627	79.0
0.9591836734693877	0.9591836734693877	13.0
0.9219088937093276	0.8872017353579176	111.0
1.0132275132275133	0.9761904761904762	170.0
0.9557069846678024	0.938671209540034	152.0
0.92	0.9163636363636364	131.0
0.9119318181818182	0.9005681818181818	134.0
0.9984076433121019	0.9617834394904459	202.0
1.0025510204081634	0.9668367346938775	169.0
0.9915966386554622	0.9495798319327731	254.0
1.0198347107438017	1.0033057851239668	113.0
0.9222797927461139	0.8860103626943006	107.0
0.9975550122249389	0.9828850855745721	194.0
0.9933333333333333	0.9633333333333334	128.0
0.988647114474929	0.967833491012299	226.0
1.05	1.0333333333333334	87.0
0.6565656565656566	0.696969696969697	30.0
0.9691516709511568	0.9331619537275064	187.0
0.8141592920353983	0.911504424778761	92.0
0.9622641509433962	0.9811320754716981	50.0
0.9556962025316456	0.9367088607594937	93.0
1.0	1.0	8.0
1.0	0.75	14.0
0.9722863741339491	0.9630484988452656	201.0
0.9656652360515021	0.9742489270386266	112.0
0.9150943396226415	0.9622641509433962	53.0
0.9871794871794872	0.9572649572649573	131.0
0.9893190921228304	0.9572763684913218	184.0
1.0	1.2857142857142858	15.0
0.8666666666666667	0.8666666666666667	18.0
0.8895027624309392	1.0	50.0
0.9921104536489151	0.9368836291913215	126.0
0.9496402877697842	0.9496402877697842	99.0
0.8504672897196262	0.9439252336448598	55.0
0.6	0.6	5.0
0.9800796812749004	0.9442231075697212	111.0
0.9875776397515528	0.9254658385093167	44.0
1.037037037037037	0.9259259259259259	27.0
0.9928379588182632	0.9534467323187108	209.0
1.2727272727272727	1.0	18.0
0.9032258064516129	0.8709677419354839	27.0
0.9886547811993517	0.9513776337115073	230.0
0.9196787148594378	0.9437751004016064	73.0
0.8547486033519553	0.8659217877094972	78.0
1.0	0.8333333333333334	18.0
0.9736070381231672	0.9501466275659824	190.0
0.9552238805970149	1.0298507462686568	49.0
1.0	1.0	11.0
0.8779220779220779	0.9298701298701298	188.0
0.8632911392405064	0.8379746835443038	104.0
1.0072992700729928	0.9379562043795621	202.0
0.9482071713147411	0.9402390438247012	141.0
0.993085566119274	0.9498703543647364	235.0
1.0101867572156198	0.967741935483871	224.0
1.0	1.0	2.0
0.937037037037037	0.9222222222222223	145.0
1.0759493670886076	0.9493670886075949	33.0
0.8461538461538461	0.7948717948717948	38.0
1.0032520325203251	0.9463414634146341	230.0
0.9728997289972899	0.8048780487804879	93.0
1.1	1.0333333333333334	35.0
1.0229885057471264	0.946360153256705	97.0
1.0877659574468086	1.0079787234042554	170.0
0.8431372549019608	0.8627450980392157	84.0
1.0080321285140563	0.9477911646586346	113.0
0.96045197740113	0.9322033898305084	102.0
0.8625954198473282	0.8015267175572519	47.0
0.8921161825726142	0.8630705394190872	133.0
0.9623529411764706	0.9623529411764706	197.0
1.0105263157894737	1.0421052631578946	95.0
0.9690140845070423	0.9492957746478873	171.0
0.9895287958115183	0.9476439790575916	239.0
1.0	0.971830985915493	99.0
0.7580645161290323	0.8064516129032258	44.0
0.9880239520958084	1.0598802395209581	44.0
0.8799612778315585	0.8799612778315585	186.0
1.0506329113924051	1.0126582278481013	119.0
0.9949748743718593	0.9748743718592965	95.0
0.952755905511811	0.937007874015748	45.0
1.029520295202952	1.044280442804428	69.0
0.8720538720538721	0.9191919191919192	89.0
1.00531208499336	1.0212483399734396	148.0
0.926509186351706	0.905511811023622	107.0
0.7872340425531915	0.7127659574468085	67.0
0.9136690647482014	0.9136690647482014	41.0
0.8095238095238095	0.7714285714285715	55.0
0.9038461538461539	0.9423076923076923	41.0
1.0	1.0	10.0
1.0	1.0	7.0
0.9622641509433962	0.9119496855345912	143.0
0.9803761242845462	0.9362224039247752	245.0
1.0138768430182135	0.9722463139635733	241.0
0.8859649122807017	1.043859649122807	62.0
0.9734513274336283	0.9336283185840708	122.0
1.0209059233449478	1.0139372822299653	142.0
0.9841897233201581	0.8972332015810277	87.0
1.24	1.24	18.0
0.9782608695652174	1.0434782608695652	37.0
0.9622641509433962	0.9018867924528302	86.0
0.9889349930843707	0.983402489626556	156.0
0.8923766816143498	0.8654708520179372	80.0
0.9204545454545454	0.9545454545454546	69.0
1.3	1.1	18.0
0.989778534923339	0.9045996592844975	156.0
1.0648648648648649	1.0432432432432432	53.0
1.0067340067340067	0.9528619528619529	80.0
0.9797979797979798	0.9595959595959596	193.0
0.9716168271667511	0.9503294475418145	313.0
0.9819458375125376	0.9538615847542627	241.0
1.0	1.0	5.0
0.9811320754716981	0.9150943396226415	114.0
1.0227920227920229	0.9772079772079773	80.0
0.9104477611940298	0.8805970149253731	34.0
0.9262820512820513	0.9423076923076923	130.0
0.9093484419263456	0.9093484419263456	91.0
1.0816326530612246	1.0	43.0
0.954140127388535	0.9898089171974522	122.0
0.9203980099502488	0.9369817578772802	141.0
0.9737827715355806	0.9588014981273408	130.0
0.8481012658227848	0.8227848101265823	27.0
0.9484978540772532	0.9141630901287554	130.0
0.979381443298969	0.9845360824742269	120.0
1.0280701754385966	0.9789473684210527	86.0
0.8780487804878049	0.8658536585365854	51.0
0.9338842975206612	0.9669421487603306	60.0
0.9962406015037594	0.9285714285714286	134.0
1.0145278450363195	1.036319612590799	127.0
0.9949958298582152	0.9516263552960801	245.0
0.9623931623931624	0.9623931623931624	163.0
0.9809523809523809	0.9206349206349206	157.0
1.0	1.0	2.0
1.1470588235294117	1.0588235294117647	26.0
1.010948905109489	0.9416058394160584	212.0
0.6666666666666666	0.4444444444444444	21.0
0.9699248120300752	0.9699248120300752	60.0
1.0148148148148148	0.964021164021164	170.0
0.945823927765237	0.9367945823927766	115.0
0.959748427672956	0.9723270440251572	121.0
1.0	0.9222222222222223	56.0
0.9507389162561576	0.9211822660098522	71.0
0.972972972972973	1.0	26.0
0.9333333333333333	0.9333333333333333	28.0
0.8089171974522293	0.8853503184713376	48.0
0.9322033898305084	0.927360774818402	107.0
1.0096618357487923	1.041062801932367	132.0
0.8962962962962963	0.837037037037037	37.0
0.9575856443719413	0.8564437194127243	117.0
1.0091603053435114	0.9969465648854962	147.0
0.8920086393088553	0.9287257019438445	157.0
1.0909090909090908	1.1818181818181819	8.0
0.9615384615384616	0.9615384615384616	131.0
0.8988095238095238	0.9345238095238095	89.0
0.9858156028368794	0.9432624113475178	95.0
0.90625	0.8958333333333334	147.0
1.0146341463414634	1.0121951219512195	159.0
0.9954128440366973	0.944954128440367	113.0
0.8040816326530612	0.8693877551020408	77.0
0.9210526315789473	0.7894736842105263	40.0
0.8852459016393442	0.8797814207650273	101.0
0.979381443298969	1.0515463917525774	86.0
0.9981447124304267	0.9573283858998145	219.0
0.9736842105263158	0.9122807017543859	62.0
0.9686684073107049	1.0182767624020888	130.0
0.9204244031830239	0.9204244031830239	112.0
1.0	0.9621848739495799	126.0
0.9976218787158145	0.9785969084423306	182.0
0.9571788413098237	0.9118387909319899	172.0
0.9751552795031055	0.9461697722567288	124.0
1.0203821656050955	1.0254777070063694	121.0
0.8041543026706232	0.8100890207715133	100.0
1.0	1.0	5.0
0.9584996009577015	0.9696727853152434	234.0
0.9537688442211055	0.9718592964824121	225.0
0.9519230769230769	0.9519230769230769	63.0
0.9834710743801653	0.9793388429752066	126.0
0.9302832244008714	0.8823529411764706	115.0
1.0148514851485149	1.0272277227722773	171.0
1.043956043956044	1.0	122.0
0.9451612903225807	0.9032258064516129	139.0
0.9571106094808126	0.9413092550790068	197.0
0.8562874251497006	0.9101796407185628	105.0
1.0	1.0	11.0
1.0169971671388103	0.9886685552407932	173.0
0.875	0.8928571428571429	65.0
0.9857651245551602	1.0213523131672597	69.0
0.930635838150289	0.9075144508670521	27.0
0.8100890207715133	0.7626112759643917	92.0
0.9493670886075949	0.9493670886075949	68.0
0.9090909090909091	1.1818181818181819	20.0
0.9865771812080537	0.9642058165548099	130.0
1.005	1.005	96.0
0.9166666666666666	1.0833333333333333	14.0
0.9640044994375703	0.9460067491563554	166.0
0.975	0.9363636363636364	180.0
0.9696969696969697	0.8939393939393939	63.0
0.9675675675675676	0.9531531531531532	156.0
0.944206008583691	0.9313304721030042	120.0
0.9412997903563941	0.9224318658280922	162.0
0.9895424836601308	0.9633986928104575	205.0
0.941944847605225	0.9274310595065312	168.0
0.9333333333333333	0.9333333333333333	62.0
0.9393939393939394	0.9653679653679653	85.0
1.0323529411764707	1.0294117647058822	163.0
1.0214067278287462	0.9969418960244648	153.0
0.8910638297872341	0.902127659574468	354.0
0.9090909090909091	1.0	17.0
0.8823529411764706	0.9019607843137255	156.0
0.9929411764705882	0.9505882352941176	218.0
0.861198738170347	0.8738170347003155	85.0
0.8072289156626506	0.8313253012048193	66.0
0.9664570230607966	0.9077568134171907	131.0
0.9044368600682594	0.9215017064846417	160.0
0.8705035971223022	0.8848920863309353	54.0
0.9798488664987406	0.9546599496221663	168.0
1.0118694362017804	0.950544015825915	231.0
0.875	0.7857142857142857	48.0
1.0	1.0	8.0
0.9852507374631269	0.9351032448377581	169.0
0.9484240687679083	0.8681948424068768	91.0
0.9337748344370861	0.9370860927152318	144.0
0.9805352798053528	0.9464720194647201	105.0
0.93	0.87	87.0
1.0909090909090908	0.9090909090909091	18.0
0.9459459459459459	0.9613899613899614	82.0
1.0208333333333333	1.0416666666666667	52.0
1.0	1.0	8.0
0.9611307420494699	0.9540636042402827	127.0
1.0	0.9464285714285714	39.0
0.8321167883211679	0.9124087591240876	79.0
1.0185185185185186	1.037037037037037	39.0
1.0381991814461118	0.9454297407912687	170.0
0.9777424483306836	0.958664546899841	146.0
0.9	0.9333333333333333	50.0
1.0571428571428572	1.0	35.0
0.9984859954579863	0.9894019682059046	246.0
1.0323325635103926	0.9676674364896074	123.0
0.9179487179487179	0.9692307692307692	38.0
0.9420935412026726	1.0133630289532294	105.0
0.9075907590759076	0.8943894389438944	144.0
1.0275862068965518	1.013793103448276	120.0
0.9173838209982789	0.9001721170395869	144.0
0.996694214876033	1.0231404958677686	113.0
1.0057553956834533	0.9510791366906475	158.0
0.940677966101695	0.9152542372881356	77.0


==> ncrCM_generated_2021-08-06_17-27-03.tex <==
ports/kieler	mixed/kieler	nodes/kieler	vtcs
0.9753086419753086	0.8703703703703703	0.9814814814814815	102.0
0.7912621359223301	0.9077669902912622	0.8276699029126213	145.0
0.8666666666666667	0.8416666666666667	0.925	87.0
1.0	1.0	1.0	18.0
0.8895152198421646	0.8162344983089064	0.8624577226606539	161.0
0.928743961352657	0.8321256038647343	0.9951690821256038	171.0
1.0966183574879227	0.9871175523349437	0.9742351046698873	152.0
1.290909090909091	1.1272727272727272	1.3636363636363635	51.0
0.7096774193548387	0.7419354838709677	0.7258064516129032	39.0
0.9527272727272728	0.9236363636363636	1.0363636363636364	123.0
0.7037037037037037	0.7037037037037037	1.1111111111111112	37.0
0.9	0.8615384615384616	0.9846153846153847	97.0
0.9655172413793104	0.9310344827586207	1.0057471264367817	118.0
0.625	0.6875	0.625	47.0
0.8798206278026905	0.8349775784753363	0.8394618834080717	170.0
0.8407643312101911	1.0636942675159236	1.0955414012738853	103.0
0.4473684210526316	0.543859649122807	0.5964912280701754	76.0
1.0	1.0	1.0	14.0
0.9419953596287703	1.0092807424593968	0.8839907192575406	157.0
0.6	0.8285714285714286	0.8	68.0
0.8715083798882681	0.9036312849162011	0.8142458100558659	125.0
0.9425287356321839	1.0	1.0191570881226053	139.0
0.8269230769230769	1.1730769230769231	1.0384615384615385	47.0
1.2272727272727273	1.2727272727272727	1.2727272727272727	30.0
0.7254901960784313	0.5098039215686274	0.6470588235294118	56.0
0.8138075313807531	0.8859832635983264	0.9194560669456067	151.0
0.8518518518518519	0.9407407407407408	0.8222222222222222	153.0
0.6625	0.8125	0.6875	78.0
0.9378378378378378	1.0013513513513514	0.8783783783783784	156.0
0.8836158192090395	0.9887005649717514	0.8723163841807909	170.0
1.0	1.0	1.0	6.0
0.8789954337899544	0.958904109589041	0.8904109589041096	159.0
0.9049694856146469	0.9110723626852659	0.9838709677419355	228.0
1.0	1.0	1.0	14.0
0.9581915410792416	0.946524064171123	0.8974234321827905	195.0
1.0	1.0	1.0	7.0
1.0521172638436482	1.1074918566775245	0.9022801302931596	131.0
0.9	0.86	0.9666666666666667	90.0
2.0	2.0	1.0	41.0
0.8160919540229885	0.903448275862069	0.7954022988505747	139.0
0.8731707317073171	0.9658536585365853	0.7414634146341463	65.0
0.73989898989899	0.8005050505050505	0.9494949494949495	140.0
0.9885931558935361	0.9657794676806084	0.9505703422053232	116.0
1.0	1.0	1.0	21.0
0.8798727128082736	0.9315831344470963	0.9872712808273667	152.0
0.6515151515151515	0.7121212121212122	0.8333333333333334	52.0
0.9388489208633094	0.8669064748201439	0.9820143884892086	131.0
0.7	0.65	1.0	22.0
0.9708454810495627	0.9300291545189504	0.9446064139941691	118.0
0.968	1.08	0.976	127.0
0.9421487603305785	0.859504132231405	0.8471074380165289	113.0
0.945624468988955	0.881053525913339	0.8903993203058623	204.0
0.8691588785046729	0.8317757009345794	1.0560747663551402	63.0
1.0263852242744063	1.0923482849604222	0.9709762532981531	143.0
0.8302231979509697	0.7939992682034395	0.8379070618368094	236.0
0.6190476190476191	0.42857142857142855	1.0	41.0
0.9275653923541247	0.9647887323943662	0.886317907444668	159.0
0.8582995951417004	0.8663967611336032	0.8866396761133604	103.0
0.9705611775528978	0.9595216191352346	1.1011959521619135	242.0
0.9484978540772532	0.944206008583691	0.9012875536480687	123.0
0.0	0.0	0.0	18.0
0.6688102893890675	0.5562700964630225	0.6816720257234726	86.0
1.088077336197637	1.0279269602577874	1.046186895810956	176.0
1.9090909090909092	1.6363636363636365	1.8181818181818181	28.0
0.8434782608695652	0.9652173913043478	0.8695652173913043	133.0
0.9064748201438849	0.9964028776978417	0.8363309352517986	158.0
0.8516042780748663	0.9679144385026738	0.9237967914438503	157.0
1.0	1.0	1.0	6.0
0.8571428571428571	1.246031746031746	1.0714285714285714	84.0
0.7485029940119761	0.9281437125748503	0.7904191616766467	83.0
0.42452830188679247	0.5094339622641509	0.5754716981132075	30.0
0.5	0.0	0.5	22.0
0.8905775075987842	0.8145896656534954	0.8966565349544073	94.0
0.9612403100775194	0.7984496124031008	0.8449612403100775	90.0
0.9049128367670365	0.9239302694136292	0.8541996830427893	117.0
0.7588832487309645	0.7741116751269036	0.7106598984771574	90.0
0.8952380952380953	0.9523809523809523	0.7666666666666667	131.0
0.8550295857988166	0.7958579881656804	0.9763313609467456	114.0
0.7777777777777778	0.9382716049382716	1.1358024691358024	42.0
1.1097560975609757	0.8292682926829268	0.8780487804878049	85.0
0.75	0.5833333333333334	0.5	24.0
0.6707818930041153	0.8106995884773662	0.7839506172839507	90.0
0.8983050847457628	0.8559322033898306	0.9067796610169492	93.0
0.7556390977443609	0.7030075187969925	0.7819548872180451	195.0
0.9602941176470589	0.8661764705882353	0.9102941176470588	121.0
1.001700680272109	0.9455782312925171	0.8894557823129252	150.0
0.8493150684931506	1.082191780821918	1.0410958904109588	38.0
0.7600527356624918	0.7818061964403428	0.7877389584706658	122.0
0.831390134529148	0.737219730941704	0.7659192825112108	165.0
0.7825443786982249	0.8121301775147929	0.6863905325443787	121.0
0.5	0.5	0.5	4.0
1.0121608980355472	1.0037418147801684	1.0163704396632367	239.0
0.8995983935742972	0.963855421686747	0.9236947791164659	128.0
0.8896210873146623	0.9654036243822076	0.8929159802306426	140.0
1.0	1.0	1.0	16.0
1.0604026845637584	0.9530201342281879	1.1812080536912752	81.0
0.7755102040816326	0.8367346938775511	1.0204081632653061	50.0
1.380952380952381	1.3333333333333333	1.4761904761904763	53.0
0.9635854341736695	1.0070028011204482	0.8431372549019608	167.0
0.8768115942028986	0.7971014492753623	0.7971014492753623	129.0
1.0	1.0	1.0	6.0
1.0	1.0	1.0	18.0
0.7245508982035929	0.8263473053892215	0.7604790419161677	88.0
0.7987341772151899	0.8987341772151899	0.7835443037974683	145.0
0.6666666666666666	0.5686274509803921	0.6862745098039216	43.0
0.902834008097166	0.8279352226720648	0.9089068825910931	129.0
0.7581863979848866	0.7204030226700252	0.906801007556675	119.0
0.9842209072978304	0.8461538461538461	0.8846153846153846	164.0
0.8335607094133697	0.888130968622101	0.8035470668485676	104.0
2.0	2.0	1.0	37.0
0.8340807174887892	0.7488789237668162	0.8071748878923767	127.0
0.903750478377344	0.927860696517413	1.0206659012629162	320.0
0.8737437185929648	0.9623115577889447	0.9899497487437185	186.0
0.7116788321167883	0.6605839416058394	0.7591240875912408	130.0
0.9455095862764884	1.0060544904137234	0.9858728557013118	148.0
1.0	0.5	1.5	8.0
0.7142857142857143	0.6666666666666666	1.0	33.0
1.1151339608979	1.0448950036205649	1.1412020275162926	162.0
0.46153846153846156	0.6076923076923076	0.5192307692307693	37.0
0.8606060606060606	0.9595959595959596	0.9777777777777777	146.0
1.0	1.0	1.0	38.0
0.6153846153846154	0.6666666666666666	0.5128205128205128	61.0
0.9503239740820735	0.9092872570194385	0.9006479481641468	133.0
0.41025641025641024	0.5897435897435898	0.6666666666666666	51.0
1.0	1.0	1.0	10.0
1.121212121212121	1.196969696969697	1.121212121212121	76.0
0.3951890034364261	0.36769759450171824	0.38831615120274915	46.0
0.7985074626865671	0.6380597014925373	0.667910447761194	91.0
1.00199203187251	0.9203187250996016	1.0059760956175299	120.0
1.2107843137254901	1.0931372549019607	1.1127450980392157	79.0
0.7369614512471655	0.8764172335600907	0.8764172335600907	158.0
0.9621380846325167	0.89086859688196	0.8240534521158129	150.0
0.856353591160221	0.7651933701657458	0.7361878453038674	202.0
1.0	1.0	2.0	19.0
0.8985507246376812	0.8840579710144928	0.9710144927536232	50.0
0.7993197278911565	0.7380952380952381	0.8707482993197279	108.0
0.8099364529173888	0.9227036395147313	0.9231658001155402	357.0
0.7942857142857143	0.7028571428571428	0.7771428571428571	78.0
0.8	0.75	0.6	59.0
0.8061224489795918	0.8061224489795918	0.9387755102040817	122.0
1.0	1.0	2.0	25.0
0.5625	0.25	0.5625	49.0
0.9601648351648352	1.0164835164835164	1.043956043956044	141.0
0.9746478873239437	0.9774647887323944	0.9746478873239437	124.0
0.7358490566037735	0.9622641509433962	0.6415094339622641	58.0
0.9130434782608695	1.0434782608695652	1.4782608695652173	30.0
1.6666666666666667	2.6666666666666665	2.6666666666666665	62.0
1.0	1.0	1.0	13.0
0.7673559822747416	0.7474150664697193	0.7769571639586411	120.0
1.3	1.3	1.4	36.0
0.8432671081677704	0.8134657836644592	0.8520971302428256	169.0
0.8283185840707965	0.8460176991150442	0.8088495575221238	159.0
0.9151193633952255	0.9310344827586207	0.713527851458886	172.0
1.1733333333333333	1.2933333333333332	1.2933333333333332	61.0
0.9079497907949791	0.8284518828451883	0.7824267782426778	105.0
1.0	1.0	1.0	5.0
0.9722222222222222	0.9722222222222222	0.7222222222222222	66.0
0.61	0.9	0.78	51.0
0.9575757575757575	0.8848484848484849	0.8242424242424242	112.0
0.8584905660377359	0.8556603773584905	0.8188679245283019	171.0
0.782608695652174	0.8478260869565217	1.065217391304348	65.0
1.0	1.0	1.0	9.0
0.7777777777777778	0.9444444444444444	0.7222222222222222	60.0
1.0192468619246862	0.8690376569037657	0.900418410041841	240.0
1.0267471958584986	0.9068162208800691	0.911993097497843	151.0
1.0278745644599303	0.8013937282229965	0.8118466898954704	125.0
0.9076576576576577	0.8963963963963963	0.990990990990991	144.0
0.5714285714285714	1.0	0.8095238095238095	21.0
0.9654126213592233	0.9399271844660194	1.0661407766990292	140.0
1.0226244343891402	0.8914027149321267	0.8597285067873304	108.0
0.8641188959660298	0.9554140127388535	0.881104033970276	154.0
1.0843373493975903	0.9457831325301205	1.0602409638554218	85.0
1.0300751879699248	0.7894736842105263	0.9323308270676691	80.0
0.9085631349782293	0.9027576197387518	0.888243831640058	142.0
1.0	1.0	1.0	7.0
0.9746376811594203	0.9528985507246377	0.9239130434782609	191.0
1.0769230769230769	1.0769230769230769	2.3076923076923075	29.0
0.7742663656884876	0.8419864559819413	0.7968397291196389	168.0
1.5	1.6666666666666667	1.6666666666666667	56.0
1.0	1.0	1.0	20.0
1.0	1.0	1.0	12.0
0.9251336898395722	0.8502673796791443	0.7486631016042781	90.0
0.9470588235294117	0.9264705882352942	0.8	129.0
1.0523076923076924	1.0707692307692307	1.0892307692307692	126.0
0.7409326424870466	0.8393782383419689	0.9093264248704663	151.0
0.660377358490566	0.49056603773584906	0.8490566037735849	40.0
0.9821428571428571	0.7797619047619048	1.0773809523809523	98.0
0.8367346938775511	0.7142857142857143	1.0612244897959184	47.0
0.7619047619047619	0.8095238095238095	0.5238095238095238	60.0
0.8571428571428571	0.888030888030888	1.0733590733590734	118.0
0.9801829268292683	0.9751016260162602	0.989329268292683	226.0
0.5555555555555556	0.8888888888888888	1.5555555555555556	34.0
0.8795045045045045	0.8051801801801802	0.7995495495495496	136.0
0.8503401360544217	0.6190476190476191	0.6326530612244898	86.0
1.0	1.0	1.0	20.0
0.8	0.7333333333333333	1.1	31.0
1.0	1.0	1.0	20.0
1.0	1.0	1.0	20.0
1.0231884057971015	1.1	0.9652173913043478	150.0
1.0	1.0	1.0	22.0
0.7329376854599406	0.6468842729970327	0.7062314540059347	113.0
1.0	0.0	1.0	36.0
0.7123287671232876	0.684931506849315	0.9041095890410958	56.0
0.8342989571263036	0.9204325994592507	0.824642719196601	210.0
1.0	1.0	1.0	5.0
0.7735849056603774	0.8490566037735849	1.0566037735849056	89.0
1.0217391304347827	1.1304347826086956	0.9782608695652174	24.0
0.84	0.88	1.24	26.0
0.8641975308641975	0.8179012345679012	0.9320987654320988	137.0
1.0256410256410255	0.8205128205128205	0.9487179487179487	50.0
0.9595141700404858	0.7368421052631579	0.854251012145749	74.0
1.0	1.0	1.0	9.0
1.0	1.0	1.0	6.0
0.7857142857142857	0.8142857142857143	0.8285714285714286	139.0
0.8412984670874661	0.821009918845807	0.8187556357078449	249.0
0.8970588235294118	0.8277310924369747	0.9264705882352942	153.0
1.0	1.0	1.0	13.0
1.1072555205047319	1.0630914826498423	1.160883280757098	128.0
0.892128279883382	0.8338192419825073	0.8979591836734694	96.0
0.898876404494382	1.0112359550561798	1.0786516853932584	68.0
0.6666666666666666	0.8888888888888888	0.9444444444444444	45.0
1.0	1.0	1.0	17.0
0.8082975679542204	0.9434907010014306	0.949928469241774	168.0
1.005050505050505	1.0606060606060606	0.9646464646464646	118.0
1.2679738562091503	1.0065359477124183	1.091503267973856	59.0
0.9	1.1	1.2833333333333334	56.0
1.1851851851851851	1.0	1.1925925925925926	119.0
1.0	1.0	1.0	12.0
0.79182156133829	0.8252788104089219	0.8513011152416357	98.0
1.0	1.0	1.0	20.0
1.4615384615384615	1.0769230769230769	1.0769230769230769	67.0
1.2666666666666666	0.8333333333333334	1.0333333333333334	48.0
1.163265306122449	0.9591836734693877	1.0	64.0
0.4	0.2	0.2	17.0
0.8115384615384615	0.8384615384615385	0.8538461538461538	105.0
0.992638036809816	0.9496932515337423	0.9104294478527607	220.0
1.0225352112676056	1.0394366197183098	1.0140845070422535	128.0
0.8093093093093093	0.7822822822822822	0.9039039039039038	114.0
0.7850467289719626	0.7538940809968847	0.9143302180685359	169.0
1.0	1.0	1.0	16.0
0.8280757097791798	0.8990536277602523	0.7018927444794952	147.0
0.8673587081891581	0.9215686274509803	0.8385236447520185	140.0
0.8315665488810365	0.856301531213192	0.8680800942285041	177.0
0.7920353982300885	0.8982300884955752	1.0044247787610618	87.0
0.9455307262569832	0.888268156424581	1.0512104283054005	356.0
0.7083333333333334	0.625	0.75	22.0
0.8563748079877113	0.8717357910906298	0.84715821812596	129.0
0.7384105960264901	0.7384105960264901	0.7052980132450332	97.0
0.9062947067238912	0.9334763948497854	0.8619456366237482	163.0
0.0	0.0	0.0	14.0
0.696969696969697	0.7272727272727273	0.9090909090909091	81.0
0.8307984790874525	0.8326996197718631	0.7642585551330798	189.0
0.9814814814814815	1.0925925925925926	0.9814814814814815	102.0
1.2571428571428571	1.2285714285714286	1.3142857142857143	86.0
1.0	1.0	1.0	11.0
0.6697566628041715	0.7311703360370799	0.6998841251448435	190.0
0.9553571428571429	0.7678571428571429	0.9255952380952381	192.0
0.8807947019867549	0.82560706401766	0.8543046357615894	122.0
0.8533333333333334	0.8266666666666667	0.81	96.0
0.7931034482758621	0.9310344827586207	1.0	78.0
0.66	0.72	0.98	51.0
0.9345454545454546	0.8739393939393939	0.8751515151515151	164.0
1.2666666666666666	1.0666666666666667	1.4666666666666666	47.0
0.953757225433526	1.0520231213872833	0.9595375722543352	112.0
0.5166666666666667	0.6666666666666666	0.6833333333333333	41.0
0.9612403100775194	0.7364341085271318	0.9050387596899225	145.0
0.9822150363783346	0.9781729991915926	1.0703314470493128	244.0
0.8089887640449438	0.797752808988764	0.6853932584269663	41.0
0.7670454545454546	0.9715909090909091	0.9659090909090909	128.0
1.001310615989515	0.9239842726081258	0.8112712975098296	205.0
0.7785630153121319	0.833922261484099	0.7491166077738516	162.0
0.8906324298621018	0.8297669995244888	0.9667142177841179	252.0
1.0	0.0	1.0	31.0
0.781431334622824	0.8839458413926499	0.8317214700193424	112.0
0.9277010560519903	0.8582453290008123	0.8277822908204712	213.0
0.8245614035087719	0.8538011695906432	0.7852965747702589	154.0
0.7647058823529411	0.6176470588235294	0.7647058823529411	34.0
1.4	1.0	1.2	28.0
0.7697368421052632	0.8717105263157895	0.7796052631578947	101.0
0.7872340425531915	0.9375	0.9042553191489362	200.0
0.9219440353460973	0.8703976435935199	0.9322533136966127	203.0
0.0	0.3333333333333333	0.3333333333333333	39.0
0.8734896943852167	0.9395877754086709	0.845771144278607	128.0
0.7586206896551724	0.8390804597701149	0.7586206896551724	76.0
0.7936507936507936	1.0476190476190477	0.7619047619047619	81.0
0.618421052631579	0.6973684210526315	0.7401315789473685	113.0
1.0492610837438423	0.9770114942528736	1.0459770114942528	124.0
0.8973214285714286	0.8861607142857143	0.9151785714285714	78.0
1.0	1.0	1.0	15.0
0.7661691542288557	0.8079601990049752	0.8238805970149253	169.0
0.9001956947162426	0.9471624266144814	0.8913894324853229	129.0
0.9824945295404814	0.9212253829321663	0.9146608315098468	135.0
0.8117977528089888	0.6460674157303371	0.7134831460674157	90.0
0.8937753721244925	0.9215155615696887	0.9039242219215156	162.0
0.8372093023255814	0.7906976744186046	1.0	34.0
1.0	1.0	1.0	18.0
1.3333333333333333	0.5833333333333334	1.1666666666666667	23.0
1.0	1.0	1.0	5.0
1.0930232558139534	1.0116279069767442	0.9186046511627907	96.0
0.8366445916114791	0.8852097130242825	0.8432671081677704	142.0
0.7128712871287128	0.8184818481848185	0.8217821782178217	138.0
1.0	1.0	1.0	31.0
1.0	1.0	1.0	13.0
0.9934747145187602	0.9314845024469821	0.933115823817292	139.0
1.0	1.0	1.0	36.0
0.7896825396825397	0.8531746031746031	0.8650793650793651	122.0
0.5736842105263158	0.6052631578947368	0.5578947368421052	60.0
0.8577946768060837	0.8463878326996198	0.8692015209125475	244.0
0.9224489795918367	0.9612244897959183	0.9857142857142858	142.0
0.9227399442453206	0.9840700915969733	0.94026284348865	206.0
1.0	1.0	1.0	15.0
0.9192751235584844	0.9357495881383855	0.8599670510708401	190.0
0.850381679389313	0.9236641221374046	0.8320610687022901	108.0
0.726962457337884	0.7610921501706485	0.8907849829351536	106.0
0.9044715447154471	0.8170731707317073	1.016260162601626	138.0
1.0265486725663717	1.008849557522124	0.9380530973451328	62.0
1.8571428571428572	1.8571428571428572	1.2857142857142858	94.0
0.9426229508196722	0.75	0.9754098360655737	88.0
0.895364238410596	0.8390728476821192	0.9754966887417219	154.0
0.5	0.5	0.5	14.0
0.9218241042345277	0.9315960912052117	1.0537459283387622	186.0
0.859375	0.9244791666666666	0.8971354166666666	193.0
0.5833333333333334	0.5833333333333334	1.25	58.0
0.7647058823529411	0.6588235294117647	0.49411764705882355	65.0
0.9005439005439005	0.940947940947941	0.728049728049728	169.0
0.8778367938194109	0.9536455818445195	0.9444712699179141	203.0
1.025390625	1.02734375	0.96875	165.0
1.188235294117647	1.0	1.0588235294117647	96.0
1.0	2.0	1.25	47.0
0.7142857142857143	0.8571428571428571	0.7142857142857143	80.0
0.7434640522875817	0.7271241830065359	0.8284313725490197	136.0
1.1355311355311355	1.1465201465201464	0.8644688644688645	119.0
0.8547297297297297	0.9391891891891891	1.0675675675675675	97.0
0.7887049659201558	0.7176241480038948	0.7497565725413826	132.0
1.3333333333333333	0.8333333333333334	0.8333333333333334	24.0
0.8710050057758952	0.8663842895648826	0.8648440508278783	248.0
1.0	1.0	1.0	11.0
0.8963210702341137	0.9732441471571907	0.9732441471571907	97.0
0.9235668789808917	0.8931351733899504	0.9646142958244869	227.0
1.037037037037037	1.0	0.6666666666666666	36.0
0.625	1.2083333333333333	1.25	23.0
0.8859315589353612	0.8124207858048162	0.899873257287706	161.0
0.9253048780487805	0.913109756097561	0.9512195121951219	137.0
0.7939508506616257	0.7485822306238186	0.888468809073724	144.0
0.938036809815951	0.9067484662576687	0.8938650306748466	217.0
0.8596491228070176	0.8070175438596491	0.7894736842105263	36.0
0.93125	0.75	0.8125	89.0
1.0066445182724253	0.8615725359911407	0.8039867109634552	176.0
1.123076923076923	0.8923076923076924	1.0769230769230769	47.0
1.0	1.0	1.0	5.0
0.9021113243761996	0.9539347408829175	0.8752399232245681	191.0
0.9657534246575342	1.0791476407914764	0.882800608828006	121.0
0.8857142857142857	0.9619047619047619	1.019047619047619	59.0
1.0	1.0	1.0	13.0
0.9444444444444444	0.8159722222222222	0.9791666666666666	89.0
0.943089430894309	0.8211382113821138	0.9349593495934959	117.0
0.6956521739130435	0.6956521739130435	0.6956521739130435	57.0
0.7365145228215768	0.7966804979253111	0.7053941908713693	86.0
1.0	1.0	1.0	19.0
0.9527389903329753	0.8088077336197637	0.9849624060150376	173.0
0.5993623804463337	0.7545164718384697	0.8416578108395324	113.0
1.2118644067796611	1.0805084745762712	1.0254237288135593	87.0
0.8715083798882681	0.8696461824953445	0.7914338919925512	143.0
0.7078825347758887	0.8207109737248841	0.8129829984544049	179.0
1.122492080253432	1.096092925026399	1.133051742344245	195.0
0.9090909090909091	0.8876262626262627	0.928030303030303	215.0
0.6627218934911243	0.7322485207100592	0.7159763313609467	110.0
1.0015847860538827	0.849445324881141	0.884310618066561	151.0
0.8152709359605911	0.9014778325123153	0.9261083743842364	157.0
0.868421052631579	0.7807017543859649	0.8333333333333334	134.0
0.8375	0.875	0.8553571428571428	172.0
1.0	0.8843537414965986	0.8775510204081632	108.0
0.5555555555555556	0.4444444444444444	0.4444444444444444	18.0
1.0571428571428572	0.9	1.2	53.0
0.8166666666666667	0.95	1.0	116.0
0.8567901234567902	0.9300411522633745	0.8765432098765432	118.0
0.6111111111111112	0.6172839506172839	0.7901234567901234	103.0
0.978	0.91	0.9826666666666667	220.0
1.0619469026548674	0.8539823008849557	0.8141592920353983	112.0
0.79	1.06	0.79	93.0
0.7317708333333334	0.8619791666666666	0.9453125	93.0
0.8864468864468864	0.8461538461538461	0.9413919413919414	126.0
1.0	1.0	1.0	22.0
0.8659112370160529	0.9886685552407932	0.9631728045325779	177.0
0.9960526315789474	0.9825187969924812	0.9531954887218045	320.0
1.0	1.0	1.0	32.0
0.8805913570887035	0.8605003790750568	0.9438968915845337	237.0
0.6164383561643836	0.726027397260274	0.8356164383561644	47.0
0.9464114832535885	0.9090909090909091	0.8354066985645933	190.0
0.5	0.631578947368421	0.7631578947368421	84.0
0.4666666666666667	0.6666666666666666	0.7333333333333333	34.0
2.0	2.0	3.0	43.0
0.5517241379310345	0.5172413793103449	0.4482758620689655	63.0
0.8990228013029316	1.260586319218241	1.1009771986970684	123.0
0.9710144927536232	0.9420289855072463	0.961352657004831	133.0
0.8567073170731707	0.7896341463414634	1.1554878048780488	143.0
0.648	0.644	0.58	141.0
1.0325476992143658	0.9225589225589226	1.0179573512906845	164.0
1.0	0.5	0.5	24.0
0.8422712933753943	0.7760252365930599	0.9274447949526814	105.0
0.5365853658536586	0.6585365853658537	0.6829268292682927	57.0
0.6203473945409429	0.7208436724565757	0.7320099255583127	136.0
1.0	1.0	1.0	13.0
0.9423076923076923	0.782051282051282	0.9166666666666666	40.0
0.9902557856272838	0.9951278928136419	1.0475030450669915	169.0
0.8067940552016986	0.8174097664543525	0.7813163481953291	100.0
0.8685669041963578	0.8721298495645289	0.9176563737133808	204.0
1.0	1.0	1.0	8.0
0.875	1.0263157894736843	0.9868421052631579	89.0
0.9156976744186046	0.8372093023255814	0.9941860465116279	133.0
0.8340740740740741	0.8055555555555556	0.9011111111111111	239.0
1.0	1.0	1.0	34.0
0.9047619047619048	0.8820861678004536	0.909297052154195	127.0
0.9336099585062241	0.8838174273858921	0.8713692946058091	123.0
0.8590057049714751	0.8581907090464548	0.8736756316218419	150.0
0.691358024691358	0.5308641975308642	0.6049382716049383	71.0
0.5370370370370371	0.6296296296296297	0.7962962962962963	73.0
0.9519230769230769	0.8576923076923076	0.9346153846153846	160.0
1.006282722513089	0.9968586387434555	0.93717277486911	198.0
0.7058823529411765	0.5294117647058824	1.6470588235294117	28.0
0.88	1.04	0.94	104.0
1.0	1.0	1.0	15.0
1.0676691729323309	0.8045112781954887	0.8947368421052632	94.0
0.867704280155642	0.980544747081712	0.8832684824902723	151.0
1.2	0.75	1.35	46.0
0.8509895227008148	0.89988358556461	0.7182770663562281	199.0
1.0	1.0	1.0	9.0
1.0	1.0	1.0	19.0
0.7941176470588235	0.8823529411764706	1.1470588235294117	30.0
0.7860394537177542	0.9484066767830045	0.8239757207890743	163.0
0.7513227513227513	0.9126984126984127	0.6957671957671958	118.0
1.0	1.0	1.0	7.0
0.9233610341643582	0.8901200369344414	0.8494921514312096	115.0
0.8632619439868204	0.8303130148270181	0.7594728171334432	158.0
1.0095238095238095	0.8952380952380953	1.0285714285714285	48.0
0.9826756496631376	0.8527430221366699	0.7921077959576516	176.0
0.6336405529953917	0.7649769585253456	0.6728110599078341	128.0
0.875	1.1875	1.5	58.0
0.775	1.35	1.1	49.0
0.9219905850706119	0.8917283120376597	0.8977807666442502	191.0
0.3333333333333333	0.3333333333333333	0.3333333333333333	4.0
0.6964285714285714	0.5	0.5535714285714286	49.0
1.8095238095238095	1.7380952380952381	1.2857142857142858	48.0
0.8445297504798465	0.7965451055662188	0.9673704414587332	134.0
1.1923076923076923	1.0384615384615385	0.5384615384615384	66.0
0.84375	0.96875	1.0625	64.0
0.8849021435228331	0.9342963653308481	0.8606710158434296	245.0
1.0	2.0	1.0	12.0
1.0	2.0	1.0	38.0
0.8505747126436781	0.7509578544061303	0.735632183908046	127.0
0.7523809523809524	0.7523809523809524	0.7166666666666667	84.0
1.0	1.0	1.0	11.0
0.6410256410256411	0.6538461538461539	0.5	70.0
0.9866666666666667	0.9333333333333333	0.9644444444444444	74.0
0.839047619047619	0.8419047619047619	0.8904761904761904	133.0
1.0077519379844961	1.058139534883721	0.9302325581395349	122.0
0.9370185772541912	0.8962392387856819	0.9710013593112823	239.0
1.0	1.0	1.0	9.0
0.9271809661139149	0.7801009372746935	0.8139870223503965	166.0
1.0	1.0	1.0	21.0
1.025609756097561	1.0682926829268293	0.9207317073170732	171.0
0.8275862068965517	0.9913793103448276	0.896551724137931	64.0
0.742928452579035	0.8527454242928453	0.8660565723793677	130.0
0.7836463223787168	0.8646322378716745	0.9017996870109546	229.0
0.831081081081081	0.8175675675675675	0.8716216216216216	66.0
0.9333333333333333	1.0666666666666667	0.9333333333333333	53.0
0.78125	0.9375	1.28125	43.0
0.65625	0.6674107142857143	0.6875	75.0
0.8538461538461538	0.8346153846153846	0.9230769230769231	115.0
0.8622273249138921	0.8714121699196326	0.9644087256027555	216.0
0.7976190476190477	0.6428571428571429	0.7738095238095238	52.0
0.8628571428571429	0.8571428571428571	0.8971428571428571	90.0
1.0	1.0	1.0	10.0
1.0182370820668694	0.9696048632218845	1.0851063829787233	221.0
0.896551724137931	0.7379310344827587	0.9586206896551724	88.0
0.9761904761904762	0.8333333333333334	0.9761904761904762	36.0
0.8143459915611815	0.7552742616033755	1.029535864978903	110.0
0.9399141630901288	0.7660944206008584	0.9291845493562232	121.0
0.9439252336448598	0.8504672897196262	1.02803738317757	96.0
0.8177361853832442	0.7789661319073083	0.7803030303030303	247.0
0.8333333333333334	0.6851851851851852	0.7592592592592593	94.0
0.7564102564102564	0.8205128205128205	0.7628205128205128	91.0
1.0	1.0	1.0	36.0
0.7142857142857143	0.2857142857142857	1.2857142857142858	39.0
0.907185628742515	0.9391217564870259	0.8502994011976048	161.0
0.8864915572232646	0.875234521575985	0.8545966228893058	161.0
1.0214285714285714	1.0928571428571427	0.8785714285714286	108.0
0.9139987445072191	0.8480853735091023	0.874450721908349	233.0
1.0	1.0	1.0	6.0
0.8926132836747361	0.8727498448168839	0.8603351955307262	155.0
0.9041095890410958	0.8287671232876712	0.8356164383561644	103.0
1.0	1.0	1.0	19.0
0.8238095238095238	0.7428571428571429	0.8571428571428571	68.0
1.0	0.8370044052863436	0.8414096916299559	109.0
0.6511627906976745	0.9651162790697675	0.7093023255813954	41.0
0.9624530663329162	0.9899874843554443	0.9987484355444305	168.0
0.8313953488372093	0.9040697674418605	0.7994186046511628	127.0
0.660377358490566	0.6415094339622641	0.7735849056603774	96.0
0.9016393442622951	0.8360655737704918	0.7868852459016393	84.0
0.821917808219178	0.8493150684931506	0.8082191780821918	34.0
0.822104466313399	0.8327024981074943	0.7751703255109765	203.0
0.8043478260869565	1.0	1.2826086956521738	54.0
0.8140597539543059	0.8235500878734622	0.7156414762741652	203.0
1.105263157894737	0.9649122807017544	0.8421052631578947	67.0
1.0	0.9666666666666667	1.1666666666666667	92.0
0.8648648648648649	0.8141891891891891	0.8783783783783784	103.0
1.040169133192389	1.0190274841437632	1.0993657505285412	140.0
1.0982142857142858	1.2008928571428572	1.0758928571428572	117.0
0.8118240807498197	0.7519826964671954	0.9870223503965393	156.0
0.9314928425357873	0.9294478527607362	1.0040899795501022	167.0
0.8024691358024691	0.5555555555555556	0.691358024691358	84.0
0.9062240663900415	0.7551867219917012	0.9684647302904564	169.0
0.559322033898305	1.0	0.7627118644067796	64.0
1.0203045685279188	0.9416243654822335	0.7791878172588832	150.0
0.9955621301775148	1.1124260355029585	1.0399408284023668	129.0
0.9702209414024976	0.8443804034582133	0.8491834774255523	155.0
1.0	1.0	1.0	14.0
0.6083916083916084	0.44755244755244755	0.5664335664335665	59.0
0.7701227830832197	0.8362892223738063	0.7776261937244202	179.0
0.9432387312186978	0.8614357262103506	0.8731218697829716	149.0
0.8123667377398721	0.7654584221748401	0.7484008528784648	132.0
0.8384146341463414	1.0274390243902438	0.9359756097560976	152.0
0.9241245136186771	0.7830739299610895	0.8929961089494164	236.0
0.8625128733264675	0.8341915550978373	0.805870236869207	247.0
0.6753246753246753	0.5064935064935064	0.5714285714285714	39.0
0.8421052631578947	0.7894736842105263	0.7368421052631579	52.0
0.7936507936507936	0.6507936507936508	0.9523809523809523	36.0
0.9082969432314411	0.9301310043668122	0.8602620087336245	119.0
0.7764705882352941	0.6970588235294117	0.7823529411764706	103.0
0.8414634146341463	0.9451219512195121	0.8353658536585366	145.0
0.8668661181750187	0.9072550486163051	0.8451757666417352	230.0
1.0068461889548153	0.9890460976722958	0.967594705613875	244.0
0.7745583038869258	0.888339222614841	0.9187279151943463	221.0
1.2850678733031675	1.0407239819004526	1.1266968325791855	113.0
0.6833333333333333	0.65	0.85	49.0
0.8754752851711026	0.7984790874524715	0.9287072243346007	167.0
0.7023809523809523	0.6666666666666666	0.6190476190476191	87.0
3.0	3.0	5.0	35.0
0.8907563025210085	1.1008403361344539	0.907563025210084	116.0
0.819078947368421	0.7631578947368421	0.7911184210526315	135.0
0.625	0.625	1.125	29.0
0.7790055248618785	0.8425414364640884	0.7762430939226519	147.0
0.6879432624113475	0.900709219858156	0.7411347517730497	140.0
1.0	1.0	1.0	6.0
0.9379310344827586	0.8827586206896552	0.8827586206896552	101.0
1.2727272727272727	1.0909090909090908	1.4545454545454546	67.0
0.9616336633663366	0.8502475247524752	0.9504950495049505	142.0
0.8072407045009785	0.8331702544031311	0.8258317025440313	208.0
1.2	1.0857142857142856	1.2285714285714286	73.0
0.9523809523809523	0.8095238095238095	1.0523809523809524	104.0
0.9267990074441688	0.913151364764268	0.826302729528536	127.0
0.8064516129032258	0.8903225806451613	0.864516129032258	57.0
0.7931818181818182	0.9590909090909091	0.7909090909090909	165.0
0.75	0.7145833333333333	0.6958333333333333	142.0
0.6938775510204082	0.782312925170068	0.891156462585034	84.0
0.8132780082987552	0.8360995850622407	0.8340248962655602	139.0
0.8225806451612904	0.8387096774193549	0.8655913978494624	124.0
0.8098591549295775	0.8591549295774648	0.8485915492957746	95.0
1.0	1.0	1.0	7.0
0.8177966101694916	0.826271186440678	0.8771186440677966	119.0
0.7801857585139319	0.8606811145510835	0.6501547987616099	101.0
0.747887323943662	0.9605633802816902	0.9014084507042254	113.0
1.0	1.173913043478261	1.1304347826086956	20.0
0.9090909090909091	0.8181818181818182	0.8268398268398268	126.0
0.9459684123025769	0.9950124688279302	0.9609310058187863	167.0
0.8416666666666667	0.9305555555555556	0.8847222222222222	162.0
0.8260869565217391	1.0869565217391304	1.2173913043478262	45.0
0.9053987122337791	0.9782070331847449	0.9148093115403665	240.0
0.8740359897172236	0.884318766066838	0.7300771208226221	113.0
0.9506172839506173	1.02880658436214	1.0781893004115226	122.0
0.8580323785803238	0.8804483188044832	0.8767123287671232	150.0
1.3333333333333333	1.2222222222222223	0.8888888888888888	34.0
0.6634615384615384	0.7451923076923077	0.7403846153846154	91.0
0.9049471928849361	0.8854919399666481	0.8321289605336298	199.0
0.8771929824561403	0.9093567251461988	0.9239766081871345	114.0
1.0	1.0	1.0	34.0
0.75	0.75	1.3333333333333333	29.0
1.1333333333333333	0.4666666666666667	0.7666666666666667	69.0
0.8061224489795918	0.8724489795918368	0.7857142857142857	68.0
0.4838709677419355	0.7096774193548387	0.5161290322580645	30.0
0.45454545454545453	0.7878787878787878	0.6666666666666666	57.0
0.9959514170040485	0.9352226720647774	0.8906882591093117	142.0
2.0	2.5	1.5	25.0
0.8620689655172413	1.0344827586206897	0.9655172413793104	48.0
0.9133537206931702	0.8256880733944955	0.9418960244648318	166.0
0.826278984173721	0.9400073610599926	0.9484725800515275	245.0
1.042081101759755	0.96327467482785	0.9196633511859219	220.0
1.0	1.0	1.0	22.0
0.9616519174041298	0.9498525073746312	1.056047197640118	111.0
1.02	0.58	0.92	39.0
1.0357142857142858	1.0542328042328042	1.0317460317460319	182.0
0.9015151515151515	0.7916666666666666	0.8901515151515151	105.0
0.9528301886792453	0.8537735849056604	0.8726415094339622	132.0
0.9230769230769231	1.0769230769230769	1.4615384615384615	73.0
0.9065420560747663	0.9252336448598131	0.9205607476635514	109.0
0.7288	0.7952	0.7024	134.0
0.779874213836478	0.939203354297694	0.9580712788259959	145.0
0.9057239057239057	0.8518518518518519	0.7542087542087542	131.0
0.9333333333333333	0.9271221532091097	0.9598343685300207	233.0
0.9051490514905149	0.9363143631436315	0.9444444444444444	165.0
0.7543859649122807	0.8385964912280702	0.8421052631578947	127.0
1.0	2.0	1.0	17.0
0.7047434656340755	0.5430784123910939	0.7725072604065828	120.0
0.7697160883280757	0.8596214511041009	0.6766561514195584	166.0
0.0	0.5	1.5	33.0
0.7	1.0	0.9	25.0
0.6790540540540541	0.7804054054054054	0.7195945945945946	107.0
1.0	1.0	1.0	6.0
0.8556067588325653	0.9877112135176651	0.977726574500768	176.0
0.8872976338729763	0.9632627646326276	0.9122042341220423	230.0
0.9088082901554404	0.7481865284974093	0.7937823834196891	190.0
0.8916256157635468	0.8472906403940886	0.7980295566502463	111.0
1.1243243243243244	0.8540540540540541	0.8648648648648649	96.0
1.090497737556561	1.088235294117647	1.160633484162896	142.0
0.8232306129359973	0.7812394175414832	0.8046054859464951	231.0
0.3333333333333333	0.6666666666666666	0.5555555555555556	32.0
0.9383617193836172	0.8921330089213301	0.7988645579886455	126.0
0.7864077669902912	0.7912621359223301	0.9854368932038835	130.0
0.9285714285714286	0.7857142857142857	1.2142857142857142	22.0
0.7739801543550165	0.8996692392502756	0.802646085997795	180.0
0.8775235531628532	0.7900403768506057	0.7738896366083445	134.0
0.7513227513227513	0.8465608465608465	0.8597883597883598	143.0
0.8571428571428571	0.8428571428571429	1.1428571428571428	53.0
0.825938566552901	0.8657565415244596	0.8100113765642776	160.0
0.7891566265060241	0.7891566265060241	0.927710843373494	110.0
0.8818565400843882	0.9353023909985936	0.9240506329113924	135.0
0.9578181818181818	0.978909090909091	0.9170909090909091	150.0
1.048417132216015	1.132216014897579	0.9739292364990689	117.0
1.236842105263158	0.8157894736842105	0.9736842105263158	64.0
0.8654353562005277	0.9261213720316622	0.7044854881266491	92.0
0.9166011014948859	0.9040125885129819	0.9158143194335169	132.0
0.7471264367816092	0.8045977011494253	0.7586206896551724	49.0
1.1622516556291391	1.0794701986754967	1.0413907284768211	187.0
1.1666666666666667	1.6666666666666667	2.3333333333333335	33.0
0.871222076215506	0.8028909329829172	0.783180026281209	174.0
0.7508650519031141	0.9100346020761245	0.8512110726643599	157.0
0.5	0.5714285714285714	0.7142857142857143	63.0
1.0	1.0	1.0	20.0
1.0	1.0	1.0	7.0
1.3571428571428572	1.2678571428571428	1.125	42.0
0.786783042394015	0.8154613466334164	0.8029925187032418	130.0
0.8836734693877552	0.9081632653061225	0.9163265306122449	174.0
0.8625	0.859375	0.8171875	165.0
0.5923566878980892	0.802547770700637	0.7707006369426752	82.0
0.23529411764705882	0.22994652406417113	0.18181818181818182	40.0
0.71875	1.0	0.78125	63.0
0.7333333333333333	0.9333333333333333	1.2	58.0
0.7231270358306189	0.6905537459283387	0.8273615635179153	122.0
0.8510726072607261	0.9174917491749175	0.9463696369636964	229.0
1.10625	0.95	0.975	105.0
0.9459459459459459	0.918918918918919	1.0	48.0
0.7491638795986622	0.7625418060200669	0.9464882943143813	141.0
0.7445848375451264	0.8583032490974729	0.8501805054151624	162.0
0.9107692307692308	0.7723076923076924	0.8123076923076923	100.0
0.9997285190715353	1.0548391475498846	0.9820822587213248	352.0
0.9351995852773458	0.9160186625194401	0.8724727838258165	241.0
1.063157894736842	1.0451127819548873	1.0706766917293233	154.0
0.8708791208791209	0.8269230769230769	0.8882783882783882	155.0
0.9257425742574258	0.900990099009901	0.6633663366336634	90.0
1.0	1.3333333333333333	1.3333333333333333	19.0
0.8025751072961373	0.9871244635193133	1.0515021459227467	78.0
1.030891438658429	1.1094439541041483	1.0820829655781112	170.0
0.8425531914893617	0.7914893617021277	0.7106382978723405	22.0
0.8076923076923077	0.7019230769230769	0.7403846153846154	74.0
0.9081515499425947	0.8897818599311137	1.0229621125143513	172.0
0.9171597633136095	0.8757396449704142	0.9260355029585798	108.0
1.119047619047619	0.8333333333333334	1.1666666666666667	75.0
1.0909090909090908	1.2727272727272727	1.0	35.0
1.0027855153203342	0.9651810584958217	1.011142061281337	156.0
1.0	1.0	1.0	26.0
0.96	0.8	0.96	69.0
0.9696387394312067	0.921598770176787	0.9146810146041506	250.0
0.877030162412993	0.9454756380510441	0.9965197215777262	202.0
0.8896551724137931	0.8672413793103448	0.878448275862069	161.0
0.8432432432432433	0.654054054054054	0.6972972972972973	71.0
0.8090909090909091	0.7890909090909091	0.8927272727272727	191.0
0.710997442455243	0.7647058823529411	0.7723785166240409	79.0
0.7384615384615385	0.7538461538461538	0.9846153846153847	50.0
0.7242857142857143	0.7628571428571429	0.7614285714285715	111.0
0.918848167539267	0.8468586387434555	0.9541884816753927	177.0
0.9848942598187311	0.9516616314199395	0.9486404833836858	122.0
0.9897959183673469	1.1326530612244898	0.9489795918367347	101.0
0.9161290322580645	0.8774193548387097	1.070967741935484	86.0
0.64	0.592	0.724	87.0
1.0571428571428572	1.1428571428571428	1.1357142857142857	81.0
1.0253164556962024	0.9683544303797469	1.0	90.0
0.8538461538461538	0.9846153846153847	1.2230769230769232	97.0
0.8211382113821138	0.8102981029810298	0.8319783197831978	188.0
0.9700598802395209	0.7964071856287425	0.9550898203592815	89.0
2.5	1.0	2.5	22.0
0.8813559322033898	1.1468926553672316	0.9548022598870056	82.0
0.7464387464387464	0.886039886039886	0.8547008547008547	116.0
0.868020304568528	0.916243654822335	0.9467005076142132	134.0
0.6255506607929515	0.6901615271659325	0.7635829662261381	111.0
0.7631578947368421	0.7368421052631579	1.0526315789473684	26.0
0.815028901734104	0.9595375722543352	0.8901734104046243	98.0
0.8486238532110092	0.8394495412844036	0.6559633027522935	99.0
1.0	1.0	1.0	30.0
0.7021276595744681	0.7021276595744681	0.8191489361702128	71.0
1.0111524163568772	0.7843866171003717	0.9851301115241635	97.0
0.8630705394190872	0.7468879668049793	0.6846473029045643	105.0
0.7198697068403909	0.7361563517915309	0.9543973941368078	108.0
1.0	1.0	1.0	16.0
1.045822102425876	0.921832884097035	0.9245283018867925	109.0
0.7096774193548387	1.032258064516129	0.8870967741935484	52.0
0.9132290184921764	0.9459459459459459	1.0014224751066856	140.0
0.8375350140056023	0.7759103641456583	0.8235294117647058	187.0
1.0	1.0	1.0	30.0
0.5411764705882353	0.5882352941176471	0.6352941176470588	51.0
0.6492985971943888	0.8897795591182365	0.8957915831663327	115.0
0.6831275720164609	0.8847736625514403	0.7983539094650206	97.0
0.9038461538461539	0.7980769230769231	0.8846153846153846	85.0
1.1047297297297298	0.981418918918919	1.0472972972972974	168.0
0.8900255754475703	0.9514066496163683	0.9641943734015346	149.0
0.8764746703678001	0.8917418459403192	0.8743927827897293	164.0
0.8461538461538461	0.2692307692307692	0.5	53.0
0.8912489379779099	0.9099405267629567	0.842820730671198	124.0
0.9565217391304348	1.05720823798627	1.0503432494279177	157.0
0.8461538461538461	0.8974358974358975	1.1282051282051282	42.0
0.7972027972027972	0.7762237762237763	0.7202797202797203	97.0
0.9130434782608695	1.0434782608695652	0.9782608695652174	41.0
1.0	1.0	1.0	25.0
0.8746397694524496	0.9798270893371758	0.8976945244956772	149.0
0.945054945054945	0.8461538461538461	1.0137362637362637	84.0
1.0225563909774436	0.9849624060150376	0.9548872180451128	94.0
1.1538461538461537	1.0923076923076922	1.2307692307692308	46.0
0.9624277456647399	1.046242774566474	1.060693641618497	121.0
1.0	0.8617511520737328	0.9078341013824884	142.0
0.38235294117647056	0.6470588235294118	0.7352941176470589	76.0
0.9121830550401979	0.9987631416202845	0.9573283858998145	219.0
0.9595238095238096	0.8071428571428572	0.9880952380952381	121.0
0.8287037037037037	0.9398148148148148	0.8981481481481481	57.0
0.9511400651465798	0.8127035830618893	0.8973941368078175	127.0
1.1233933161953729	0.9665809768637532	1.1465295629820051	146.0
1.0	1.0	1.0	28.0
0.7941176470588235	0.9852941176470589	1.1397058823529411	107.0
0.7697594501718213	0.8487972508591065	0.9725085910652921	118.0
0.9826589595375722	0.9710982658959537	1.0346820809248556	117.0
0.9640718562874252	1.1916167664670658	1.1437125748502994	82.0
0.8	1.6	1.1166666666666667	50.0
0.7625	0.755	0.8075	124.0
1.0572972972972974	0.9848648648648649	0.96	147.0
0.9977142857142857	0.9954285714285714	0.9657142857142857	213.0
0.8666666666666667	0.8583333333333333	1.0166666666666666	130.0
0.5424528301886793	0.5094339622641509	0.6037735849056604	24.0
0.9123809523809524	0.9123809523809524	0.8952380952380953	186.0
0.9779735682819384	0.9251101321585903	0.8193832599118943	121.0
0.9331779331779332	0.9137529137529138	0.8477078477078477	123.0
0.8679245283018868	1.1320754716981132	1.2339622641509433	112.0
0.6904761904761905	0.6279761904761905	0.7827380952380952	115.0
0.9359712230215828	0.9719424460431655	0.9086330935251798	183.0
0.9327956989247311	0.8575268817204301	1.010752688172043	94.0
0.8175895765472313	1.009771986970684	0.9153094462540716	129.0
1.0	1.0	1.0	10.0
1.5588235294117647	0.7941176470588235	1.3235294117647058	64.0
0.41605839416058393	0.4927007299270073	0.6021897810218978	98.0
0.8725413060582219	0.7057435090479937	0.8465774980330448	119.0
0.8108108108108109	0.972972972972973	0.918918918918919	46.0
0.7520661157024794	0.7727272727272727	0.8099173553719008	91.0
0.9667093469910372	0.9884763124199744	0.9884763124199744	156.0
0.9119496855345912	1.0566037735849056	0.9308176100628931	100.0
1.1189499589827727	1.0648072190319935	1.1279737489745694	175.0
0.8408408408408409	0.8708708708708709	0.8828828828828829	148.0
0.625	0.375	0.625	36.0
0.8712574850299402	0.936377245508982	0.7986526946107785	129.0
0.7428571428571429	0.8571428571428571	1.0714285714285714	85.0
0.8072289156626506	0.7542168674698795	0.8698795180722891	160.0
1.0	1.0	1.0	34.0
0.9355509355509356	0.9376299376299376	0.9604989604989606	144.0
0.9627329192546584	1.0	0.9813664596273292	75.0
0.5448343079922028	0.7153996101364523	0.6276803118908382	117.0
0.953307392996109	0.7470817120622568	0.7782101167315175	134.0
0.7646258503401361	0.8380952380952381	0.7904761904761904	155.0
0.5	0.5	0.5	28.0
1.0	1.0	1.0	15.0
0.9741379310344828	0.9956896551724138	0.9310344827586207	98.0
0.9970059880239521	1.089820359281437	1.0	113.0
0.8626292466765141	0.8995568685376661	0.8389955686853766	150.0
0.8364705882352941	0.8258823529411765	0.8705882352941177	205.0
0.8593974175035868	0.9232424677187948	0.9013629842180775	247.0
0.9134275618374559	0.9063604240282686	0.8948763250883393	186.0
0.8095238095238095	0.7142857142857143	1.1428571428571428	49.0
0.7157464212678937	0.7484662576687117	0.7443762781186094	137.0
1.2299546142208775	1.1270801815431164	1.2102874432677762	129.0
0.7536231884057971	0.782608695652174	0.9130434782608695	91.0
0.8702031602708804	0.9830699774266366	1.010158013544018	173.0
0.9139280125195618	0.7433489827856025	0.8904538341158059	201.0
1.0763358778625953	0.9007633587786259	0.9236641221374046	89.0
0.7141162514827996	0.9383155397390273	0.8564650059311981	120.0
0.5531914893617021	0.6170212765957447	0.574468085106383	23.0
0.7580645161290323	0.8440860215053764	0.9408602150537635	115.0
0.9533333333333334	0.9706666666666667	0.9853333333333333	183.0
1.1176470588235294	0.9117647058823529	0.8529411764705882	49.0
0.8	0.9153846153846154	0.8598290598290599	164.0
0.7240506329113924	0.830379746835443	0.7721518987341772	93.0
0.9562189054726368	0.9144278606965174	0.8477611940298507	159.0
1.0	1.0	1.0	8.0
0.8866213151927438	0.9138321995464853	0.9727891156462585	130.0
0.9333333333333333	0.8333333333333334	0.9493150684931507	233.0
0.8009852216748768	0.812807881773399	0.8285714285714286	171.0
0.7133479212253829	0.7177242888402626	0.8577680525164114	111.0
1.7	1.2	1.0	39.0
0.9553203997648442	0.8406819517930629	0.8830099941211053	161.0
0.926829268292683	0.6829268292682927	0.8536585365853658	42.0
0.9003831417624522	0.7777777777777778	0.6628352490421456	129.0
0.8516250588789449	0.8087611869995289	0.784267545925577	220.0
0.7601442741208295	0.8674481514878268	0.8106402164111812	121.0
1.0	1.0	1.0	8.0
0.8333333333333334	1.2916666666666667	2.7083333333333335	55.0
0.9208791208791208	0.9684981684981685	0.9721611721611721	178.0
0.8422669853192216	0.8900648685558211	0.8436326391259815	232.0
0.8348424483882652	0.7826874320898225	0.8167330677290837	232.0
0.7562724014336918	0.7096774193548387	0.953405017921147	95.0
1.0	1.0	1.0	22.0
1.0	0.8870292887029289	0.9497907949790795	132.0
0.6590330788804071	0.7048346055979644	0.6997455470737913	128.0
1.0333333333333334	0.9888888888888889	0.9111111111111111	91.0
0.9036144578313253	0.8955823293172691	0.8594377510040161	128.0
1.0704225352112675	1.0035211267605635	1.0492957746478873	112.0
1.0085106382978724	0.9872340425531915	1.0	119.0
0.8177269478198713	0.910650464617584	0.9006433166547534	126.0
0.8318471337579618	0.8407643312101911	0.8738853503184714	158.0
0.7619047619047619	0.9285714285714286	0.9523809523809523	58.0
0.6268656716417911	0.5771144278606966	0.5522388059701493	79.0
0.7420965058236273	0.7603993344425957	0.8119800332778702	112.0
0.6571428571428571	0.6	0.8	68.0
0.8998646820027063	0.8227334235453315	0.8497970230040596	115.0
0.851063829787234	0.9787234042553191	1.3404255319148937	54.0
0.8888888888888888	0.5555555555555556	1.1111111111111112	38.0
0.9251592356687898	0.9187898089171974	0.8312101910828026	120.0
0.7551020408163265	0.6394557823129252	0.6394557823129252	35.0
0.8177966101694916	0.8411016949152542	0.760593220338983	131.0
0.8838383838383839	0.8767676767676768	0.9505050505050505	156.0
0.9664804469273743	0.8547486033519553	0.7653631284916201	120.0
1.2575757575757576	0.7424242424242424	0.8787878787878788	67.0
0.872236958443855	0.8779840848806366	0.8846153846153846	241.0
0.8191056910569106	0.8678861788617886	0.7886178861788617	107.0
1.1311154598825832	1.086105675146771	1.0019569471624266	115.0
0.9621212121212122	0.9090909090909091	0.9393939393939394	93.0
1.0	1.0	1.0	13.0
1.1870967741935483	1.0451612903225806	1.2193548387096773	86.0
0.9608669476219145	0.9789283564118001	0.925948223961469	182.0
0.883248730964467	0.7893401015228426	0.7284263959390863	113.0
0.8645374449339207	0.7533039647577092	0.7709251101321586	153.0
1.0	1.0	1.0	6.0
0.8730853391684902	0.8512035010940919	0.8315098468271335	188.0
1.0026385224274406	0.8970976253298153	0.9947229551451188	135.0
0.9218637992831541	0.8673835125448028	0.8931899641577061	116.0
0.75	0.675	0.5625	68.0
0.6517341040462428	0.7760115606936416	0.7369942196531792	116.0
0.8575916230366493	0.8910994764397906	1.0167539267015706	165.0
0.7174887892376681	0.7623318385650224	0.8878923766816144	127.0
0.9102564102564102	0.9358974358974359	0.8076923076923077	54.0
1.0	1.0	1.0	18.0
0.9408284023668639	0.757396449704142	0.9349112426035503	125.0
1.25	0.375	1.25	13.0
0.9274809160305344	0.8816793893129771	0.8396946564885496	169.0
0.8333333333333334	0.7941176470588235	0.8823529411764706	37.0
0.9673776662484316	0.7998745294855709	0.8989962358845671	163.0
0.7363636363636363	0.9090909090909091	0.7272727272727273	92.0
0.8577405857740585	0.8493723849372385	0.9651324965132496	126.0
0.7375886524822695	0.9716312056737588	0.6808510638297872	89.0
1.0	1.0	1.0	1.0
1.0	1.0	1.0	23.0
0.7974683544303798	0.7215189873417721	0.759493670886076	99.0
0.7543352601156069	0.7658959537572254	0.8554913294797688	145.0
0.817831590533847	0.7330764997248211	0.9521188772702256	243.0
0.9274570982839313	0.9477379095163807	0.8673946957878315	243.0
0.7194092827004219	0.8417721518987342	0.6223628691983122	126.0
0.8852097130242825	0.9448123620309051	0.8896247240618101	118.0
0.5581395348837209	0.5348837209302325	0.6046511627906976	70.0
0.8421733505821475	0.9650711513583441	0.8525226390685641	113.0
0.8491803278688524	0.7081967213114754	0.9278688524590164	131.0
0.7796934865900383	0.789272030651341	0.814176245210728	145.0
0.66	0.855	0.905	110.0
0.7272727272727273	0.7272727272727273	0.8181818181818182	61.0
0.9401840490797546	0.7944785276073619	0.8128834355828221	183.0
0.9050279329608939	0.5921787709497207	0.7318435754189944	113.0
1.0181132075471697	0.810566037735849	0.9441509433962264	229.0
0.9633099141295862	1.1436377829820452	0.9578454332552693	213.0
1.0	1.0	1.0	12.0
0.826530612244898	0.9030612244897959	0.9030612244897959	88.0
1.1429213483146068	1.0952808988764045	1.007191011235955	235.0
1.2650602409638554	1.0120481927710843	1.2771084337349397	80.0
0.908284023668639	0.849112426035503	0.9437869822485208	108.0
1.1129032258064515	0.9032258064516129	1.1290322580645162	77.0
1.0	1.0	1.0	5.0
0.8882618510158014	0.9379232505643341	0.8103837471783296	194.0
0.8514970059880239	0.9640718562874252	0.8479041916167664	200.0
1.0	1.0	1.0	25.0
1.0256410256410255	0.8974358974358975	0.9358974358974359	63.0
1.2045454545454546	1.4393939393939394	1.378787878787879	90.0
0.1	0.0	0.2	14.0
0.8367911479944675	0.9986168741355463	0.8105117565698479	148.0
1.0	1.0	1.0	24.0
0.8275862068965517	0.8120689655172414	0.9137931034482759	244.0
1.0	1.0	1.0	22.0
0.7941176470588235	0.7397058823529412	0.7470588235294118	112.0
0.7647058823529411	0.7815126050420168	0.82953181272509	195.0
1.0	1.0	1.0	4.0
0.7724719101123596	0.851123595505618	0.9129213483146067	89.0
0.5	1.5	1.5	16.0
1.3448275862068966	1.3103448275862069	1.3103448275862069	40.0
0.8333333333333334	0.9722222222222222	1.0555555555555556	86.0
0.7735849056603774	0.8490566037735849	1.0377358490566038	76.0
0.9606227106227107	0.9835164835164835	0.9331501831501832	197.0
0.8181818181818182	0.6136363636363636	0.6363636363636364	40.0
0.25	1.0	1.0	2.0
0.7164179104477612	0.7126865671641791	0.753731343283582	163.0
1.2439024390243902	1.0975609756097562	0.9146341463414634	49.0
0.9863874345549738	0.962652705061082	0.9071553228621292	240.0
0.9457900807381776	0.9711649365628604	1.0034602076124568	252.0
0.9393139841688655	0.8254177660510115	0.7233948988566403	201.0
0.73502722323049	0.8257713248638838	0.705989110707804	142.0
0.9133924799324039	1.0506970849176172	0.9670468948035488	243.0
1.0	1.0	1.0	8.0
0.8580645161290322	0.7322580645161291	0.9838709677419355	90.0
1.135135135135135	0.8378378378378378	1.0810810810810811	51.0
0.9029535864978903	0.8291139240506329	0.9345991561181435	120.0
0.9541284403669725	0.908256880733945	0.8899082568807339	99.0
1.035820895522388	1.0597014925373134	0.9671641791044776	102.0
0.8888888888888888	0.7810457516339869	0.9215686274509803	80.0
0.930379746835443	0.8949367088607595	0.769620253164557	164.0
0.9710773680404917	0.9996384671005062	0.9331164135936371	241.0
0.4898989898989899	0.6464646464646465	0.6313131313131313	39.0
0.8030534351145038	0.9251908396946565	0.9450381679389313	107.0
0.9009174311926605	0.8220183486238533	0.8018348623853211	120.0
0.7931034482758621	0.9310344827586207	0.8758620689655172	96.0
0.9050279329608939	0.8100558659217877	0.8603351955307262	103.0
1.1298076923076923	0.9903846153846154	0.8798076923076923	92.0
0.8156565656565656	0.9368686868686869	0.803030303030303	109.0
0.7073170731707317	0.6829268292682927	0.7073170731707317	47.0
0.9569160997732427	1.0	0.9047619047619048	106.0
1.34	0.74	0.82	71.0
0.950207468879668	0.9004149377593361	0.8672199170124482	107.0
0.768595041322314	0.8615702479338843	1.012396694214876	140.0
0.8281481481481482	0.9155555555555556	0.9007407407407407	141.0
0.746268656716418	0.6318407960199005	0.8109452736318408	89.0
0.7817589576547231	0.7882736156351792	0.7198697068403909	120.0
1.7142857142857142	0.8571428571428571	1.2142857142857142	42.0
0.8571428571428571	0.7619047619047619	1.0	38.0
0.871413390010627	0.6907545164718385	0.8310308182784272	204.0
0.7495175607873408	0.8178309532998842	0.8004631416441529	244.0
1.0	1.0	1.0	9.0
0.6923076923076923	0.6923076923076923	0.7692307692307693	43.0
0.9738493723849372	0.9550209205020921	0.8985355648535565	143.0
0.8192090395480226	0.9887005649717514	1.073446327683616	62.0
0.9	0.8	1.05	58.0
1.008230452674897	0.8518518518518519	0.7530864197530864	135.0
1.0	1.0	1.0	9.0
1.0	1.0	1.0	13.0
0.756838905775076	0.817629179331307	0.8662613981762918	138.0
0.8738738738738738	0.9279279279279279	1.015015015015015	148.0
0.9864661654135338	0.9107769423558897	0.9548872180451128	251.0
0.9855072463768116	1.0724637681159421	1.2753623188405796	45.0
0.7948717948717948	0.8321678321678322	0.831002331002331	200.0
1.0018315018315018	0.9139194139194139	1.0476190476190477	164.0
1.0069444444444444	0.9791666666666666	0.8958333333333334	110.0
0.9201101928374655	0.8815426997245179	0.9214876033057852	144.0
0.8020086083213773	0.7890961262553802	0.8378766140602583	108.0
0.8641975308641975	0.9012345679012346	0.8765432098765432	86.0
0.6875	0.6875	0.8125	18.0
0.9112860892388451	0.9034120734908136	0.952755905511811	203.0
0.7651515151515151	0.8446969696969697	0.7537878787878788	123.0
0.7758620689655172	0.8793103448275862	0.9655172413793104	61.0
0.8426395939086294	0.8426395939086294	1.0355329949238579	103.0
0.7292682926829268	0.7390243902439024	0.8414634146341463	104.0
1.5	1.5	1.25	40.0
0.7593220338983051	0.7610169491525424	0.8033898305084746	139.0
1.1926605504587156	0.9357798165137615	1.2477064220183487	82.0
0.8136645962732919	0.9089026915113871	0.8364389233954451	93.0
0.9420625724217845	0.9049826187717266	1.037079953650058	131.0
0.8251599147121536	0.9221748400852878	0.920042643923241	195.0
0.7991452991452992	1.017094017094017	0.7585470085470085	183.0
0.7297297297297297	0.8438438438438438	0.6816816816816816	88.0
1.0	1.0	1.0	28.0
0.9216494845360824	1.1154639175257732	1.0762886597938144	109.0
0.6923076923076923	0.7384615384615385	0.7461538461538462	50.0
0.8683853459972863	0.9199457259158752	0.7137042062415196	157.0
0.7206703910614525	0.664804469273743	0.5921787709497207	94.0
0.863013698630137	0.7853881278538812	0.9269406392694064	80.0
0.5138121546961326	0.6629834254143646	0.47513812154696133	53.0
0.9271332694151486	0.9232981783317353	0.9314477468839885	240.0
1.0714285714285714	1.0	0.8928571428571429	35.0
0.8383838383838383	1.0527497194163862	0.9304152637485971	105.0
0.8508771929824561	0.9072681704260651	0.7355889724310777	110.0
1.0224438902743143	0.9625935162094763	0.8528678304239401	149.0
1.0845360824742267	1.0494845360824743	0.9670103092783505	114.0
0.8709677419354839	0.7270471464019851	0.7295285359801489	113.0
0.8456591639871383	0.9614147909967846	0.9581993569131833	111.0
1.0	1.0	1.0	4.0
1.0	1.1428571428571428	1.1428571428571428	57.0
0.4482758620689655	0.4827586206896552	0.6896551724137931	42.0
0.7574421168687983	0.7872105843439912	0.7794928335170893	168.0
0.8633093525179856	0.9712230215827338	0.9136690647482014	99.0
0.6830601092896175	0.7431693989071039	0.7131147540983607	93.0
1.0	1.0	1.0	9.0
1.0	1.0	1.0	14.0
0.9136363636363637	0.9	0.9590909090909091	80.0
0.9466666666666667	0.92	0.8533333333333334	91.0
1.0044910179640718	0.938622754491018	0.9221556886227545	143.0
0.5909090909090909	0.7136363636363636	0.8045454545454546	39.0
1.0	0.6923076923076923	0.8076923076923077	26.0
0.8317757009345794	0.8582017402513696	0.8466000644537545	240.0
1.0909090909090908	0.8181818181818182	1.0	69.0
0.8931818181818182	0.8443181818181819	0.9375	185.0
0.9213051823416507	0.9155470249520153	0.8349328214971209	142.0
0.8669201520912547	0.7376425855513308	0.9277566539923955	102.0
0.0	2.0	1.0	25.0
0.8014796547472256	0.8594327990135635	0.6966707768187423	174.0
0.7875894988066826	0.7899761336515513	0.7183770883054893	99.0
0.8244013683010262	0.8129988597491448	0.7616875712656784	156.0
1.1374325782092773	1.1089536138079827	1.1354908306364617	309.0
1.0620689655172413	1.0482758620689656	0.993103448275862	121.0
0.15625	0.15625	0.225	39.0
0.9485420240137221	0.8679245283018868	0.8319039451114922	171.0
0.8707926167209555	0.8751357220412594	0.9305103148751357	179.0
0.5714285714285714	0.9523809523809523	0.8412698412698413	62.0
1.1568627450980393	0.9215686274509803	0.6862745098039216	32.0
0.9142857142857143	0.889795918367347	0.7714285714285715	126.0
1.0	1.0	1.0	15.0
0.8825831702544031	0.9980430528375733	0.8473581213307241	104.0
0.9226519337016574	0.9252018699532512	0.9260518487037824	196.0
0.8155555555555556	0.7822222222222223	0.9422222222222222	133.0
0.9344262295081968	1.1147540983606556	1.2131147540983607	43.0
0.7938775510204081	0.8530612244897959	0.8183673469387756	104.0
0.924956369982548	0.9301919720767888	1.0261780104712042	189.0
0.8082901554404145	0.7694300518134715	0.7979274611398963	118.0
0.9796582587469488	0.9210740439381611	1.0227827502034175	226.0
0.7383512544802867	0.8709677419354839	0.8960573476702509	87.0
0.7943009795191451	0.8548530721282279	0.8940338379341051	213.0
1.3076923076923077	1.3846153846153846	1.4615384615384615	43.0
0.9653846153846154	0.8346153846153846	0.926923076923077	135.0
0.7584541062801933	0.7246376811594203	0.8115942028985508	108.0
0.8045977011494253	0.7471264367816092	0.9655172413793104	68.0
0.847953216374269	0.543859649122807	0.8538011695906432	93.0
0.7777777777777778	0.8680555555555556	0.8402777777777778	115.0
0.5102040816326531	0.8367346938775511	1.0408163265306123	53.0
0.8275862068965517	0.6206896551724138	0.8620689655172413	24.0
0.5166666666666667	0.5166666666666667	0.7	55.0
1.0	1.0	1.0	5.0
1.0	1.0	1.0	27.0
1.1165146909827761	1.0972644376899696	0.8368794326241135	219.0
0.6407766990291263	0.7669902912621359	0.7766990291262136	88.0
0.7083333333333334	0.8333333333333334	0.875	59.0
1.0758928571428572	1.0625	1.0267857142857142	79.0
0.995850622406639	0.9276164130935916	0.9557399723374828	244.0
0.9535962877030162	1.0301624129930393	0.8584686774941995	140.0
1.0	0.8	1.6	37.0
0.8168789808917197	0.8614649681528662	0.732484076433121	147.0
1.2222222222222223	0.5925925925925926	1.5185185185185186	42.0
1.0615114235500878	0.9261862917398945	0.8242530755711776	189.0
0.8	0.8533632286995516	0.8982062780269058	232.0
0.8743243243243243	0.8391891891891892	0.85	109.0
0.6875	0.8809523809523809	0.7916666666666666	87.0
1.5238095238095237	1.0	1.0714285714285714	47.0
0.75	0.9523809523809523	0.8511904761904762	106.0
0.5	0.8333333333333334	1.0	38.0
0.75	1.0208333333333333	0.9270833333333334	92.0
0.8841059602649006	0.9486754966887417	0.9735099337748344	140.0
1.0	1.0	1.0	13.0
0.7953667953667953	0.7837837837837838	0.8494208494208494	99.0
0.8679950186799502	0.7870485678704857	0.8188044831880449	127.0
0.92	0.7466666666666667	0.5733333333333334	65.0
0.9681528662420382	0.7659235668789809	0.9235668789808917	146.0
0.8372093023255814	1.069767441860465	1.0930232558139534	83.0
0.7023809523809523	0.6944444444444444	0.876984126984127	109.0
0.9116582186821144	0.998551774076756	0.999275887038378	224.0
1.0	0.8333333333333334	0.8333333333333334	29.0
0.8980667838312829	0.945518453427065	0.8383128295254832	184.0
1.0	1.0	1.0	8.0
0.9708141321044547	0.9124423963133641	0.9600614439324117	160.0
0.2	0.4	1.0	34.0
0.8990536277602523	0.9305993690851735	0.9022082018927445	109.0
0.6589147286821705	0.710594315245478	0.7571059431524548	103.0
0.9418960244648318	0.8318042813455657	0.8027522935779816	190.0
1.0	1.0	1.0	6.0
1.0126582278481013	0.9493670886075949	0.9113924050632911	85.0
0.9043478260869565	0.8826086956521739	0.8521739130434782	98.0
1.0	1.0	1.0	12.0
1.0	0.6666666666666666	0.6666666666666666	17.0
0.6468842729970327	0.6320474777448071	0.5816023738872403	93.0
0.9609120521172638	0.762214983713355	0.8957654723127035	109.0
0.8916083916083916	0.986013986013986	0.8531468531468531	103.0
0.8317073170731707	0.8853658536585366	0.8804878048780488	145.0
0.9316770186335404	0.8757763975155279	1.0062111801242235	124.0
0.8982300884955752	0.9236725663716814	0.7920353982300885	170.0
0.7975609756097561	0.7804878048780488	0.8146341463414634	104.0
0.9381443298969072	0.9626288659793815	0.8492268041237113	129.0
0.8356481481481481	0.9398148148148148	0.8726851851851852	132.0
0.8531468531468531	0.958041958041958	0.8391608391608392	152.0
0.8682352941176471	0.8305882352941176	0.8188235294117647	118.0
0.6730158730158731	0.8984126984126984	0.8920634920634921	103.0
0.8224932249322493	0.8048780487804879	0.8292682926829268	174.0
1.018181818181818	0.9636363636363636	0.9272727272727272	61.0
0.7965533748204883	0.8109143130684539	0.9205361416945907	223.0
0.8439716312056738	0.5851063829787234	0.6453900709219859	51.0
1.0	1.0	1.0	11.0
1.0851063829787233	1.297872340425532	1.2340425531914894	52.0
0.8344827586206897	0.8620689655172413	0.7689655172413793	112.0
1.0	1.0	1.0	18.0
1.0	0.8571428571428571	0.8571428571428571	57.0
0.8621359223300971	0.9087378640776699	0.9844660194174757	124.0
0.25	0.25	0.75	22.0
0.7536231884057971	0.8633540372670807	0.855072463768116	157.0
1.0	0.9505582137161085	0.8341307814992025	139.0
0.8052325581395349	0.8343023255813954	0.9069767441860465	91.0
1.131578947368421	0.9824561403508771	0.9824561403508771	88.0
1.0533333333333332	1.0666666666666667	0.8133333333333334	63.0
0.5217391304347826	0.6956521739130435	0.9130434782608695	28.0
1.0172143974960877	0.852112676056338	0.9992175273865415	174.0
0.8169491525423729	0.7796610169491526	0.9423728813559322	110.0
1.0	1.0	2.0	24.0
0.8476702508960573	0.8853046594982079	0.8512544802867383	167.0
0.9280575539568345	1.0071942446043165	1.014388489208633	90.0
0.6823529411764706	0.6911764705882353	0.8176470588235294	79.0
0.9667221297836939	0.930116472545757	0.8469217970049917	164.0
0.9792993630573248	1.1464968152866242	0.9570063694267515	130.0
0.2	0.2	0.4	20.0
0.9241516966067864	0.9021956087824351	0.9481037924151696	190.0
0.8326693227091634	0.8565737051792829	0.8605577689243028	125.0
0.9180113388573921	0.8791975577845617	0.8499781945050152	224.0
0.868995633187773	0.759825327510917	0.7030567685589519	48.0
0.8566978193146417	0.8473520249221184	0.9657320872274143	95.0
1.0	1.0	1.0	5.0
0.82	0.9	0.94	41.0
0.803088803088803	0.9845559845559846	0.9433719433719434	172.0
0.47115384615384615	0.46153846153846156	0.5336538461538461	69.0
1.0	0.5	0.5	27.0
1.5119047619047619	1.4523809523809523	1.1666666666666667	64.0
0.0	0.0	0.0	13.0
0.8526570048309179	0.7705314009661836	0.751207729468599	135.0
1.0544554455445545	1.1287128712871286	0.8910891089108911	60.0
1.0	1.0	1.0	22.0
1.0808080808080809	0.9797979797979798	0.9494949494949495	82.0
0.9772727272727273	1.1590909090909092	0.9318181818181818	63.0
0.7904442581726739	0.7715842414082146	0.769907795473596	237.0
0.9153439153439153	0.7936507936507936	0.9206349206349206	120.0
0.8181818181818182	0.7443181818181818	0.9715909090909091	88.0
0.7317073170731707	0.7804878048780488	0.8327526132404182	133.0


==> ncrCM_praline-package-2020-05-18.tex <==
ports/kieler	nodes/kieler	mixed/kieler	vtcs
0.0	0.0	0.0	8.0
0.751269035532995	0.8959390862944162	0.7715736040609137	169.0
0.2222222222222222	1.3703703703703705	0.8148148148148148	50.0
0.6277777777777778	0.7555555555555555	0.8555555555555555	104.0
0.8784530386740331	0.7265193370165746	0.8066298342541437	44.0
0.0	0.0	0.0	8.0
0.5933852140077821	0.7120622568093385	0.688715953307393	201.0
0.5805739514348786	0.7373068432671082	0.6556291390728477	197.0
0.4602649006622517	0.48344370860927155	0.33774834437086093	119.0
0.6842105263157895	1.0526315789473684	0.7368421052631579	27.0
0.6746765249537893	0.7190388170055453	0.7578558225508318	156.0
0.3684210526315789	0.47719298245614034	0.4280701754385965	119.0
0.22110552763819097	0.2613065326633166	0.2864321608040201	86.0
0.37540453074433655	0.5016181229773463	0.39805825242718446	121.0
0.8090909090909091	0.7909090909090909	0.8454545454545455	95.0
0.6858054226475279	0.6267942583732058	0.7208931419457735	231.0
0.7918918918918919	0.7648648648648648	0.845945945945946	169.0
0.7724867724867724	0.7301587301587301	0.798941798941799	126.0
0.0	0.3333333333333333	0.0	28.0
1.0443037974683544	1.0443037974683544	0.8227848101265823	101.0
0.6153846153846154	1.5384615384615385	0.6153846153846154	27.0
1.0	1.0	1.0	11.0
0.7853107344632768	0.9096045197740112	0.7796610169491526	112.0
0.38596491228070173	0.5614035087719298	0.3333333333333333	77.0
0.7355679702048417	0.8472998137802608	0.7728119180633147	134.0
0.8271604938271605	0.8518518518518519	1.0740740740740742	86.0
0.6135922330097088	0.7320388349514563	0.6466019417475728	131.0
0.4752851711026616	0.6045627376425855	0.4068441064638783	122.0
1.0	1.0	1.0	5.0
0.8611111111111112	0.8638888888888889	0.7611111111111111	86.0
0.5925925925925926	0.8888888888888888	0.5925925925925926	48.0
0.7	0.85	0.65	26.0
0.26666666666666666	0.5555555555555556	0.13333333333333333	28.0
0.7025316455696202	0.7278481012658228	0.6329113924050633	134.0
0.42813455657492355	0.5657492354740061	0.45871559633027525	133.0
0.3333333333333333	0.8333333333333334	0.3333333333333333	41.0
0.6441281138790036	0.6156583629893239	0.6156583629893239	93.0
0.7873303167420814	0.7285067873303167	0.6289592760180995	154.0
0.5653266331658291	0.7361809045226131	0.5979899497487438	194.0
0.7512776831345827	0.8100511073253833	0.7461669505962522	209.0
0.3870967741935484	0.4055299539170507	0.391705069124424	110.0
0.8952380952380953	0.9023809523809524	0.8833333333333333	113.0
0.6857142857142857	0.5904761904761905	0.5238095238095238	62.0
0.7072147651006712	0.6895973154362416	0.7483221476510067	202.0
0.8287292817679558	0.6408839779005525	0.6519337016574586	134.0
1.0	1.0	1.0	18.0
0.7409972299168975	0.7853185595567868	0.889196675900277	105.0
0.5575757575757576	0.6303030303030303	0.6272727272727273	139.0
0.6826347305389222	0.842814371257485	0.7949101796407185	180.0
0.5939849624060151	0.6541353383458647	0.8195488721804511	194.0
0.8154981549815498	0.7970479704797048	0.788929889298893	354.0
1.0	1.0	1.0	11.0
0.6201550387596899	0.627906976744186	0.627906976744186	98.0
0.7030685920577617	0.8402527075812274	0.6877256317689531	235.0
0.5778210116731517	0.6478599221789884	0.6361867704280155	163.0
0.7292307692307692	0.7753846153846153	0.6707692307692308	168.0
0.8074074074074075	0.6962962962962963	0.7481481481481481	128.0
0.7630331753554502	0.7582938388625592	0.7227488151658767	205.0
0.6486486486486487	0.5135135135135135	0.5540540540540541	50.0
0.6340694006309149	0.6435331230283912	0.6041009463722398	218.0
0.5873493975903614	0.5753012048192772	0.5060240963855421	80.0
0.6737160120845922	0.7341389728096677	0.7477341389728097	170.0
0.41798941798941797	0.6058201058201058	0.4947089947089947	113.0
1.0	1.0	1.0	17.0
0.0	0.0	0.0	5.0
0.4690265486725664	0.6017699115044248	0.504424778761062	147.0
0.8726937269372693	0.8293357933579336	0.8450184501845018	199.0
0.6277777777777778	0.7444444444444445	0.8777777777777778	63.0
0.0	0.14285714285714285	0.0	36.0
0.1935483870967742	0.2903225806451613	0.13978494623655913	44.0
1.0	1.0	1.0	13.0
0.7274569402228976	0.7244174265450861	0.7304964539007093	226.0
0.5867768595041323	0.7107438016528925	0.6735537190082644	115.0
0.7009966777408638	0.8230897009966778	0.643687707641196	241.0
0.8017751479289941	0.691715976331361	0.7153846153846154	241.0
0.6455479452054794	0.5993150684931506	0.6095890410958904	184.0
0.6088560885608856	0.5387453874538746	0.6457564575645757	156.0
0.7871485943775101	1.0160642570281124	0.6706827309236948	134.0
0.5297872340425532	0.5765957446808511	0.551063829787234	168.0
0.8511904761904762	0.75	0.9523809523809523	123.0
0.5528089887640449	0.6247191011235955	0.5752808988764045	146.0
0.4272930648769575	0.5615212527964206	0.5480984340044742	144.0
0.325	0.6	0.375	55.0
0.5833333333333334	0.875	0.4166666666666667	55.0
1.0	1.0	1.0	7.0
0.5779376498800959	0.6306954436450839	0.645083932853717	159.0
0.7324955116696589	0.895870736086176	0.6588868940754039	194.0
0.0	0.5	0.0	17.0
0.6949152542372882	0.7796610169491526	0.7457627118644068	86.0
1.0	1.0	1.0	18.0
0.8666666666666667	0.6533333333333333	0.6933333333333334	87.0
0.5585585585585585	0.9099099099099099	0.6396396396396397	190.0
0.0	0.2	0.0	35.0
0.6557377049180327	0.825136612021858	0.6666666666666666	122.0
0.8137254901960784	0.8774509803921569	0.8480392156862745	152.0
0.7295597484276729	0.8427672955974843	0.8238993710691824	120.0
0.680327868852459	0.6885245901639344	0.6229508196721312	124.0
0.8013245033112583	0.7218543046357616	0.7112582781456953	225.0
0.5476190476190477	0.6904761904761905	0.5595238095238095	73.0
0.3333333333333333	1.0	0.6666666666666666	38.0
0.84	1.0	0.64	45.0
0.2857142857142857	0.5714285714285714	0.5714285714285714	15.0
0.5446009389671361	0.7323943661971831	0.6572769953051644	130.0
0.0	4.0	0.0	20.0
0.8214285714285714	0.9	0.8285714285714286	120.0
0.8823529411764706	1.411764705882353	1.1568627450980393	60.0
0.4448979591836735	0.46122448979591835	0.3673469387755102	102.0
0.6729411764705883	0.7423529411764705	0.6023529411764705	254.0
0.8167053364269141	0.9269141531322506	0.9083526682134571	157.0
0.5632183908045977	0.7471264367816092	0.5632183908045977	102.0
0.7124824684431977	0.7461430575035063	0.7524544179523142	230.0
0.7422852376980817	0.7364470391993327	0.7597998331943286	244.0
1.0	1.0	1.0	8.0
0.7685185185185185	0.6712962962962963	0.7962962962962963	144.0
0.7010309278350515	1.0515463917525774	0.7731958762886598	80.0
0.8316831683168316	0.7623762376237624	0.9207920792079208	112.0
0.6363636363636364	0.5	0.5	39.0
0.3160377358490566	0.42452830188679247	0.330188679245283	91.0
0.9056122448979592	0.9017857142857143	0.8303571428571429	121.0
0.9071347678369196	1.0056625141562854	0.9365798414496036	132.0
0.6953125	0.6796875	0.4453125	89.0
0.7684729064039408	0.8866995073891626	0.9630541871921182	170.0
0.7534246575342466	0.7031963470319634	0.7853881278538812	53.0
0.57875	0.805	0.6	171.0
0.7424812030075187	0.6898496240601504	0.650375939849624	170.0
0.7837837837837838	0.8108108108108109	0.5135135135135135	63.0
0.7506631299734748	0.8222811671087533	0.6710875331564987	187.0
0.7510917030567685	0.7379912663755459	0.8296943231441049	147.0
0.18627450980392157	0.3333333333333333	0.2549019607843137	79.0
0.628099173553719	0.5867768595041323	0.6714876033057852	168.0
1.4166666666666667	1.3333333333333333	1.1666666666666667	48.0
1.0	1.0	1.0	18.0
0.8170212765957446	0.5829787234042553	0.625531914893617	111.0
0.7678571428571429	0.7678571428571429	0.6607142857142857	49.0
0.7590361445783133	0.7349397590361446	0.763855421686747	186.0
0.5566666666666666	0.6466666666666666	0.62	142.0
0.68	0.84	0.6333333333333333	69.0
0.5686274509803921	0.43137254901960786	0.7450980392156863	62.0
0.9492063492063492	0.9809523809523809	0.8507936507936508	122.0
0.5635451505016722	0.6739130434782609	0.5551839464882943	127.0
0.5	1.6666666666666667	0.6666666666666666	60.0
0.7078313253012049	0.9216867469879518	0.9186746987951807	193.0
0.43478260869565216	0.8405797101449275	0.4927536231884058	47.0
1.144927536231884	1.4927536231884058	0.8840579710144928	61.0
1.0	1.0	1.0	43.0
1.0	1.0	1.0	21.0
0.6320621468926554	0.702683615819209	0.8248587570621468	237.0
0.35	0.675	0.525	40.0
0.0	1.0	0.0	21.0
0.6965317919075145	0.8121387283236994	0.7263969171483622	246.0
0.36	0.88	0.56	55.0
0.6825842696629213	0.6966292134831461	0.6544943820224719	163.0
0.6392156862745098	0.6980392156862745	0.6862745098039216	145.0
0.9642857142857143	1.0	0.8571428571428571	37.0
0.4	0.8	1.6	41.0
0.6918844566712518	0.7579092159559835	0.782668500687758	149.0
0.9032258064516129	0.9354838709677419	0.8709677419354839	44.0
0.6076923076923076	0.8538461538461538	0.7	107.0
0.7365269461077845	0.8922155688622755	1.0239520958083832	97.0
0.9154929577464789	0.676056338028169	0.9084507042253521	114.0
0.8067226890756303	0.9915966386554622	0.680672268907563	169.0
1.0	1.0	1.0	8.0
0.4959349593495935	0.5691056910569106	0.6747967479674797	109.0
0.84472049689441	0.6211180124223602	0.7577639751552795	120.0
0.6636363636363637	0.7568181818181818	0.6772727272727272	188.0
1.0	1.0	1.0	10.0
0.7469879518072289	0.7349397590361446	0.8382099827882961	158.0
1.0	1.0	1.0	2.0
0.46153846153846156	0.8461538461538461	0.46153846153846156	34.0
0.8418230563002681	0.8123324396782842	0.9410187667560321	178.0
0.5	0.7333333333333333	0.643859649122807	170.0
0.8888888888888888	0.8888888888888888	0.8888888888888888	65.0
0.0	0.6666666666666666	0.0	8.0
0.6265560165975104	0.9294605809128631	0.4896265560165975	111.0
0.7797619047619048	0.8154761904761905	0.7559523809523809	113.0
0.3317307692307692	0.4951923076923077	0.4519230769230769	91.0
0.47706422018348627	0.5596330275229358	0.5114678899082569	131.0
0.6071428571428571	0.8154761904761905	0.7321428571428571	102.0
0.4166666666666667	0.75	0.25	33.0
0.0	0.0	0.0	14.0
0.75	0.5	0.5	24.0
0.4090909090909091	0.6818181818181818	0.5454545454545454	87.0
1.0	1.0	1.0	8.0
0.5611702127659575	0.6569148936170213	0.625	190.0
1.0	1.0	1.0	14.0
0.31343283582089554	0.24875621890547264	0.2885572139303483	99.0
0.7945652173913044	0.9206521739130434	0.7358695652173913	127.0
0.3961661341853035	0.5782747603833865	0.3929712460063898	115.0
0.4722222222222222	0.5277777777777778	0.6944444444444444	58.0
0.9635036496350365	0.8321167883211679	0.5401459854014599	120.0
0.7573529411764706	0.8406862745098039	0.8725490196078431	153.0
0.796875	0.921875	0.53125	50.0
0.4650537634408602	0.510752688172043	0.48655913978494625	105.0
0.5046511627906977	0.7604651162790698	0.6674418604651163	79.0
0.8770595690747782	0.9505703422053232	0.9328263624841572	121.0
0.8047904191616766	0.7868263473053893	0.7005988023952096	130.0
0.5795918367346938	0.5142857142857142	0.6224489795918368	168.0
0.7577142857142857	0.832	0.7668571428571429	202.0
0.26666666666666666	0.8222222222222222	0.26666666666666666	67.0
0.6528497409326425	0.6735751295336787	0.5958549222797928	123.0
0.96	1.24	1.12	66.0
0.7869565217391304	0.8695652173913043	0.7260869565217392	97.0
0.652241112828439	0.7727975270479135	0.6955177743431221	172.0
0.4	0.8	0.5	66.0
0.6081330868761553	0.6469500924214417	0.6266173752310537	173.0
0.7796610169491526	0.8587570621468926	0.8135593220338984	99.0
0.8255813953488372	0.8604651162790697	0.6569767441860465	126.0
0.0	3.0	0.0	18.0
0.0	0.0	0.0	15.0
0.47368421052631576	1.3157894736842106	0.5789473684210527	26.0
0.6257142857142857	0.6228571428571429	0.6114285714285714	138.0
1.0	1.0	1.0	7.0
0.6440903054448871	0.6613545816733067	0.7065073041168659	168.0
0.5	1.0	0.38461538461538464	30.0
0.7142857142857143	1.2857142857142858	1.4285714285714286	54.0
0.7266666666666667	0.7733333333333333	0.8133333333333334	113.0
0.4411764705882353	1.5	1.0	37.0
0.6020408163265306	0.6913265306122449	0.6964285714285714	148.0
0.330188679245283	0.6320754716981132	0.6792452830188679	70.0
0.8881118881118881	0.8811188811188811	0.6433566433566433	133.0
0.6195652173913043	0.8043478260869565	0.5217391304347826	132.0
0.6847635726795096	0.7985989492119089	0.7250437828371279	157.0
0.3448275862068966	1.0344827586206897	0.3793103448275862	67.0
1.0	1.0	1.0	18.0
0.352112676056338	0.5211267605633803	0.5211267605633803	71.0
0.4970414201183432	0.6035502958579881	0.4911242603550296	82.0
0.7022900763358778	0.7595419847328244	0.6335877862595419	117.0
0.381294964028777	0.5719424460431655	0.6187050359712231	126.0
0.7336032388663968	0.7522267206477733	0.8024291497975709	234.0
0.520891364902507	0.584958217270195	0.5793871866295265	143.0
0.6666666666666666	0.6941176470588235	0.5568627450980392	93.0
0.58	0.7	0.6	37.0
0.9767441860465116	1.0232558139534884	1.069767441860465	99.0
0.3936651583710407	0.47058823529411764	0.4660633484162896	100.0
0.35175879396984927	0.32663316582914576	0.38190954773869346	91.0
0.9281842818428184	0.9701897018970189	0.9742547425474255	122.0
0.5607779578606159	0.6790923824959482	0.6256077795786061	169.0
0.87248322147651	0.8926174496644296	0.8657718120805369	122.0
0.6952789699570815	0.7296137339055794	0.703862660944206	95.0
0.9053254437869822	0.9053254437869822	0.7751479289940828	126.0
0.6463768115942029	0.8202898550724638	0.6376811594202898	157.0
0.5	1.0	1.0	14.0
0.27586206896551724	0.5172413793103449	0.1724137931034483	63.0
0.4264705882352941	0.7647058823529411	0.5245098039215687	104.0
0.694300518134715	0.7305699481865285	0.47668393782383417	113.0
0.6666666666666666	2.3333333333333335	1.3333333333333333	27.0
0.13636363636363635	0.5	0.09090909090909091	55.0
0.6055900621118012	0.6335403726708074	0.6128364389233955	148.0
0.6086956521739131	1.7826086956521738	0.9565217391304348	60.0
0.9070735090152566	0.9583911234396671	0.8543689320388349	186.0
0.8395061728395061	1.0802469135802468	0.7592592592592593	141.0
0.9678571428571429	1.2214285714285715	1.0803571428571428	153.0
0.6138613861386139	0.698019801980198	0.7326732673267327	115.0
0.7217473884140551	0.8262108262108262	0.7359924026590693	162.0
0.958904109589041	0.8835616438356164	0.863013698630137	122.0
0.7419354838709677	0.7258064516129032	0.6129032258064516	43.0
0.6782608695652174	0.6695652173913044	0.8173913043478261	107.0
0.6354515050167224	0.6413043478260869	0.6705685618729097	245.0
0.7879604672057502	0.8382749326145552	0.6891284815813118	245.0
1.0	1.0	1.0	11.0
0.7333333333333333	0.5777777777777777	0.8444444444444444	53.0
0.72	1.0	0.8577777777777778	142.0
0.897196261682243	0.8691588785046729	0.897196261682243	107.0
0.8636363636363636	1.0625	0.8636363636363636	113.0
1.0	1.0	1.0	32.0
0.4642857142857143	0.47619047619047616	0.2857142857142857	77.0
0.6446280991735537	0.6033057851239669	0.7272727272727273	129.0
0.6766467065868264	0.8263473053892215	0.5748502994011976	118.0
0.4588744588744589	0.5541125541125541	0.551948051948052	135.0
0.698992443324937	0.7405541561712846	0.5957178841309824	182.0
0.6627218934911243	0.9526627218934911	0.727810650887574	96.0
0.8691588785046729	0.8878504672897196	0.794392523364486	80.0
0.37962962962962965	0.6574074074074074	0.46296296296296297	52.0
1.0	1.0	1.0	10.0
0.9035087719298246	0.9210526315789473	0.9956140350877193	133.0
0.8223776223776224	0.8391608391608392	0.737062937062937	241.0
0.6706586826347305	0.6586826347305389	0.6287425149700598	111.0
0.65625	0.875	0.59375	41.0
0.8627450980392157	0.9019607843137255	0.6470588235294118	87.0
0.8040313549832027	0.7928331466965286	0.786114221724524	219.0
0.5664160401002506	0.6892230576441103	0.6240601503759399	165.0
1.0	1.0	1.0	5.0
0.5735294117647058	1.0588235294117647	0.8382352941176471	58.0
0.8905908096280087	0.7614879649890591	0.7571115973741794	164.0
0.49162011173184356	0.7318435754189944	0.41899441340782123	92.0
0.4208955223880597	0.564179104477612	0.5522388059701493	94.0
0.8604651162790697	0.8905608755129959	0.8440492476060192	112.0
1.0	1.2	1.2	62.0
0.0	0.0	0.0	14.0
0.7909090909090909	0.7454545454545455	0.9272727272727272	105.0
0.43956043956043955	0.6813186813186813	0.46153846153846156	82.0
0.52	0.39	0.38	56.0
1.0	1.0	1.0	18.0
0.724025974025974	0.9172077922077922	0.8425324675324676	197.0
0.6923076923076923	0.7980769230769231	0.6009615384615384	105.0
0.5811965811965812	0.7948717948717948	0.5726495726495726	105.0
0.7687074829931972	0.8231292517006803	0.7097505668934241	164.0
1.0	1.0	3.0	31.0
0.7922077922077922	0.8363636363636363	0.8	156.0
0.37339055793991416	0.5407725321888412	0.3562231759656652	107.0
1.125	1.125	1.75	78.0
0.7583892617449665	0.8523489932885906	0.7248322147651006	130.0
0.8718487394957983	0.7478991596638656	0.819327731092437	128.0
0.4781609195402299	0.49885057471264366	0.496551724137931	144.0
0.7894736842105263	0.7485380116959064	0.5672514619883041	91.0
0.515695067264574	0.7533632286995515	0.7847533632286996	38.0
0.7514450867052023	0.6127167630057804	0.5433526011560693	105.0
0.7134146341463414	0.7134146341463414	0.5914634146341463	69.0
0.8827751196172249	0.9976076555023924	0.9019138755980861	113.0
0.8272425249169435	0.6079734219269103	0.7475083056478405	156.0
0.5210084033613446	0.6218487394957983	0.5756302521008403	115.0
0.7630522088353414	0.7108433734939759	0.7530120481927711	217.0
0.043478260869565216	0.391304347826087	0.043478260869565216	40.0
0.4406779661016949	0.847457627118644	0.6949152542372882	43.0
1.2142857142857142	1.0714285714285714	0.9285714285714286	92.0
1.0395387149917628	1.1334431630971993	0.9110378912685337	166.0
0.521505376344086	0.8225806451612904	0.6935483870967742	150.0
0.6226415094339622	0.41509433962264153	0.49056603773584906	95.0
1.0	1.0	1.0	2.0
0.3333333333333333	0.5238095238095238	0.3333333333333333	47.0
0.8313953488372093	0.8633720930232558	0.7587209302325582	147.0
0.40816326530612246	0.6326530612244898	0.20408163265306123	76.0
0.6	1.2	0.5	69.0
0.6470588235294118	0.35294117647058826	0.4411764705882353	49.0
0.6510721247563352	0.6861598440545809	0.7816764132553606	174.0
0.6305418719211823	0.6305418719211823	0.5714285714285714	92.0
0.5445859872611465	0.7006369426751592	0.60828025477707	145.0
1.0	10.0	1.0	13.0
0.6677018633540373	0.6180124223602484	0.7453416149068323	139.0
1.4736842105263157	0.7894736842105263	1.105263157894737	40.0
0.9448373408769448	0.9321074964639321	0.9603960396039604	123.0
0.6	0.5	0.5	60.0
0.6666666666666666	1.037037037037037	0.7037037037037037	40.0
0.5531914893617021	0.5531914893617021	0.3617021276595745	47.0
0.5526315789473685	0.7105263157894737	0.5789473684210527	51.0
0.7409261576971214	0.7966207759699625	0.6470588235294118	239.0
0.3135593220338983	0.4364406779661017	0.4491525423728814	84.0
0.510548523206751	0.5274261603375527	0.48945147679324896	115.0
0.7858472998137802	0.7150837988826816	0.6536312849162011	187.0
0.9080882352941176	0.7904411764705882	0.8088235294117647	160.0
0.04	0.08	0.05	39.0
0.44155844155844154	0.4675324675324675	0.4805194805194805	54.0
0.8070175438596491	0.9210526315789473	0.7894736842105263	102.0
0.0	0.0	0.0	21.0
0.8878026070763501	0.883147113594041	0.8389199255121043	313.0
0.7704918032786885	0.8114754098360656	0.7704918032786885	100.0
0.5655172413793104	0.5747126436781609	0.503448275862069	144.0
0.6036036036036037	0.5045045045045045	0.45045045045045046	93.0
0.6599162011173184	0.6668994413407822	0.678072625698324	234.0
0.7840909090909091	0.7897727272727273	0.75	131.0
0.46368715083798884	0.5754189944134078	0.5418994413407822	97.0
0.5940054495912807	0.6457765667574932	0.6566757493188011	171.0
0.875	0.7613636363636364	0.7840909090909091	133.0
0.7521613832853026	0.7204610951008645	0.7031700288184438	141.0
0.46511627906976744	0.7209302325581395	0.46511627906976744	80.0
1.0	1.0	1.0	35.0
0.8539325842696629	0.8426966292134831	0.7865168539325843	131.0
0.47368421052631576	0.6842105263157895	0.5263157894736842	25.0
0.6530612244897959	0.9285714285714286	0.5918367346938775	84.0
0.42408376963350786	0.44502617801047123	0.38219895287958117	89.0
0.5707762557077626	0.6757990867579908	0.4977168949771689	27.0
0.7095990279465371	0.9234507897934386	0.827460510328068	224.0
0.584720861900098	0.6101860920666013	0.6258570029382958	159.0
0.41825095057034223	0.4752851711026616	0.5247148288973384	107.0
0.2857142857142857	0.5714285714285714	0.2857142857142857	27.0
0.41509433962264153	0.5471698113207547	0.5283018867924528	85.0
0.7790055248618785	0.7578268876611418	0.7771639042357275	241.0
0.6238003838771593	0.6756238003838771	0.746641074856046	130.0
1.0	1.0	1.0	11.0
0.8221709006928406	0.9191685912240185	0.7344110854503464	114.0
1.1153846153846154	1.0384615384615385	1.0769230769230769	68.0
0.0	0.0	0.0	22.0
0.6148409893992933	0.7455830388692579	0.8551236749116607	130.0
0.40092879256965946	0.6934984520123839	0.4040247678018576	117.0
0.9607843137254902	0.9607843137254902	0.954248366013072	131.0
0.5	0.8333333333333334	0.5	31.0
1.0	1.0	1.0	14.0
0.2789473684210526	0.3736842105263158	0.21578947368421053	85.0
0.585499316005472	0.6641586867305062	0.48084815321477425	212.0
0.7583333333333333	0.8358333333333333	0.8033333333333333	230.0


==> ncrDA_generated_2021-08-06_17-27-03.tex <==
bfs/rand	fd/rand	vtcs
0.5850622406639004	0.5062240663900415	102.0
0.6378299120234604	0.48240469208211145	145.0
0.75177304964539	0.6595744680851063	87.0
1.0	1.0	18.0
0.6609271523178808	0.5172185430463576	161.0
0.9212746016869728	0.7047797563261481	171.0
0.6333656644034917	0.5965082444228904	152.0
0.6551724137931034	0.5689655172413793	51.0
0.7313432835820896	0.6119402985074627	39.0
0.6466019417475728	0.5106796116504855	123.0
1.0333333333333334	0.7	37.0
0.6195652173913043	0.3804347826086957	97.0
0.7357142857142858	0.5857142857142857	118.0
0.45	0.35	47.0
0.7955414012738854	0.6197452229299363	170.0
0.7396313364055299	0.6705069124423964	103.0
0.4742268041237113	0.7938144329896907	76.0
1.0	1.0	14.0
0.7692307692307693	0.6369770580296896	157.0
0.5555555555555556	0.3888888888888889	68.0
0.7611777535441657	0.7186477644492911	125.0
0.5910714285714286	0.43392857142857144	139.0
1.1153846153846154	1.0769230769230769	47.0
0.5555555555555556	0.5185185185185185	30.0
0.547945205479452	0.4931506849315068	56.0
0.8458559256390396	0.7087529047250194	151.0
0.5533333333333333	0.44	153.0
0.7232142857142857	0.48214285714285715	78.0
0.8196443691786621	0.56731583403895	156.0
0.69108049311095	0.6490210297316896	170.0
1.0	1.0	6.0
0.6739130434782609	0.5122282608695652	159.0
0.7047790339157246	0.5513874614594039	228.0
1.0	1.0	14.0
0.7565345080763582	0.5744493392070484	195.0
1.0	1.0	7.0
0.7072310405643739	0.6137566137566137	131.0
0.7800829875518672	0.5518672199170125	90.0
0.6	0.4	41.0
0.6562942008486563	0.5332390381895332	139.0
0.6813725490196079	0.9313725490196079	65.0
0.7472527472527473	0.5353218210361067	140.0
0.8351351351351352	0.6594594594594595	116.0
1.0	1.0	21.0
0.6531914893617021	0.6345744680851064	152.0
0.7058823529411765	0.5058823529411764	52.0
0.659047619047619	0.43238095238095237	131.0
0.2571428571428571	0.5142857142857142	22.0
0.7105263157894737	0.6146616541353384	118.0
0.6995967741935484	0.4959677419354839	127.0
0.7174887892376681	0.4910313901345291	113.0
0.7728343365611097	0.600366396231353	204.0
0.7841726618705036	0.6187050359712231	63.0
0.679160419790105	0.4947526236881559	143.0
0.8063120386866888	0.6026978875031814	236.0
0.6521739130434783	0.6521739130434783	41.0
0.9084041548630784	0.8054768649669499	159.0
0.6467661691542289	0.4527363184079602	103.0
0.7774827403080191	0.5825809877854488	242.0
0.5969498910675382	0.5010893246187363	123.0
1.0	1.0	18.0
0.6256544502617801	0.6649214659685864	86.0
0.6396574440052701	0.6455862977602108	176.0
1.0	1.4666666666666666	28.0
0.5531062124248497	0.43286573146292584	133.0
0.7800925925925926	0.5601851851851852	158.0
0.7121346324180691	0.6014171833480957	157.0
1.0	1.0	6.0
0.8464912280701754	0.6885964912280702	84.0
0.694560669456067	0.5983263598326359	83.0
1.1240875912408759	0.6131386861313869	30.0
1.0	1.0	22.0
0.8222222222222222	0.6644444444444444	94.0
0.6767676767676768	0.4797979797979798	90.0
0.8419117647058824	0.7573529411764706	117.0
0.5092592592592593	0.5092592592592593	90.0
0.7454545454545455	0.5272727272727272	131.0
0.6767241379310345	0.7306034482758621	114.0
0.9866666666666667	0.92	42.0
0.6283783783783784	0.5472972972972973	85.0
0.5833333333333334	0.4166666666666667	24.0
1.0428265524625269	0.7387580299785867	90.0
0.4663677130044843	0.47085201793721976	93.0
0.7272727272727273	0.4772727272727273	195.0
0.6248715313463515	0.6094552929085303	121.0
0.7613390928725702	0.5151187904967602	150.0
1.25	0.96875	38.0
0.8327702702702703	0.7117117117117117	122.0
0.6905637254901961	0.5839460784313726	165.0
0.8605263157894737	0.7157894736842105	121.0
1.0	1.0	4.0
0.7637362637362637	0.5618131868131868	239.0
0.64375	0.4479166666666667	128.0
0.6929046563192904	0.623059866962306	140.0
1.0	1.0	16.0
0.7692307692307693	0.5269230769230769	81.0
1.0	0.8235294117647058	50.0
0.6933333333333334	0.6666666666666666	53.0
0.8137730358874878	0.565470417070805	167.0
0.715261958997722	0.5125284738041003	129.0
1.0	1.0	6.0
1.0	1.0	18.0
0.4109090909090909	0.52	88.0
0.8300359712230215	0.5881294964028777	145.0
0.8888888888888888	0.8333333333333334	43.0
0.925	0.7014705882352941	129.0
0.7693661971830986	0.6214788732394366	119.0
0.7434725848563969	0.6266318537859008	164.0
0.5487571701720841	0.5659655831739961	104.0
0.25	0.5	37.0
0.5486111111111112	0.5115740740740741	127.0
0.8174762143214822	0.6464697045568353	320.0
0.8073351903435468	0.6527390900649953	186.0
0.6342710997442456	0.5063938618925832	130.0
0.7225725094577553	0.5435056746532156	148.0
1.0	1.0	8.0
0.5625	0.53125	33.0
0.8217770929635336	0.6913199794555727	162.0
0.7674418604651163	0.7093023255813954	37.0
0.896774193548387	0.6774193548387096	146.0
0.0	0.0	38.0
0.373134328358209	0.40298507462686567	61.0
0.6573816155988857	0.5863509749303621	133.0
0.29411764705882354	0.6470588235294118	51.0
1.0	1.0	10.0
0.648854961832061	0.48091603053435117	76.0
1.0086206896551724	1.1637931034482758	46.0
0.7610062893081762	0.7295597484276729	91.0
0.7433862433862434	0.623015873015873	120.0
0.7531172069825436	0.5635910224438903	79.0
0.6802529866479269	0.5614898102600141	158.0
0.8100407055630936	0.4898236092265943	150.0
0.6108022239872914	0.5011914217633042	202.0
0.0	0.6666666666666666	19.0
0.5308641975308642	0.691358024691358	50.0
0.6601941747572816	0.5946601941747572	108.0
0.7656789941916036	0.5320932284390854	357.0
0.7329376854599406	0.6765578635014837	78.0
0.37142857142857144	0.5428571428571428	59.0
0.5130434782608696	0.39420289855072466	122.0
1.0	1.0	25.0
0.6	0.6	49.0
0.7298611111111111	0.5125	141.0
0.7487266553480475	0.6587436332767402	124.0
0.2903225806451613	0.8387096774193549	58.0
0.6216216216216216	0.4864864864864865	30.0
0.5555555555555556	0.7777777777777778	62.0
1.0	1.0	13.0
0.8687459389213775	0.7400909681611436	120.0
0.5238095238095238	0.5714285714285714	36.0
0.674504041146216	0.5789860396767083	169.0
0.6567505720823799	0.551487414187643	159.0
0.663768115942029	0.5623188405797102	172.0
0.49264705882352944	0.5294117647058824	61.0
0.7044198895027625	0.5386740331491713	105.0
1.0	1.0	5.0
0.5086206896551724	0.1810344827586207	66.0
0.7898550724637681	0.7318840579710145	51.0
0.5724137931034483	0.5344827586206896	112.0
0.8078055964653903	0.6811487481590575	171.0
0.5959595959595959	0.5757575757575758	65.0
1.0	1.0	9.0
0.7727272727272727	0.45454545454545453	60.0
0.8943212875797145	0.6052232007288187	240.0
0.8253404381290704	0.6731793960923623	151.0
0.683111954459203	0.5313092979127134	125.0
0.913477537437604	0.8502495840266223	144.0
0.5	0.75	21.0
0.8592730661696178	0.8000931966449207	140.0
0.9799635701275046	0.6520947176684881	108.0
0.6658878504672897	0.5467289719626168	154.0
0.73	0.61	85.0
0.8010204081632653	0.7193877551020408	80.0
0.6839677047289504	0.6851211072664359	142.0
1.0	1.0	7.0
0.615686274509804	0.503921568627451	191.0
0.9166666666666666	0.7083333333333334	29.0
0.7671118530884808	0.6101836393989983	168.0
0.78	0.4	56.0
1.0	1.0	20.0
1.0	1.0	12.0
0.7598425196850394	0.5708661417322834	90.0
0.7322097378277154	0.6161048689138576	129.0
0.6458684654300169	0.554806070826307	126.0
0.8988877654196158	0.6056622851365016	151.0
0.7575757575757576	0.8181818181818182	40.0
0.711340206185567	0.47079037800687284	98.0
0.59375	0.8125	47.0
0.6	0.6285714285714286	60.0
0.6764705882352942	0.5084033613445378	118.0
0.6562408652440807	0.5624086524408067	226.0
0.3076923076923077	0.23076923076923078	34.0
0.8114446529080676	0.6885553470919324	136.0
0.6783625730994152	0.783625730994152	86.0
1.0	1.0	20.0
0.6486486486486487	0.3783783783783784	31.0
1.0	1.0	20.0
1.0	1.0	20.0
0.9282700421940928	0.7616033755274262	150.0
1.0	0.0	22.0
0.5521064301552107	0.4811529933481153	113.0
0.3333333333333333	0.0	36.0
0.735632183908046	0.7471264367816092	56.0
0.843978102189781	0.6982968369829684	210.0
1.0	1.0	5.0
0.5350877192982456	0.4298245614035088	89.0
0.9444444444444444	0.6481481481481481	24.0
0.8571428571428571	0.6785714285714286	26.0
0.7276051188299817	0.4753199268738574	137.0
0.575	0.6	50.0
1.007905138339921	0.7984189723320159	74.0
1.0	1.0	9.0
1.0	1.0	6.0
0.6200980392156863	0.5318627450980392	139.0
0.7871188372755771	0.5961812482188658	249.0
0.9092307692307692	0.7092307692307692	153.0
1.0	1.0	13.0
0.8260038240917782	0.5831739961759083	128.0
0.8477751756440282	0.7845433255269321	96.0
0.6396396396396397	0.6126126126126126	68.0
0.723404255319149	0.425531914893617	45.0
1.0	1.0	17.0
0.8106995884773662	0.6604938271604939	168.0
0.6279761904761905	0.5446428571428571	118.0
0.5454545454545454	0.6859504132231405	59.0
0.5045045045045045	0.5945945945945946	56.0
0.48412698412698413	0.36507936507936506	119.0
1.0	1.0	12.0
0.5141509433962265	0.47877358490566035	98.0
1.0	1.0	20.0
0.5789473684210527	0.7368421052631579	67.0
0.6666666666666666	0.6923076923076923	48.0
0.7525773195876289	0.5257731958762887	64.0
3.0	2.0	17.0
0.6641414141414141	0.5606060606060606	105.0
0.6614583333333334	0.50390625	220.0
0.6098191214470284	0.46382428940568476	128.0
0.6621004566210046	0.660958904109589	114.0
0.6463414634146342	0.5416666666666666	169.0
1.0	1.0	16.0
0.7077244258872651	0.5323590814196242	147.0
0.9737335834896811	0.6848030018761726	140.0
0.8316906747536013	0.5928733889310084	177.0
0.5846645367412141	0.731629392971246	87.0
0.7241259651253579	0.5582545328359504	356.0
0.6363636363636364	0.7878787878787878	22.0
0.852717708942139	0.706019871420222	129.0
0.907608695652174	0.6141304347826086	97.0
0.7590741714886902	0.6549184639663335	163.0
1.0	1.0	14.0
0.5692307692307692	0.36923076923076925	81.0
0.6211009174311927	0.37155963302752293	189.0
0.6801152737752162	0.6570605187319885	102.0
0.5747126436781609	0.42528735632183906	86.0
1.0	1.0	11.0
0.8194706994328923	0.5378071833648393	190.0
0.6792792792792792	0.563963963963964	192.0
0.7769652650822669	0.5648994515539305	122.0
0.8209366391184573	0.6115702479338843	96.0
0.6792452830188679	0.5660377358490566	78.0
1.0	0.5952380952380952	51.0
0.8404634581105169	0.624777183600713	164.0
0.5517241379310345	0.41379310344827586	47.0
0.6142857142857143	0.5	112.0
1.0952380952380953	0.746031746031746	41.0
0.6978818283166109	0.46265328874024525	145.0
0.9858075503831961	0.7550383196139654	244.0
0.8354430379746836	1.0759493670886076	41.0
0.6197183098591549	0.5176056338028169	128.0
0.7424496644295302	0.5226510067114094	205.0
0.7650501672240803	0.5794314381270903	162.0
0.7720436449424949	0.5617811854910056	252.0
0.0	0.0	31.0
0.6795827123695977	0.6348733233979136	112.0
0.6886688668866887	0.5902090209020903	213.0
0.703951367781155	0.5750759878419452	154.0
0.4117647058823529	0.5588235294117647	34.0
0.5	0.375	28.0
0.5339366515837104	0.5542986425339367	101.0
0.6797124600638977	0.4768370607028754	200.0
0.5637393767705382	0.4936260623229462	203.0
0.0	0.0	39.0
0.9707736389684813	0.7415472779369627	128.0
0.576271186440678	0.576271186440678	76.0
0.4537037037037037	0.37037037037037035	81.0
0.7773972602739726	0.8253424657534246	113.0
0.8280123583934088	0.7312049433573635	124.0
0.6333938294010889	0.7096188747731398	78.0
1.0	1.0	15.0
0.7724982001439885	0.599712023038157	169.0
0.6568345323741007	0.6294964028776978	129.0
0.7024096385542169	0.5313253012048192	135.0
0.7745358090185677	0.5915119363395226	90.0
0.7459789240155297	0.7282307265668331	162.0
1.2903225806451613	0.7741935483870968	34.0
1.0	1.0	18.0
0.8333333333333334	1.3333333333333333	23.0
1.0	1.0	5.0
0.8008130081300813	0.6788617886178862	96.0
0.7332474226804123	0.6095360824742269	142.0
0.6875	0.5625	138.0
2.0	1.0	31.0
1.0	1.0	13.0
0.9541616405307599	0.6984318455971049	139.0
0.0	0.0	36.0
0.583969465648855	0.4580152671755725	122.0
0.6541353383458647	0.9624060150375939	60.0
0.8532796317606444	0.622554660529344	244.0
0.7856173677069199	0.6146540027137042	142.0
0.8285561210822395	0.6348781141173319	206.0
0.0	0.0	15.0
0.9361948955916474	0.6032482598607889	190.0
0.9645776566757494	0.7029972752043597	108.0
0.6961722488038278	0.6052631578947368	106.0
0.8025387870239774	0.6346967559943583	138.0
0.581151832460733	0.6858638743455497	62.0
0.24242424242424243	0.45454545454545453	94.0
0.6144278606965174	0.5920398009950248	88.0
0.8269794721407625	0.6490713587487781	154.0
0.6666666666666666	0.6666666666666666	14.0
0.7250257466529351	0.6189495365602472	186.0
0.8784965034965035	0.5743006993006993	193.0
0.21428571428571427	0.5714285714285714	58.0
0.9857142857142858	0.6142857142857143	65.0
0.6838638858397366	0.6114160263446762	169.0
0.7014333638304361	0.5773101555352241	203.0
0.7214514407684098	0.6029882604055496	165.0
0.7349397590361446	0.4819277108433735	96.0
0.4444444444444444	0.5555555555555556	47.0
0.4067796610169492	0.423728813559322	80.0
0.6917040358744395	0.5672645739910314	136.0
0.7523105360443623	0.4048059149722736	119.0
0.7882599580712788	0.5513626834381551	97.0
0.6977099236641221	0.601526717557252	132.0
0.6	0.4666666666666667	24.0
0.898300283286119	0.6801699716713882	248.0
1.0	1.0	11.0
0.7398058252427184	0.5883495145631068	97.0
0.7680391357521402	0.521810028536486	227.0
0.6756756756756757	0.8378378378378378	36.0
0.6904761904761905	0.4523809523809524	23.0
0.8220973782771536	0.7106741573033708	161.0
0.8957399103139013	0.7399103139013453	137.0
0.7202881152460985	0.575030012004802	144.0
0.7694753577106518	0.5520667726550079	217.0
0.6629213483146067	0.6179775280898876	36.0
0.6548042704626335	0.4555160142348754	89.0
0.7441176470588236	0.5661764705882353	176.0
0.9464285714285714	0.9821428571428571	47.0
1.0	1.0	5.0
0.7560209424083769	0.406282722513089	191.0
0.839253461770018	0.8199879590608068	121.0
0.7014925373134329	0.6119402985074627	59.0
1.0	1.0	13.0
0.7936117936117936	0.6511056511056511	89.0
0.6858006042296072	0.6435045317220544	117.0
0.4523809523809524	0.23809523809523808	57.0
0.6648451730418944	0.5282331511839709	86.0
1.0	1.0	19.0
0.7638786084381939	0.5780903034789046	173.0
0.7384751773049646	0.5806737588652482	113.0
0.8269794721407625	0.7565982404692082	87.0
0.6220994475138122	0.5458563535911602	143.0
0.7074235807860262	0.3624454148471616	179.0
0.6697341513292433	0.5081799591002045	195.0
0.7266462480857581	0.5436447166921899	215.0
0.6842837273991655	0.6244784422809457	110.0
0.7711496746203904	0.6561822125813449	151.0
0.7429718875502008	0.5244979919678715	157.0
0.6290726817042607	0.5488721804511278	134.0
0.7183406113537117	0.4606986899563319	172.0
0.72	0.5911111111111111	108.0
2.0	1.3333333333333333	18.0
0.639344262295082	0.6065573770491803	53.0
0.4448669201520912	0.5209125475285171	116.0
0.8562834224598931	0.7346256684491979	118.0
0.6623931623931624	0.48717948717948717	103.0
0.8757987220447284	0.6010383386581469	220.0
0.7896440129449838	0.6828478964401294	112.0
0.7877551020408163	0.6489795918367347	93.0
0.7556818181818182	0.6041666666666666	93.0
0.8702830188679245	0.5542452830188679	126.0
1.0	1.0	22.0
0.7587006960556845	0.4756380510440835	177.0
0.8364057971014492	0.5797101449275363	320.0
0.0	0.0	32.0
0.850725828540126	0.6485894275540948	237.0
0.9375	0.75	47.0
0.6590346534653465	0.5785891089108911	190.0
0.24390243902439024	0.45121951219512196	84.0
1.0	0.75	34.0
2.0	0.0	43.0
0.7068965517241379	0.41379310344827586	63.0
0.7255216693418941	0.5585874799357945	123.0
0.5962566844919787	0.47058823529411764	133.0
0.762962962962963	0.5722222222222222	143.0
0.47044917257683216	0.3475177304964539	141.0
0.8260542168674698	0.6920180722891566	164.0
0.5	0.5	24.0
0.7767653758542141	0.6059225512528473	105.0
0.39622641509433965	0.6415094339622641	57.0
0.5739130434782609	0.6843478260869565	136.0
1.0	1.0	13.0
1.0335570469798658	0.959731543624161	40.0
0.8427128427128427	0.5743145743145743	169.0
0.7749576988155669	0.5922165820642978	100.0
0.7370977534911961	0.647237401335762	204.0
1.0	1.0	8.0
0.6318181818181818	0.5636363636363636	89.0
0.724950884086444	0.48330058939096265	133.0
0.7336548767416935	0.5814576634512326	239.0
1.0	1.0	34.0
0.7829457364341085	0.6682170542635659	127.0
0.8518518518518519	0.6243386243386243	123.0
0.7152103559870551	0.6089536138079827	150.0
0.7747252747252747	0.6978021978021978	71.0
0.6533333333333333	0.4533333333333333	73.0
0.7272727272727273	0.5526315789473685	160.0
0.718005540166205	0.4858725761772853	198.0
0.52	0.52	28.0
0.4561933534743202	0.3564954682779456	104.0
1.0	1.0	15.0
0.6746411483253588	0.583732057416268	94.0
0.6213592233009708	0.487378640776699	151.0
0.3953488372093023	0.5581395348837209	46.0
0.715629522431259	0.4934876989869754	199.0
1.0	1.0	9.0
1.0	1.0	19.0
0.8292682926829268	0.926829268292683	30.0
0.6246031746031746	0.46190476190476193	163.0
0.8	0.5690721649484536	118.0
1.0	1.0	7.0
0.8303448275862069	0.5413793103448276	115.0
0.7920529801324503	0.680794701986755	158.0
0.8103448275862069	0.9741379310344828	48.0
0.7298716452742123	0.5606767794632439	176.0
0.62426614481409	0.5909980430528375	128.0
0.48484848484848486	0.6666666666666666	58.0
0.5714285714285714	0.4155844155844156	49.0
0.7990033222591362	0.5660299003322259	191.0
1.0	1.0	4.0
0.84375	0.5	49.0
0.5588235294117647	0.6078431372549019	48.0
0.609375	0.47596153846153844	134.0
0.19230769230769232	0.25	66.0
0.7407407407407407	0.6666666666666666	64.0
0.6932551319648094	0.5527859237536656	245.0
1.0	1.0	12.0
0.3333333333333333	0.3333333333333333	38.0
0.6091954022988506	0.5057471264367817	127.0
0.7794117647058824	0.6470588235294118	84.0
1.0	1.0	11.0
0.43	0.5	70.0
0.7391304347826086	0.5217391304347826	74.0
0.7565095003518649	0.6213933849401829	133.0
0.6442516268980477	0.648590021691974	122.0
0.93037088873338	0.6469559132260322	239.0
1.0	1.0	9.0
0.9227963525835866	0.6139817629179332	166.0
1.0	1.0	21.0
0.7213930348258707	0.5437100213219617	171.0
0.8095238095238095	0.7083333333333334	64.0
0.7882197220383852	0.6551952349437459	130.0
0.8903559127439724	0.6452353616532721	229.0
0.7640449438202247	0.7640449438202247	66.0
0.4782608695652174	0.5652173913043478	53.0
1.0	1.0	43.0
0.8241758241758241	0.7120879120879121	75.0
0.9383116883116883	0.7175324675324676	115.0
0.655819774718398	0.5832290362953693	216.0
0.6086956521739131	0.5434782608695652	52.0
0.8061224489795918	0.673469387755102	90.0
1.0	1.0	10.0
0.715203426124197	0.5840471092077087	221.0
0.6745098039215687	0.4980392156862745	88.0
0.9459459459459459	1.027027027027027	36.0
0.7811634349030471	0.7202216066481995	110.0
0.7851622874806801	0.5873261205564142	121.0
0.617816091954023	0.5833333333333334	96.0
0.7509845501363224	0.6179945471069372	247.0
0.42105263157894735	0.34210526315789475	94.0
0.610655737704918	0.4036885245901639	91.0
1.0	1.0	36.0
0.7142857142857143	1.4285714285714286	39.0
0.826936026936027	0.6478114478114478	161.0
0.7519325368938862	0.6289529163738581	161.0
0.7991967871485943	0.43775100401606426	108.0
0.6751730103806228	0.5242214532871973	233.0
1.0	1.0	6.0
0.6931818181818182	0.5580808080808081	155.0
0.6382113821138211	0.5894308943089431	103.0
1.0	1.0	19.0
0.7534883720930232	0.6930232558139535	68.0
0.7813211845102506	0.6355353075170843	109.0
0.8256880733944955	0.5688073394495413	41.0
0.7190934065934066	0.6016483516483516	168.0
0.7753623188405797	0.5271739130434783	127.0
0.4326923076923077	0.4326923076923077	96.0
0.5275590551181102	0.3228346456692913	84.0
0.676056338028169	0.6901408450704225	34.0
0.8507601613403661	0.6621160409556314	203.0
0.7752808988764045	0.42696629213483145	54.0
0.7353970390309555	0.6541049798115747	203.0
0.8901098901098901	0.6813186813186813	67.0
0.581081081081081	0.3783783783783784	92.0
0.9390862944162437	0.5253807106598984	103.0
0.7663551401869159	0.5362149532710281	140.0
0.7726218097447796	0.5939675174013921	117.0
0.8706896551724138	0.6695402298850575	156.0
0.7355072463768116	0.6246376811594203	167.0
0.8064516129032258	0.41935483870967744	84.0
0.694720334553058	0.5023523261892315	169.0
1.1147540983606556	0.8852459016393442	64.0
0.6227272727272727	0.5575757575757576	150.0
0.8204878048780487	0.6380487804878049	129.0
0.797886393659181	0.5733157199471598	155.0
1.0	1.0	14.0
0.6126760563380281	0.6549295774647887	59.0
0.7309417040358744	0.5480817140009965	179.0
0.6791120080726539	0.5216952573158425	149.0
0.750392464678179	0.5447409733124019	132.0
0.7516714422158548	0.5348615090735435	152.0
0.7791044776119403	0.5892537313432836	236.0
0.8474959612277867	0.5722132471728595	247.0
1.28	0.72	39.0
0.8333333333333334	0.9814814814814815	52.0
0.8846153846153846	0.8461538461538461	36.0
0.7663817663817664	0.6210826210826211	119.0
0.8567839195979899	0.6306532663316583	103.0
0.7037037037037037	0.6203703703703703	145.0
0.5909816440542698	0.4736632083000798	230.0
0.823020625415835	0.6640053226879574	244.0
0.7076051015588096	0.6329711856400567	221.0
0.6468172484599589	0.5236139630390144	113.0
0.6166666666666667	0.5333333333333333	49.0
0.8186813186813187	0.5262515262515263	167.0
0.8080808080808081	0.5808080808080808	87.0
0.0	0.0	35.0
0.7688888888888888	0.5155555555555555	116.0
0.7493333333333333	0.616	135.0
1.75	1.25	29.0
0.7461406518010292	0.4751286449399657	147.0
0.8567164179104477	0.7074626865671642	140.0
1.0	1.0	6.0
0.6968325791855203	0.5294117647058824	101.0
1.2580645161290323	0.8709677419354839	67.0
0.7348659003831418	0.6490421455938697	142.0
0.745719489981785	0.5985428051001821	208.0
0.6063829787234043	0.3670212765957447	73.0
0.6563307493540051	0.4005167958656331	104.0
0.935064935064935	0.827922077922078	127.0
0.9573170731707317	0.9390243902439024	57.0
0.6240875912408759	0.45742092457420924	165.0
0.7509986684420772	0.4007989347536618	142.0
0.519650655021834	0.42358078602620086	84.0
0.7807407407407407	0.4696296296296296	139.0
0.4520884520884521	0.4176904176904177	124.0
0.7215777262180975	0.5081206496519721	95.0
1.0	1.0	7.0
0.6262886597938144	0.5438144329896907	119.0
0.8179551122194514	0.5586034912718204	101.0
0.8243398392652124	0.7359357060849598	113.0
0.8148148148148148	0.7407407407407407	20.0
0.8328530259365994	0.5734870317002881	126.0
0.8495370370370371	0.6857638888888888	167.0
0.7014694508894045	0.5328692962103635	162.0
0.7307692307692307	0.8076923076923077	45.0
0.6635784597568037	0.5347423277359583	240.0
0.8716904276985743	0.670061099796334	113.0
0.658051689860835	0.5228628230616302	122.0
0.7566820276497696	0.6986175115207374	150.0
0.75	0.75	34.0
0.7781954887218046	0.5488721804511278	91.0
0.8165337200870196	0.5971718636693256	199.0
0.857487922705314	0.5217391304347826	114.0
0.0	0.0	34.0
0.7	0.5	29.0
0.49019607843137253	0.39215686274509803	69.0
0.9943181818181818	0.8636363636363636	68.0
0.4166666666666667	0.875	30.0
0.4375	0.6875	57.0
0.6642156862745098	0.5833333333333334	142.0
0.6666666666666666	0.6666666666666666	25.0
0.6829268292682927	0.4634146341463415	48.0
0.6531942633637549	0.5958279009126467	166.0
0.7155318633389871	0.6588320814150714	245.0
0.7368421052631579	0.5910267471958585	220.0
1.0	1.0	22.0
0.8635437881873728	0.7535641547861507	111.0
0.5416666666666666	0.8541666666666666	39.0
0.7227241139680334	0.5434329395413482	182.0
0.5284210526315789	0.42526315789473684	105.0
0.8245125348189415	0.43454038997214484	132.0
0.4375	0.5	73.0
0.6319612590799032	0.5108958837772397	109.0
0.7465802735781137	0.5946724262059035	134.0
0.772169167803547	0.6002728512960437	145.0
0.6326530612244898	0.45102040816326533	131.0
0.8138345864661655	0.6748872180451128	233.0
0.7669376693766937	0.7009936766034327	165.0
0.6373276776246023	0.4814422057264051	127.0
1.0	1.0	17.0
0.6394618834080718	0.5623318385650224	120.0
0.6001757469244289	0.44991212653778556	166.0
0.16666666666666666	0.0	33.0
1.1	1.1	25.0
0.6845360824742268	0.5298969072164949	107.0
1.0	1.0	6.0
0.6989463120923232	0.6332162568991471	176.0
0.7019164955509924	0.5783709787816564	230.0
0.918744971842317	0.6339501206757844	190.0
0.7614942528735632	0.4109195402298851	111.0
0.6721311475409836	0.8524590163934426	96.0
0.8284574468085106	0.6569148936170213	142.0
0.8177153659195248	0.6078854982446665	231.0
0.5	0.5	32.0
0.783256880733945	0.6077981651376146	126.0
0.7658862876254181	0.5852842809364549	130.0
0.6428571428571429	0.9285714285714286	22.0
0.7352264006139677	0.6377590176515733	180.0
0.7354085603112841	0.5549610894941635	134.0
0.643598615916955	0.5051903114186851	143.0
0.616822429906542	0.7289719626168224	53.0
0.8399646330680813	0.6604774535809018	160.0
0.6900826446280992	0.47520661157024796	110.0
0.8097014925373134	0.601679104477612	135.0
0.6741028128031038	0.5902036857419981	150.0
0.7378318584070797	0.6603982300884956	117.0
0.3	0.3142857142857143	64.0
0.7958236658932715	0.679814385150812	92.0
0.7431466030989273	0.6793802145411204	132.0
0.6323529411764706	0.7132352941176471	49.0
0.7381546134663342	0.5195344970906068	187.0
0.8888888888888888	1.0	33.0
0.6015503875968993	0.5387596899224806	174.0
0.7027027027027027	0.5664864864864865	157.0
0.41935483870967744	0.25806451612903225	63.0
1.0	1.0	20.0
1.0	1.0	7.0
0.5168539325842697	0.5280898876404494	42.0
0.6658767772511849	0.5955766192733017	130.0
1.0245022970903521	0.6263399693721287	174.0
0.6203259827420902	0.5819750719079578	165.0
0.7170731707317073	0.7707317073170732	82.0
0.7142857142857143	1.0	40.0
0.5925925925925926	0.5555555555555556	63.0
0.36666666666666664	0.5333333333333333	58.0
0.7458823529411764	0.6329411764705882	122.0
0.9443359375	0.7496744791666666	229.0
0.6655405405405406	0.5	105.0
1.0	1.0	48.0
0.6814159292035398	0.4889380530973451	141.0
0.7216494845360825	0.6891356066613799	162.0
0.7401247401247402	0.5696465696465697	100.0
0.7724957555178268	0.562200956937799	352.0
0.9013568023469014	0.6787678767876788	241.0
0.7440423654015887	0.6045895851721095	154.0
0.5975889781859931	0.4827784156142365	155.0
0.7727272727272727	0.731404958677686	90.0
0.3333333333333333	0.3333333333333333	19.0
0.6457765667574932	0.6076294277929155	78.0
0.8110195674562307	0.6163748712667353	170.0
0.9513274336283186	0.8053097345132744	22.0
0.6122448979591837	0.4336734693877551	74.0
0.6969099276791585	0.5851413543721236	172.0
0.8314606741573034	0.6539325842696629	108.0
0.2857142857142857	0.25396825396825395	75.0
0.25	0.375	35.0
0.7425343018563357	0.5980629539951574	156.0
1.0	1.0	26.0
0.5517241379310345	0.7413793103448276	69.0
0.7891223733003708	0.630407911001236	250.0
0.8402457757296466	0.5852534562211982	202.0
0.7767495662232504	0.600347021399653	161.0
0.6106194690265486	0.588495575221239	71.0
0.8975979772439949	0.6005056890012642	191.0
0.7694117647058824	0.7176470588235294	79.0
0.5494505494505495	0.5824175824175825	50.0
1.279926335174954	0.9226519337016574	111.0
0.805414551607445	0.5812182741116751	177.0
0.7232824427480916	0.6125954198473282	122.0
0.6855123674911661	0.6148409893992933	101.0
0.6790123456790124	0.588477366255144	86.0
0.9173913043478261	0.5739130434782609	87.0
0.6713286713286714	0.5244755244755245	81.0
0.8368794326241135	0.599290780141844	90.0
0.5080906148867314	0.44336569579288027	97.0
0.8490926456542502	0.606494746895893	188.0
0.6956521739130435	0.9254658385093167	89.0
0.16666666666666666	0.3333333333333333	22.0
0.7018181818181818	0.7272727272727273	82.0
0.7672253258845437	0.638733705772812	116.0
0.7785714285714286	0.5057142857142857	134.0
0.7698412698412699	0.6613756613756614	111.0
0.5952380952380952	0.5714285714285714	26.0
0.8256410256410256	0.9025641025641026	98.0
0.5464788732394367	0.4507042253521127	99.0
1.0	1.0	30.0
0.5777777777777777	0.362962962962963	71.0
0.9203187250996016	0.8685258964143426	97.0
0.6767676767676768	0.6296296296296297	105.0
0.8776041666666666	0.6770833333333334	108.0
1.0	1.0	16.0
0.8235294117647058	0.5424836601307189	109.0
0.6736842105263158	0.8105263157894737	52.0
0.7698783910196445	0.5594013096351731	140.0
0.6765523632993512	0.5013901760889713	187.0
1.0	1.0	30.0
0.39603960396039606	0.48514851485148514	51.0
0.7698170731707317	0.6402439024390244	115.0
0.7854785478547854	0.8877887788778878	97.0
0.9887640449438202	0.6320224719101124	85.0
0.85969868173258	0.5546139359698682	168.0
0.7823741007194245	0.6402877697841727	149.0
0.8038897893030794	0.6677471636952999	164.0
0.6	1.12	53.0
0.9006535947712418	0.6660130718954248	124.0
0.6878172588832487	0.4352791878172589	157.0
0.5370370370370371	0.46296296296296297	42.0
0.8979591836734694	0.6268221574344023	97.0
0.5802469135802469	0.5925925925925926	41.0
1.0	1.0	25.0
0.7618198037466548	0.5370205173951829	149.0
0.6686746987951807	0.7329317269076305	84.0
0.7304347826086957	0.5565217391304348	94.0
0.8558558558558559	0.6666666666666666	46.0
0.7740112994350282	0.544256120527307	121.0
0.5117924528301887	0.5471698113207547	142.0
0.4	0.36666666666666664	76.0
0.7158764367816092	0.59375	219.0
1.1386138613861385	0.7524752475247525	121.0
0.8454545454545455	0.7636363636363637	57.0
0.9089820359281438	0.6119760479041916	127.0
0.7867950481430537	0.6121045392022009	146.0
1.0	1.0	28.0
0.6877470355731226	0.5691699604743083	107.0
0.7001897533206831	0.5692599620493358	118.0
0.9325842696629213	0.6966292134831461	117.0
0.7086614173228346	0.6417322834645669	82.0
0.8333333333333334	0.7916666666666666	50.0
0.6444444444444445	0.597979797979798	124.0
0.8354814253222138	0.7035633055344959	147.0
0.6884389288047028	0.6329196603527106	213.0
0.549645390070922	0.5070921985815603	130.0
0.9574468085106383	0.851063829787234	24.0
0.8765603328710125	0.6601941747572816	186.0
0.585081585081585	0.45454545454545453	121.0
0.7763558805606338	0.6489945155393053	123.0
0.6349206349206349	0.4585537918871252	112.0
0.6581740976645435	0.45222929936305734	115.0
0.8688876947877485	0.5722729715206878	183.0
0.7833001988071571	0.6560636182902585	94.0
0.8072916666666666	0.84375	129.0
1.0	1.0	10.0
0.4406779661016949	0.3050847457627119	64.0
0.7272727272727273	0.67003367003367	98.0
0.6677195198989261	0.7561591914087177	119.0
0.6415094339622641	0.6981132075471698	46.0
0.5924050632911393	0.4962025316455696	91.0
0.6167330677290837	0.48366533864541833	156.0
0.5413793103448276	0.43103448275862066	100.0
0.8870449678800857	0.6761241970021413	175.0
0.7029702970297029	0.601980198019802	148.0
0.2727272727272727	0.2727272727272727	36.0
0.7901639344262295	0.7324590163934426	129.0
0.6691729323308271	0.48872180451127817	85.0
0.7736549165120594	0.7031539888682746	160.0
1.0	1.0	34.0
0.7020506634499397	0.5802171290711701	144.0
0.71900826446281	0.6239669421487604	75.0
0.7525206232813932	0.6810265811182401	117.0
0.697841726618705	0.5707434052757794	134.0
0.8620331950207469	0.578838174273859	155.0
0.5	0.0	28.0
1.0	2.0	15.0
0.7235772357723578	0.6314363143631436	98.0
0.5596026490066225	0.5629139072847682	113.0
0.7273603082851637	0.5973025048169557	150.0
0.5556291390728477	0.5456953642384106	205.0
0.617303023615096	0.5076142131979695	247.0
0.7140549273021002	0.620893914916532	186.0
0.35714285714285715	0.38095238095238093	49.0
0.8519793459552496	0.6179001721170396	137.0
0.6867671691792295	0.5360134003350083	129.0
0.7938144329896907	0.5979381443298969	91.0
0.6774861878453039	0.5732044198895028	173.0
0.5730800990916598	0.3897605284888522	201.0
0.6244725738396625	0.5316455696202531	89.0
0.9469469469469469	0.7327327327327328	120.0
0.9166666666666666	1.125	23.0
0.5224274406332454	0.49868073878627966	115.0
0.7402258905299739	0.6012163336229366	183.0
0.36619718309859156	0.4084507042253521	49.0
0.8008130081300813	0.7425474254742548	164.0
0.8557213930348259	0.7014925373134329	93.0
0.7515883100381194	0.6797966963151207	159.0
1.0	1.0	8.0
0.7305555555555555	0.6166666666666667	130.0
0.7832731314253959	0.5568213392609058	233.0
0.7248539909149903	0.5944192083062946	171.0
0.8442028985507246	0.5942028985507246	111.0
0.4166666666666667	0.20833333333333334	39.0
0.7369186046511628	0.7611434108527132	161.0
0.8627450980392157	0.5294117647058824	42.0
0.6074074074074074	0.5185185185185185	129.0
0.863749555318392	0.5955176093916755	220.0
0.823021582733813	0.7079136690647482	121.0
1.0	1.0	8.0
0.40789473684210525	0.15789473684210525	55.0
0.8452502553626149	0.7354443309499489	178.0
0.8660274682560248	0.6398030577869914	232.0
0.7851134335967372	0.5692072393576345	232.0
0.8362369337979094	0.9303135888501742	95.0
1.0	1.0	22.0
0.6921296296296297	0.4930555555555556	132.0
0.8579088471849866	0.7319034852546917	128.0
0.5159574468085106	0.5212765957446809	91.0
0.800982800982801	0.4742014742014742	128.0
0.5498281786941581	0.5360824742268041	112.0
0.7867036011080333	0.5955678670360111	119.0
0.8002232142857143	0.6573660714285714	126.0
0.7330895795246801	0.6663619744058501	158.0
0.8775510204081632	0.7551020408163265	58.0
0.768361581920904	0.6610169491525424	79.0
0.6921212121212121	0.5175757575757576	112.0
0.46938775510204084	0.5510204081632653	68.0
0.7958015267175572	0.6412213740458015	115.0
0.5454545454545454	0.4935064935064935	54.0
0.75	0.5	38.0
0.5763546798029556	0.547783251231527	120.0
0.9690721649484536	1.0309278350515463	35.0
0.6329113924050633	0.6781193490054249	131.0
0.7277397260273972	0.466324200913242	156.0
0.8333333333333334	0.5871212121212122	120.0
0.7207792207792207	0.5714285714285714	67.0
0.7380265435660704	0.5894402769763416	241.0
0.7649572649572649	0.5769230769230769	107.0
0.7727272727272727	0.5490430622009569	115.0
0.7149122807017544	0.5701754385964912	93.0
1.0	1.0	13.0
0.7292418772563177	0.6714801444043321	86.0
0.7405781192828393	0.5188437614343212	182.0
0.7265238879736409	0.5502471169686985	113.0
0.6413934426229508	0.5846994535519126	153.0
1.0	1.0	6.0
0.6099110546378653	0.4701397712833545	188.0
0.648062015503876	0.4930232558139535	135.0
1.010939510939511	0.8082368082368082	116.0
0.5714285714285714	0.3904761904761905	68.0
0.7941888619854721	0.7215496368038741	116.0
0.7300613496932515	0.5116564417177915	165.0
0.5794392523364486	0.4088785046728972	127.0
0.6481481481481481	0.5277777777777778	54.0
1.0	1.0	18.0
0.6272189349112426	0.6173570019723866	125.0
0.7777777777777778	0.6666666666666666	13.0
0.6821782178217822	0.5089108910891089	169.0
0.6229508196721312	0.7540983606557377	37.0
0.8211529732183386	0.5905583295506128	163.0
0.5827814569536424	0.5231788079470199	92.0
0.8404840484048405	0.6677667766776678	126.0
0.6683937823834197	0.5803108808290155	89.0
1.0	1.0	1.0
1.0	1.0	23.0
0.448	0.448	99.0
0.7442922374429224	0.634703196347032	145.0
0.8848600508905853	0.5585241730279898	243.0
0.82861328125	0.6142578125	243.0
0.8944223107569721	0.6593625498007968	126.0
0.8228228228228228	0.6771771771771772	118.0
0.5277777777777778	0.2638888888888889	70.0
0.6996871741397289	0.7017726798748697	113.0
0.7570093457943925	0.6261682242990654	131.0
0.6917960088691796	0.458980044345898	145.0
0.6374269005847953	0.3654970760233918	110.0
0.4482758620689655	0.2413793103448276	61.0
0.7341532639545885	0.6007568590350048	183.0
0.6857142857142857	0.4035714285714286	113.0
0.764433206911083	0.483354403708386	229.0
0.8295307791648731	0.6134309083082221	213.0
1.0	1.0	12.0
0.8402061855670103	0.7216494845360825	88.0
0.8425591098748262	0.6606397774687065	235.0
0.6727272727272727	0.6242424242424243	80.0
0.7467811158798283	0.628755364806867	108.0
0.39864864864864863	0.3310810810810811	77.0
1.0	1.0	5.0
0.9692307692307692	0.7307692307692307	194.0
0.8043785310734464	0.6045197740112994	200.0
0.0	0.0	25.0
0.7121212121212122	0.42424242424242425	63.0
0.49612403100775193	0.5348837209302325	90.0
0.6666666666666666	0.0	14.0
0.9362380446333688	0.7290116896918172	148.0
1.0	1.0	24.0
0.7335766423357665	0.5647810218978102	244.0
1.0	1.0	22.0
0.5585492227979275	0.49326424870466323	112.0
0.5961977186311787	0.4935361216730038	195.0
1.0	1.0	4.0
0.7366482504604052	0.6758747697974218	89.0
1.0	1.0	16.0
0.95	0.95	40.0
0.5857142857142857	0.2714285714285714	86.0
0.6831683168316832	0.33663366336633666	76.0
0.8012958963282938	0.6983441324694024	197.0
0.7288135593220338	0.3898305084745763	40.0
2.0	1.0	2.0
0.6640401146131805	0.4512893982808023	163.0
0.7563025210084033	0.7899159663865546	49.0
0.7995505617977529	0.6258426966292134	240.0
0.6903253985586373	0.5763267088884035	252.0
0.8728615863141524	0.7869362363919129	201.0
0.815406976744186	0.5523255813953488	142.0
0.8641352714328092	0.6828834173835657	243.0
1.0	1.0	8.0
1.1378299120234605	0.8914956011730205	90.0
0.54	0.78	51.0
0.9252971137521222	0.7487266553480475	120.0
0.5186721991701245	0.3029045643153527	99.0
0.7116104868913857	0.5692883895131086	102.0
1.0063091482649842	0.7791798107255521	80.0
0.5629043853342919	0.507548526240115	164.0
0.6839935882757041	0.6258300893061598	241.0
0.7318435754189944	0.6703910614525139	39.0
0.8521536670547147	0.6461001164144354	107.0
0.9446064139941691	0.7332361516034985	120.0
0.5585284280936454	0.4414715719063545	96.0
0.7314487632508834	0.5865724381625441	103.0
0.7694915254237288	0.6474576271186441	92.0
0.7012987012987013	0.5324675324675324	109.0
0.5769230769230769	0.5576923076923077	47.0
0.9768211920529801	0.8278145695364238	106.0
0.3652173913043478	0.5391304347826087	71.0
0.7174515235457064	0.6066481994459834	107.0
0.7821229050279329	0.6187150837988827	140.0
0.6138448707256047	0.5062552126772311	141.0
0.8007380073800738	0.5645756457564576	89.0
0.5444234404536862	0.42344045368620037	120.0
0.8333333333333334	0.5833333333333334	42.0
0.5454545454545454	0.3939393939393939	38.0
0.7203791469194313	0.608214849921011	204.0
0.8060344827586207	0.549712643678161	244.0
1.0	1.0	9.0
0.42105263157894735	0.8947368421052632	43.0
0.920028818443804	0.6455331412103746	143.0
0.7165991902834008	0.757085020242915	62.0
0.38461538461538464	0.5769230769230769	58.0
0.6407185628742516	0.46706586826347307	135.0
1.0	1.0	9.0
1.0	1.0	13.0
0.6435643564356436	0.5742574257425742	138.0
0.6986062717770035	0.578397212543554	148.0
0.7878699941961694	0.5681950087057458	251.0
1.3015873015873016	1.2380952380952381	45.0
0.7865853658536586	0.5464939024390244	200.0
0.6781970649895178	0.5618448637316562	164.0
0.6865671641791045	0.5634328358208955	110.0
0.8540218470705064	0.6722939424031777	144.0
0.7534591194968554	0.7333333333333333	108.0
0.6923076923076923	0.5846153846153846	86.0
0.6428571428571429	0.9285714285714286	18.0
0.7814001372683597	0.63761153054221	203.0
0.6401673640167364	0.45188284518828453	123.0
0.5694444444444444	0.5277777777777778	61.0
0.6142433234421365	0.4896142433234421	103.0
0.8777506112469438	0.7775061124694377	104.0
0.5882352941176471	0.8823529411764706	40.0
0.755868544600939	0.5551643192488263	139.0
0.6847290640394089	0.5714285714285714	82.0
0.948076923076923	0.7615384615384615	93.0
0.7410926365795725	0.7600950118764845	131.0
0.7693430656934307	0.6233576642335766	195.0
0.5867469879518072	0.491566265060241	183.0
1.0851063829787233	0.7056737588652482	88.0
1.0	1.0	28.0
0.7414500683994528	0.5841313269493844	109.0
0.8146341463414634	0.6682926829268293	50.0
0.6738013698630136	0.5308219178082192	157.0
0.78125	0.5677083333333334	94.0
1.0769230769230769	0.5785953177257525	80.0
0.8431372549019608	0.9411764705882353	53.0
0.6975308641975309	0.5340848094471283	240.0
0.9523809523809523	0.9523809523809523	35.0
0.9504459861248761	0.8424182358771061	105.0
1.1172932330827068	0.9142857142857143	110.0
0.6169630642954856	0.4911080711354309	149.0
0.9367469879518072	0.7259036144578314	114.0
0.648936170212766	0.50177304964539	113.0
0.5783365570599613	0.504835589941973	111.0
1.0	1.0	4.0
0.5645161290322581	0.5	57.0
0.8	0.6333333333333333	42.0
0.712955779674166	0.5896043444530644	168.0
0.713302752293578	0.7018348623853211	99.0
0.5	0.47580645161290325	93.0
1.0	1.0	9.0
1.0	1.0	14.0
0.9217391304347826	0.5043478260869565	80.0
0.5034013605442177	0.46258503401360546	91.0
0.7644824311490979	0.6571699905033238	143.0
0.88268156424581	0.8100558659217877	39.0
0.88	0.8	26.0
0.7260821309655938	0.6235294117647059	240.0
0.65	0.4	69.0
0.9174977334542158	0.7769718948322756	185.0
0.6859688195991092	0.522271714922049	142.0
0.5323383084577115	0.6368159203980099	102.0
1.0	1.0	25.0
0.8497316636851521	0.6627906976744186	174.0
0.8163265306122449	0.6077097505668935	99.0
0.6263736263736264	0.5391941391941392	156.0
0.8062300130285444	0.589956176714438	309.0
0.7468354430379747	0.5009041591320073	121.0
1.5	0.9761904761904762	39.0
0.8793103448275862	0.6620689655172414	171.0
0.7345807345807346	0.5835065835065835	179.0
0.5357142857142857	0.4107142857142857	62.0
0.9344262295081968	0.9180327868852459	32.0
0.6069651741293532	0.5	126.0
1.0	1.0	15.0
0.7159090909090909	0.6388888888888888	104.0
0.8578367875647669	0.697538860103627	196.0
0.6591865357643759	0.45582047685834504	133.0
0.35714285714285715	0.6938775510204082	43.0
0.8591304347826086	0.7669565217391304	104.0
0.6444644464446445	0.5355535553555355	189.0
0.7150537634408602	0.5	118.0
0.6771369721936148	0.5550978372811535	226.0
0.6033653846153846	0.5697115384615384	87.0
0.815442561205273	0.564030131826742	213.0
0.8285714285714286	0.8285714285714286	43.0
0.6652173913043479	0.4369565217391304	135.0
0.6989966555183946	0.5886287625418061	108.0
0.8108108108108109	0.7117117117117117	68.0
0.4045307443365696	0.3268608414239482	93.0
0.7571428571428571	0.5452380952380952	115.0
0.6973684210526315	0.3815789473684211	53.0
1.2105263157894737	0.6842105263157895	24.0
0.9111111111111111	0.4666666666666667	55.0
1.0	1.0	5.0
1.0	1.0	27.0
0.6261491317671093	0.5081716036772217	219.0
0.8636363636363636	0.7181818181818181	88.0
0.3409090909090909	0.4090909090909091	59.0
0.7902097902097902	0.7097902097902098	79.0
0.7820965842167256	0.6222025912838633	244.0
0.8161865569272977	0.5651577503429356	140.0
0.5384615384615384	0.5384615384615384	37.0
0.744874715261959	0.5774487471526196	147.0
0.45098039215686275	0.5686274509803921	42.0
0.6849073256840247	0.5225066195939982	189.0
0.8650586701434159	0.6616688396349413	232.0
0.7090719499478624	0.64859228362878	109.0
0.7797270955165692	0.6237816764132553	87.0
1.0681818181818181	1.0681818181818181	47.0
0.773109243697479	0.634453781512605	106.0
0.5714285714285714	0.7142857142857143	38.0
0.603448275862069	0.7275862068965517	92.0
0.6267672007540056	0.527803958529689	140.0
1.0	1.0	13.0
1.0418006430868167	0.5627009646302251	99.0
0.803476581361661	0.6330275229357798	127.0
0.5465116279069767	0.8023255813953488	65.0
0.7842046718576196	0.6840934371523916	146.0
0.6656050955414012	0.5636942675159236	83.0
0.7211267605633803	0.5943661971830986	109.0
0.7378472222222222	0.5338541666666666	224.0
3.5	2.5	29.0
0.7745454545454545	0.6157575757575757	184.0
1.0	1.0	8.0
0.7868020304568528	0.6243654822335025	160.0
0.4	0.4	34.0
0.6571936056838366	0.4511545293072824	109.0
0.7139830508474576	0.5720338983050848	103.0
0.884090909090909	0.634090909090909	190.0
1.0	1.0	6.0
1.0	0.9239130434782609	85.0
0.8323699421965318	0.5375722543352601	98.0
1.0	1.0	12.0
1.5	1.5	17.0
1.0954198473282444	0.8129770992366412	93.0
0.704225352112676	0.5704225352112676	109.0
0.7476851851851852	0.5787037037037037	103.0
0.5912280701754385	0.5807017543859649	145.0
0.7475409836065574	0.4786885245901639	124.0
0.9163636363636364	0.7072727272727273	170.0
0.5733788395904437	0.5068259385665529	104.0
0.9140926640926641	0.693050193050193	129.0
0.7941176470588235	0.4579831932773109	132.0
0.6504854368932039	0.541747572815534	152.0
0.6140808344198174	0.4498044328552803	118.0
0.7456140350877193	0.6549707602339181	103.0
0.613413715146948	0.47098718914845517	174.0
0.5060240963855421	0.8192771084337349	61.0
0.8006012024048096	0.5968603874415498	223.0
0.9421052631578948	0.9210526315789473	51.0
1.0	1.0	11.0
0.7386363636363636	0.625	52.0
0.865	0.5625	112.0
2.0	0.0	18.0
0.6538461538461539	0.5	57.0
0.8659476117103235	0.674884437596302	124.0
0.2	0.4	22.0
0.7990654205607477	0.6401869158878505	157.0
0.7347347347347347	0.6646646646646647	139.0
0.7127659574468085	0.7606382978723404	91.0
0.7318435754189944	0.659217877094972	88.0
0.543046357615894	0.5562913907284768	63.0
1.375	1.4375	28.0
0.7839955232232793	0.6032456631225518	174.0
0.6119791666666666	0.6796875	110.0
0.5	0.5	24.0
0.6563706563706564	0.5984555984555985	167.0
0.5585284280936454	0.43478260869565216	90.0
0.9941176470588236	0.9441176470588235	79.0
0.7215320910973085	0.5279503105590062	164.0
0.6529175050301811	0.6217303822937625	130.0
0.3333333333333333	0.3333333333333333	20.0
0.6842105263157895	0.6289473684210526	190.0
0.7166666666666667	0.5972222222222222	125.0
0.6957801766437685	0.514720314033366	224.0
0.7649769585253456	0.7004608294930875	48.0
0.7682926829268293	0.5317073170731708	95.0
1.0	1.0	5.0
0.6521739130434783	0.6304347826086957	41.0
0.768491124260355	0.5850591715976331	172.0
0.45054945054945056	0.43956043956043955	69.0
0.5	0.5	27.0
0.7593984962406015	0.8120300751879699	64.0
1.0	1.0	13.0
0.8781362007168458	0.6666666666666666	135.0
0.763265306122449	0.8448979591836735	60.0
0.0	0.0	22.0
0.6575342465753424	0.6986301369863014	82.0
0.8245614035087719	0.7894736842105263	63.0
0.749595600129408	0.5988353283726949	237.0
0.6851211072664359	0.5259515570934256	120.0
0.7050691244239631	0.5990783410138248	88.0
0.7334630350194552	0.4377431906614786	133.0


==> ncrDA_praline-package-2020-05-18.tex <==
bfs/rand	fd/rand	vtcs
1.0	1.0	8.0
0.4343558282208589	0.41226993865030676	169.0
0.40540540540540543	0.4594594594594595	50.0
0.49279538904899134	0.4092219020172911	104.0
1.0393700787401574	1.2283464566929134	44.0
1.0	1.0	8.0
0.43918053777208704	0.38412291933418696	201.0
0.5899843505477308	0.514866979655712	197.0
0.44959128065395093	0.335149863760218	119.0
0.8571428571428571	0.7857142857142857	27.0
0.45513513513513515	0.5027027027027027	156.0
0.5134408602150538	0.3709677419354839	119.0
0.6	0.2923076923076923	86.0
0.5354107648725213	0.3314447592067989	121.0
0.6511627906976745	0.47674418604651164	95.0
0.6073619631901841	0.3540753724802805	231.0
0.4462686567164179	0.46417910447761196	169.0
0.5614035087719298	0.5877192982456141	126.0
0.0	0.0	28.0
0.525	0.4857142857142857	101.0
0.47619047619047616	0.38095238095238093	27.0
1.0	1.0	11.0
0.723404255319149	0.48936170212765956	112.0
0.2222222222222222	0.2345679012345679	77.0
0.6384872080088988	0.44493882091212456	134.0
1.015267175572519	0.5038167938931297	86.0
0.5936199722607489	0.37170596393897365	131.0
0.45789473684210524	0.34210526315789475	122.0
1.0	1.0	5.0
0.7797619047619048	0.8422619047619048	86.0
0.36666666666666664	0.43333333333333335	48.0
0.56	0.48	26.0
0.7857142857142857	0.5714285714285714	28.0
0.473015873015873	0.2571428571428571	134.0
0.437219730941704	0.3721973094170404	133.0
0.14285714285714285	0.6428571428571429	41.0
0.6551724137931034	0.6206896551724138	93.0
0.705607476635514	0.5809968847352025	154.0
0.5997993981945837	0.5366098294884654	194.0
0.6832504145936982	0.5146489773355445	209.0
0.44495412844036697	0.22935779816513763	110.0
0.6511627906976745	0.6201550387596899	113.0
0.4742268041237113	0.5567010309278351	62.0
0.6318593500266383	0.3937133724027704	202.0
0.4519230769230769	0.4807692307692308	134.0
1.0	1.0	18.0
0.768837803320562	0.6551724137931034	105.0
0.4846938775510204	0.4107142857142857	139.0
0.5440944881889764	0.40393700787401576	180.0
0.4511784511784512	0.2727272727272727	194.0
0.6051758460517584	0.49878345498783455	354.0
1.0	1.0	11.0
0.5591397849462365	0.489247311827957	98.0
0.9314205738278516	0.5472358292512246	235.0
0.6222961730449251	0.5490848585690515	163.0
0.5780669144981413	0.4721189591078067	168.0
0.46511627906976744	0.4697674418604651	128.0
0.5550847457627118	0.3785310734463277	205.0
0.8148148148148148	0.7407407407407407	50.0
0.7732394366197183	0.6140845070422535	218.0
0.8461538461538461	0.5701357466063348	80.0
0.4863849765258216	0.47699530516431926	170.0
0.509090909090909	0.2636363636363636	113.0
0.0	0.0	17.0
1.0	1.0	5.0
0.47305389221556887	0.3023952095808383	147.0
0.5037234042553191	0.43031914893617024	199.0
0.7142857142857143	0.5840336134453782	63.0
0.0	1.0	36.0
1.1428571428571428	1.2142857142857142	44.0
1.0	1.0	13.0
0.5971223021582733	0.5582733812949641	226.0
0.7985347985347986	0.5311355311355311	115.0
0.7014767932489452	0.4630801687763713	241.0
0.67890625	0.4875	241.0
0.6479885057471264	0.5517241379310345	184.0
0.5118483412322274	0.4052132701421801	156.0
0.6761229314420804	0.491725768321513	134.0
0.5040106951871658	0.3622994652406417	168.0
0.8481675392670157	0.6649214659685864	123.0
0.65	0.44166666666666665	146.0
0.6393762183235867	0.4873294346978557	144.0
0.9142857142857143	0.4857142857142857	55.0
0.2903225806451613	0.25806451612903225	55.0
1.0	1.0	7.0
0.601123595505618	0.4438202247191011	159.0
0.5642398286937902	0.430406852248394	194.0
1.0	1.0	17.0
0.449438202247191	0.4943820224719101	86.0
1.0	1.0	18.0
0.36764705882352944	0.3161764705882353	87.0
0.5500878734622144	0.4358523725834798	190.0
1.0	1.0	35.0
0.5350553505535055	0.4317343173431734	122.0
0.39552238805970147	0.3283582089552239	152.0
0.4983277591973244	0.3110367892976589	120.0
0.5769230769230769	0.6461538461538462	124.0
0.5461165048543689	0.4441747572815534	225.0
0.5157894736842106	0.45263157894736844	73.0
0.25	0.5	38.0
0.6896551724137931	0.5862068965517241	45.0
1.5	1.5	15.0
0.49603174603174605	0.5079365079365079	130.0
0.0	0.0	20.0
0.5670103092783505	0.5360824742268041	120.0
0.6410256410256411	0.5897435897435898	60.0
0.3649025069637883	0.30362116991643456	102.0
0.6514611546685674	0.391304347826087	254.0
0.9264816204051013	0.5041260315078769	157.0
0.6328125	0.4609375	102.0
0.6281431334622823	0.5527079303675049	230.0
0.8452451269935026	0.5339633786178382	244.0
1.0	1.0	8.0
0.3912175648702595	0.3193612774451098	144.0
0.8936170212765957	0.8014184397163121	80.0
0.7908496732026143	0.45751633986928103	112.0
0.6666666666666666	0.4666666666666667	39.0
0.515527950310559	0.4658385093167702	91.0
0.651528384279476	0.6323144104803493	121.0
0.784639746634996	0.6104513064133017	132.0
0.43243243243243246	0.27927927927927926	89.0
0.5811373092926491	0.44105409153952846	170.0
0.8156424581005587	1.0223463687150838	53.0
0.7409579667644184	0.4858260019550342	171.0
0.5776209677419355	0.4183467741935484	170.0
0.32857142857142857	0.38571428571428573	63.0
0.6823899371069182	0.4371069182389937	187.0
0.5552631578947368	0.46578947368421053	147.0
0.7821782178217822	0.48514851485148514	79.0
0.5922038980509745	0.4407796101949025	168.0
0.10344827586206896	0.4827586206896552	48.0
1.0	1.0	18.0
0.7337883959044369	0.5085324232081911	111.0
0.5555555555555556	0.494949494949495	49.0
0.5859247135842881	0.4337152209492635	186.0
0.6772486772486772	0.47619047619047616	142.0
0.6013071895424836	0.7320261437908496	69.0
0.4954954954954955	0.32432432432432434	62.0
0.7211328976034859	0.6078431372549019	122.0
0.6967741935483871	0.614516129032258	127.0
0.42105263157894735	0.6842105263157895	60.0
0.47701149425287354	0.33620689655172414	193.0
1.3181818181818181	0.6363636363636364	47.0
1.0638297872340425	0.7127659574468085	61.0
1.0	1.0	43.0
1.0	1.0	21.0
0.5917836713468538	0.5949037961518461	237.0
0.30952380952380953	0.40476190476190477	40.0
1.0	1.0	21.0
0.48777648428405124	0.4051222351571595	246.0
0.56	0.2	55.0
0.5688259109311741	0.3967611336032389	163.0
0.5818181818181818	0.38181818181818183	145.0
1.0649350649350648	0.9090909090909091	37.0
0.5555555555555556	0.8888888888888888	41.0
0.7777777777777778	0.6339181286549708	149.0
0.21428571428571427	0.35714285714285715	44.0
0.5107296137339056	0.31759656652360513	107.0
0.549079754601227	0.5276073619631901	97.0
0.6677631578947368	0.27631578947368424	114.0
0.6720977596741344	0.3604887983706721	169.0
1.0	1.0	8.0
0.4218009478672986	0.27488151658767773	109.0
0.559322033898305	0.4915254237288136	120.0
0.38450502152080346	0.4332855093256815	188.0
1.0	1.0	10.0
0.5862433862433862	0.42433862433862435	158.0
1.0	2.0	2.0
1.0	0.6666666666666666	34.0
0.5872340425531914	0.47801418439716314	178.0
0.6944444444444444	0.44565217391304346	170.0
0.3125	0.375	65.0
2.0	2.0	8.0
0.6918429003021148	0.47129909365558914	111.0
0.4936708860759494	0.5063291139240507	113.0
0.4117647058823529	0.3284313725490196	91.0
0.6035087719298246	0.2982456140350877	131.0
0.7549019607843137	0.5686274509803921	102.0
0.3076923076923077	0.6153846153846154	33.0
1.0	1.0	14.0
0.25	0.5	24.0
0.15384615384615385	0.3076923076923077	87.0
1.0	1.0	8.0
0.5220125786163522	0.44025157232704404	190.0
1.0	1.0	14.0
0.4968152866242038	0.46496815286624205	99.0
0.6643625192012289	0.6766513056835638	127.0
0.4810810810810811	0.33513513513513515	115.0
0.2692307692307692	0.25	58.0
0.5806451612903226	0.5668202764976958	120.0
0.7034035656401945	0.4991896272285251	153.0
0.5135135135135135	0.5675675675675675	50.0
0.5281501340482574	0.42359249329758714	105.0
1.103448275862069	1.1379310344827587	79.0
0.7997967479674797	0.6859756097560976	121.0
0.6840113528855251	0.609271523178808	130.0
0.5458646616541354	0.4150375939849624	168.0
0.8042105263157895	0.5511578947368421	202.0
0.2857142857142857	0.2571428571428571	67.0
0.6652542372881356	0.538135593220339	123.0
0.39705882352941174	0.23529411764705882	66.0
0.5238095238095238	0.9629629629629629	97.0
0.6019522776572668	0.5216919739696312	172.0
0.06451612903225806	0.5806451612903226	66.0
0.5705368289637952	0.36704119850187267	173.0
0.6599552572706935	0.6062639821029083	99.0
0.7830882352941176	0.5367647058823529	126.0
0.3333333333333333	0.0	18.0
1.0	1.0	15.0
1.0714285714285714	0.9285714285714286	26.0
0.6666666666666666	0.572463768115942	138.0
1.0	1.0	7.0
0.6646551724137931	0.4543103448275862	168.0
1.25	0.75	30.0
0.26785714285714285	0.2857142857142857	54.0
0.5222222222222223	0.6222222222222222	113.0
0.6612903225806451	0.45161290322580644	37.0
0.5817843866171004	0.4275092936802974	148.0
0.782051282051282	0.8846153846153846	70.0
0.34444444444444444	0.3074074074074074	133.0
0.48257372654155495	0.3136729222520107	132.0
0.4594594594594595	0.40124740124740127	157.0
0.4074074074074074	0.37037037037037035	67.0
1.0	1.0	18.0
0.6666666666666666	0.8571428571428571	71.0
0.6535433070866141	0.5748031496062992	82.0
0.4489795918367347	0.37244897959183676	117.0
0.49507389162561577	0.29064039408866993	126.0
0.6891405043746783	0.5115800308800823	234.0
0.46119402985074626	0.2701492537313433	143.0
0.5983935742971888	0.6947791164658634	93.0
0.7941176470588235	0.8823529411764706	37.0
0.20952380952380953	0.3238095238095238	99.0
0.4666666666666667	0.37333333333333335	100.0
0.6940298507462687	0.5074626865671642	91.0
0.783410138248848	0.6350230414746544	122.0
0.7723785166240409	0.4437340153452685	169.0
0.548951048951049	0.4195804195804196	122.0
0.5347043701799485	0.4498714652956298	95.0
0.4756554307116105	0.4419475655430712	126.0
0.7283702213279678	0.4607645875251509	157.0
0.5	0.5	14.0
0.6	1.0	63.0
0.26506024096385544	0.2921686746987952	104.0
0.29394812680115273	0.34870317002881845	113.0
0.5	0.25	27.0
0.36363636363636365	0.4090909090909091	55.0
0.5289323553382234	0.4938875305623472	148.0
0.4	0.7	60.0
0.6216908625106746	0.47993168232280103	186.0
0.6278026905829597	0.5919282511210763	141.0
0.7969598262757872	0.6840390879478827	153.0
0.5421686746987951	0.43775100401606426	115.0
0.7170953101361573	0.5726172465960666	162.0
0.4393939393939394	0.48484848484848486	122.0
0.9	0.92	43.0
0.5432692307692307	0.3894230769230769	107.0
0.6353646353646354	0.4485514485514486	245.0
0.6197860962566845	0.4711229946524064	245.0
1.0	1.0	11.0
1.0	0.975609756097561	53.0
0.7485714285714286	0.44	142.0
0.9541284403669725	0.7247706422018348	107.0
0.7721088435374149	0.6462585034013606	113.0
0.0	0.0	32.0
0.45714285714285713	0.3	77.0
0.5638297872340425	0.5212765957446809	129.0
0.39858490566037735	0.2617924528301887	118.0
0.6252189141856392	0.404553415061296	135.0
0.749031007751938	0.42151162790697677	182.0
0.5066666666666667	0.5422222222222223	96.0
0.6153846153846154	0.6025641025641025	80.0
0.26	0.7	52.0
1.0	1.0	10.0
0.8184615384615385	0.64	133.0
0.5666666666666667	0.4543859649122807	241.0
0.6991150442477876	0.497787610619469	111.0
0.42	0.38	41.0
0.2905982905982906	0.3504273504273504	87.0
0.6062215477996965	0.5455235204855842	219.0
0.5942622950819673	0.430327868852459	165.0
1.0	1.0	5.0
0.5098039215686274	0.3627450980392157	58.0
0.5544303797468354	0.49873417721518987	164.0
0.3850267379679144	0.35294117647058826	92.0
0.5488721804511278	0.6766917293233082	94.0
0.9985163204747775	0.8056379821958457	112.0
0.2	0.3142857142857143	62.0
1.0	1.0	14.0
0.7282608695652174	0.3967391304347826	105.0
0.55	0.55	82.0
1.1111111111111112	1.0222222222222221	56.0
1.0	1.0	18.0
0.6134215500945179	0.4678638941398866	197.0
0.47692307692307695	0.4307692307692308	105.0
0.288135593220339	0.2824858757062147	105.0
0.5368567454798331	0.4728789986091794	164.0
2.0	1.0	31.0
0.7235649546827795	0.44561933534743203	156.0
0.4588744588744589	0.49783549783549785	107.0
0.6666666666666666	0.4074074074074074	78.0
0.34600760456273766	0.311787072243346	130.0
0.7168576104746317	0.5875613747954174	128.0
0.46551724137931033	0.3775862068965517	144.0
0.4474708171206226	0.49416342412451364	91.0
0.9873417721518988	0.8164556962025317	38.0
0.4523809523809524	0.5	105.0
0.6263736263736264	0.5879120879120879	69.0
0.7860615883306321	0.5235008103727715	113.0
0.5831381733021077	0.48243559718969553	156.0
0.44299674267100975	0.36482084690553745	115.0
0.5139211136890951	0.4071925754060325	217.0
0.0	0.2222222222222222	40.0
0.8837209302325582	0.7906976744186046	43.0
0.22807017543859648	0.17543859649122806	92.0
0.6672268907563025	0.446218487394958	166.0
0.4300341296928328	0.3310580204778157	150.0
1.0434782608695652	0.8695652173913043	95.0
1.0	2.0	2.0
0.8	0.6	47.0
0.681184668989547	0.5296167247386759	147.0
0.23863636363636365	0.14772727272727273	76.0
0.16666666666666666	0.3333333333333333	69.0
0.6071428571428571	0.6428571428571429	49.0
0.5357590966122961	0.4328732747804266	174.0
0.6858638743455497	0.643979057591623	92.0
0.5041551246537396	0.5401662049861495	145.0
0.0	0.0	13.0
0.5592592592592592	0.3907407407407407	139.0
0.5833333333333334	0.5416666666666666	40.0
0.5924908424908425	0.5952380952380952	123.0
0.2692307692307692	0.3076923076923077	60.0
0.6451612903225806	0.3870967741935484	40.0
0.41304347826086957	0.34782608695652173	47.0
0.23076923076923078	0.717948717948718	51.0
0.8108974358974359	0.5705128205128205	239.0
0.5654761904761905	0.30952380952380953	84.0
0.5907172995780591	0.5063291139240507	115.0
0.597444089456869	0.45580404685835996	187.0
0.6449086161879896	0.5718015665796344	160.0
0.5454545454545454	0.45454545454545453	39.0
0.5645161290322581	0.5967741935483871	54.0
0.5796178343949044	0.5732484076433121	102.0
1.0	1.0	21.0
0.8624288425047438	0.560404807084124	313.0
0.4030612244897959	0.413265306122449	100.0
0.6018181818181818	0.38181818181818183	144.0
0.5063291139240507	0.2848101265822785	93.0
0.7271794871794872	0.5538461538461539	234.0
0.5414012738853503	0.3980891719745223	131.0
0.5158730158730159	0.35714285714285715	97.0
0.6300884955752213	0.5132743362831859	171.0
0.3888888888888889	0.36944444444444446	133.0
0.5605786618444847	0.3960216998191682	141.0
0.46808510638297873	0.574468085106383	80.0
0.0	0.0	35.0
0.5254901960784314	0.5333333333333333	131.0
0.9047619047619048	0.9047619047619048	25.0
0.46511627906976744	0.4069767441860465	84.0
0.5904255319148937	0.3882978723404255	89.0
0.8785714285714286	0.8785714285714286	27.0
0.6035007610350076	0.4299847792998478	224.0
0.6128226477935054	0.5378850957535387	159.0
0.7129186602870813	0.5358851674641149	107.0
0.2857142857142857	0.42857142857142855	27.0
0.21296296296296297	0.37037037037037035	85.0
0.6324582338902148	0.5316229116945107	241.0
0.6585365853658537	0.583739837398374	130.0
1.0	1.0	11.0
0.6123032904148784	0.547925608011445	114.0
0.7428571428571429	0.6	68.0
0.0	0.0	22.0
0.7724358974358975	0.7275641025641025	130.0
0.8	0.5222222222222223	117.0
0.48109965635738833	0.5395189003436426	131.0
0.4	0.6	31.0
1.0	1.0	14.0
0.3132530120481928	0.27710843373493976	85.0
0.7935222672064778	0.4742625795257374	212.0
0.6422521175884405	0.40308918784255104	230.0

